An Analysis of Concurrency Control Protocols for In-Memory Databases with CCBench (Extended Version)

This paper presents yet another concurrency control analysis platform, CCBench. CCBench supports seven protocols (Silo, TicToc, MOCC, Cicada, SI, SI with latch-free SSN, 2PL) and seven versatile optimization methods and enables the configuration of seven workload parameters. We analyzed the protocols and optimization methods using various workload parameters and a thread count of 224. Previous studies focused on thread scalability and did not explore the space analyzed here. We classified the optimization methods on the basis of three performance factors: CPU cache, delay on conflict, and version lifetime. Analyses using CCBench and 224 threads, produced six insights. (I1) The performance of optimistic concurrency control protocol for a read only workload rapidly degrades as cardinality increases even without L3 cache misses. (I2) Silo can outperform TicToc for some write-intensive workloads by using invisible reads optimization. (I3) The effectiveness of two approaches to coping with conflict (wait and no-wait) depends on the situation. (I4) OCC reads the same record two or more times if a concurrent transaction interruption occurs, which can improve performance. (I5) Mixing different implementations is inappropriate for deep analysis. (I6) Even a state-of-the-art garbage collection method cannot improve the performance of multi-version protocols if there is a single long transaction mixed into the workload. On the basis of I4, we defined the read phase extension optimization in which an artificial delay is added to the read phase. On the basis of I6, we defined the aggressive garbage collection optimization in which even visible versions are collected. The code for CCBench and all the data in this paper are available online at GitHub.

==> README <==
As of 2021, 8/18, 
I succeeded to typeset this article using "pdflatex". To upload an article to arXiv, one needs to use pdflatex instead of platex. This is very important. The former version can be compiled using platex, but it cannot be using pdflatex because the following commands did not work for pdflatex. Please do not forget that pdflatex is required to upload your manuscript to arXiv.

% make caption info bold
%\makeatletter
%\long\def\@makecaption#1#2{%redefine \@makecaption
%\vskip\abovecaptionskip
%\iftdir\sbox\@tempboxa{#1\hskip1zw#2}%
%\else\sbox\@tempboxa{\textbf{#1:} #2}%revise
%\fi
%\ifdim \wd\@tempboxa >\hsize%
%\iftdir #1\hskip1zw#2\relax\par
%\else \textbf{#1:} #2\relax\par\fi%revise
%\else
%\global \@minipagefalse
%\hbox to\hsize{\hfil\box\@tempboxa\hfil}
%\fi
%\vskip\belowcaptionskip}
%\makeatother        


8/18, 2021, Hideyuki Kawashima

==> err <==
This is pdfTeX, Version 3.14159265-2.6-1.40.20 (TeX Live 2019/Debian) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2020-02-02> patch level 2
L3 programming layer <2020-02-14> (./vldb.cls
(/usr/share/texlive/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/share/texlive/texmf-dist/tex/generic/iftex/ifvtex.sty
(/usr/share/texlive/texmf-dist/tex/generic/iftex/iftex.sty)))
(/usr/share/texlive/texmf-dist/tex/latex/graphics/epsfig.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/share/texlive/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/graphics-def/dvipdfmx.def))))
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsopn.sty))
Document Class 'vldb' - based on 'sig-alternate' <26th. July '05>. Modified by 
G.K.M. Tobin/Gerry Murray
Based in part upon document Style `acmconf' <22 May 89>. Hacked 4/91 by
shivers@cs.cmu.edu, 4/93 by theobald@cs.mcgill.ca
Excerpts were taken from (Journal Style) 'esub2acm.cls'.
****** Bugs/comments/suggestions/technicalities to Gerry Murray -- murray@hq.ac
m.org ******
Questions on the style, SIGS policies, etc. to Adrienne Griscti griscti@acm.org

Document Class: vldb 2010/10/19 - V1.8b - based on sig-alternate V1.8 - based o
n acmproc.cls V1.3 <Nov. 30 '99>
(/usr/share/texlive/texmf-dist/tex/latex/base/latexsym.sty)
Using 'Abbrev' bibliography style
) (./header.tex (/usr/share/texlive/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/share/texlive/texmf-dist/tex/latex/caption/caption.sty
(/usr/share/texlive/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

) (/usr/share/texlive/texmf-dist/tex/latex/caption/subcaption.sty)
(/usr/share/texlive/texmf-dist/tex/latex/ascmac/ascmac.sty
(/usr/share/texlive/texmf-dist/tex/latex/ascmac/tascmac.sty))
(/usr/share/texlive/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/share/texlive/texmf-dist/tex/latex/seqsplit/seqsplit.sty)
(/usr/share/texlive/texmf-dist/tex/latex/graphics/color.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/url/url.sty)
(/usr/share/texlive/texmf-dist/tex/latex/cite/cite.sty)

! LaTeX3 Error: Backend request inconsistent with engine: using 'pdfmode'
(LaTeX3)        backend.

For immediate help type H <return>.
 ...                                              
                                                  
l.50 \begin{document}
                     
? No pages of output.
Transcript written on main.log.


==> letter/core-item.tex <==
\begin{itemize}
 \item Comment by Meta-Reviewer

       \begin{screen}
	If you want, you can include a summary of the results in the main body of the paper and cite an extended version that has more detailed numbers, such as a technical report or arXiv submission. In that case, we would like to see the latter too, before approving the revision for publication.	
       \end{screen}

 \item Response to Comment by Meta-Reviewer

       Thank you for your comment.
       Since the contents about TPC-C was not short, we made an extended version, {\tt arXiv.pdf}.
       Evaluation regarding to TPC-C is described in the Appendix of {\tt arXiv.pdf}.
       %
       The file for VLDB version is {\tt pvldb.pdf}, and we are happy if you find the summary of the results in Section 3.4 (in \color{blue} blue color\color{black})
       in {\tt pvldb.pdf} and {\tt arXiv.pdf}.
       
 \item Comment 1 by Reviewers

       \begin{screen}
	Therefore, if you don’t implement full TPC-C, but do a thorough job with the experimental analysis of the two update transactions, and explain the likely performance implications of the three missing queries, we will still accept the paper, provided that you also promise to publish full TPC-C results in the near future.
       \end{screen}
       
 \item Response to Comment 1 by Reviewers
       
       % NP, not full-mix
       We did not implement TPC-C full-mix, and we instead implemented two (NewOrder and Payment) out of five transactions in TPC-C. 
       We refer to this workload as NP.
       %
       % Two variants
       We implemented two variants of NP.
       They are without insertion and with insertion, and they are referred to as NP-Insert and NP-NoInsert, respectively.
       Both of them were also supported by the DBx1000 system.
       %
       % Silo only 
       Among protocols, CCBench currently supports only Silo.
       The effort to implement insertion operation was not small because
       it required not only the revision of protocol itself,
       but also the fix of two bugs in publicly available Masstree.
       The details are described in the Appendix of {\tt arXiv.pdf}.
       %The bug fixes are as follows, and we cite them in the arXiv version.
       \if 0
       \begin{enumerate}
	\item Debug Masstree about Cast.\\
	      {\tt https://github.com/thawk105/masstree-beta/commit/\\
	      d4bcf7711dc027818b1719a5a4c29aee547c58f6.}
	\item Debug Masstree about string slice.hh.\\
	      {\tt https://github.com/thawk105/masstree-beta/commit/\\
	      77ef355f868a6db4eac7b44669c508d8db053502.}
       \end{enumerate}
       \fi
       Thus we could not implement other protocols within the limited time.
       % Promise
       However, we promise you that we will add TPC-C full-mix in the near future.
       This promise is described not only in this letter, but also in the Appendix of {\tt arXiv.pdf}
       (in \color{blue} blue color\color{black}).

       \if 0
       % Justification
       We evaluated the workloads using CCBench, the original DBx1000, and an extension of DBx1000 by Cicada team in {\rm Appendix A.3.1}.
       The results were consistent with prior work.
       We found that the performances of {\rm NP-Insert} were much lower than {\rm NP-NoInsert} there.
       Thus, the insertion operation can deteriorate performance.
       
       % New knowledge
       To explore the reasons for performance deterioration, 
       we analyzed the impact of index accesses to performance in {\rm Appendix A.3.1}.
       We found that execution times of 68.4\% and 58.9\% 
       were spent respectively for {\tt New-Order} and {\tt Payment} transactions on search, update, and insert.
       These operations need to find a record, and require frequent Masstree traversal.
       Thus, we claim that the acceleration of tree indexes is vital to make TPC-C efficient.

       % More than NP
       We also discussed the difference between NP and full-mix in {\rm Appendix A.3.3}.
       If full-mix workload, which includes all of five transactions, its performance would deteriorate to a fraction of NP. This is shown in the original Cicada paper.
       The reason for the performance degradation is due to the large {\tt Delivery} transaction.
       %
       \fi
 \item Comment 2 by Reviewers

       \begin{screen}
       Your VLDB paper should cite an extended version (e.g., as a technical report or arXiv paper)  “to appear”, which includes the full TPC-C results. The TPC-C implementation should  be serializable, meaning that it has B-Trees or other ordered data structures that avoids phantoms and the write skew problem that can occur with snapshot isolation.
       \end{screen}
	
 \item Response to Comment 2 by Reviewers

       Thank you for your comment.
       %
       The file {\tt pvldb.pdf} cites the arXiv version as follows.
       
       \begin{screen}
	$\left[ 50 \right]$ T. Tanabe, T. Hoshino, H. Kawashima, and O. Tatebe. An Analysis of Concurrency Control Protocols for In-Memory Database with CCBench (Extended Version). {\tt http://arxiv.org/abs/XXX.YYY}, 2020.
       \end{screen}

       If our paper is accepted, then we will update {\tt XXX.YYY} in {\tt pvldb.pdf} and upload {\tt arXiv.pdf} to arXiv.
       After implementing and evaluating TPC-C full-mix, we will update contents of the extended version to the arXiv.org.

\end{itemize}


==> letter/err <==
pdflatex main.tex
This is pdfTeX, Version 3.14159265-2.6-1.40.18 (TeX Live 2017/Debian) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2017-04-15>
Babel <3.18> and hyphenation patterns for 30 language(s) loaded.
(/usr/share/texlive/texmf-dist/tex/latex/base/letter.cls
Document Class: letter 2014/09/29 v1.2z Standard LaTeX document class
(/usr/share/texlive/texmf-dist/tex/latex/base/size11.clo))
(/usr/share/texlive/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ifpdf.sty)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ifvtex.sty)
(/usr/share/texlive/texmf-dist/tex/generic/ifxetex/ifxetex.sty))
(/usr/share/texlive/texmf-dist/tex/latex/base/fontenc.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/t1enc.def))
(/usr/share/texlive/texmf-dist/tex/latex/base/inputenc.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/utf8.def
(/usr/share/texlive/texmf-dist/tex/latex/base/t1enc.dfu)
(/usr/share/texlive/texmf-dist/tex/latex/base/ot1enc.dfu)
(/usr/share/texlive/texmf-dist/tex/latex/base/omsenc.dfu)))
(/usr/share/texlive/texmf-dist/tex/latex/stix/stix.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/textcomp.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/ts1enc.def
(/usr/share/texlive/texmf-dist/tex/latex/base/ts1enc.dfu))))
(/usr/share/texlive/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/share/texlive/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/share/texlive/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/graphics/color.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics-cfg/color.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/graphics-def/pdftex.def))
(/usr/share/texlive/texmf-dist/tex/platex/base/ascmac.sty
(/usr/share/texlive/texmf-dist/tex/platex/base/tascmac.sty{/var/lib/texmf/fonts
/map/pdftex/updmap/pdftex.map})) (./main.aux)
(/usr/share/texlive/texmf-dist/tex/latex/base/ts1cmr.fd)
(/usr/share/texlive/texmf-dist/tex/latex/stix/ls1stix.fd)
(/usr/share/texlive/texmf-dist/tex/latex/stix/ls2stix.fd)
(/usr/share/texlive/texmf-dist/tex/latex/stix/t1stix.fd)
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
(/usr/share/texlive/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/share/texlive/texmf-dist/tex/latex/stix/ls1stixscr.fd)
(/usr/share/texlive/texmf-dist/tex/latex/stix/ls2stixex.fd)
(/usr/share/texlive/texmf-dist/tex/latex/stix/ls1stixfrak.fd)
(/usr/share/texlive/texmf-dist/tex/latex/stix/ls1stixbb.fd)
(/usr/share/texlive/texmf-dist/tex/latex/stix/ls2stixcal.fd)
(/usr/share/texlive/texmf-dist/tex/latex/stix/ls1stixsf.fd)
(/usr/share/texlive/texmf-dist/tex/latex/stix/ls2stixtt.fd)
Underfull \hbox (badness 10000) in paragraph at lines 80--87


Underfull \hbox (badness 1348) in paragraph at lines 80--87
\T1/stix/m/n/10.95 (+20) Therefore, if you don't im-ple-ment full TPC-C, but do
 a thor-ough

Underfull \hbox (badness 10000) in paragraph at lines 80--87

(./core-item.tex (/usr/share/texlive/texmf-dist/tex/latex/stix/ts1stix.fd)
[1] (/usr/share/texlive/texmf-dist/tex/latex/base/t1cmtt.fd)
(/usr/share/texlive/texmf-dist/tex/latex/base/t1cmss.fd)
Overfull \hbox (1.36275pt too wide) in paragraph at lines 50--56
\T1/cmtt/m/n/10.95 New-Order \T1/stix/m/n/10.95 (-20) and \T1/cmtt/m/n/10.95 Pa
yment \T1/stix/m/n/10.95 (-20) trans-ac-tions on search, up-date, and in-sert. 
These
[2
! pdfTeX error (font expansion): auto expansion is only possible with scalable 
fonts.
<to be read again> 
                   \endgroup \set@typeset@protect 
l.80 \end{itemize}
                  
!  ==> Fatal error occurred, no output PDF file produced!
Transcript written on main.log.
Makefile:4: recipe for target 'main.pdf' failed
make: *** [main.pdf] Error 1


==> letter/tmp/core.tex <==
  \subsection{Comment 1.}
   \subsubsection{Comment}     
   If you don’t implement full TPC-C, but do a thorough job with the experimental analysis of the two update transactions, and explain the likely performance implications of the three missing queries, we will still accept the paper, provided that you also promise to publish full TPC-C results in the near future.
       
   \subsubsection{Response}     
   Thank you for your comment.
   
   % NP, not full-mix
   We did not implement TPC-C full-mix.
   We instead implemented two (Payment and NewOrder) out of five transactions in TPC-C. 
   We refer to this workload as TPC-C-NP.

       % Two variants
       We implemented two variants of TPC-C-NP.
       They are without insertion and with insertion.
       We refer to them as TPC-C-NP-Insert and TPC-C-NP-NoInsert, respectively.
       Both TPC-C-NP-NoInsert and TPC-C-NP-Insert are also supported by DBx1000.
       % Silo only 
       Among protocols, CCBench currently supports only Silo.
       The effort to support insertion operation was large.
       It required not only the revision of protocol itself,
       but also the debug of Masstree.
       Thus we could not implement other protocols.
       % Promise
       However, we promise you that we will add the other six protocols for TPC-C full-mix in the near future.
       
       % Justification
       We evaluated the workloads using CCBench, the original DBx1000, and an extension of DBx1000 by Cicada team. The results were consistent with prior work.
       % mouchoi-kaku?
       
       % New knowledge
       We To understand the impact of index to performance,
       we measured latency breakdown of transactions in NP-Insert workload of CCBench on 224 threads and 224 warehouses using the Linux perf tool.
       %
       %       As shown in Fig. \ref{fig:breakdown}, execution times of 68.4\% and 58.9\%
       We found that execution times of 68.4\% and 58.9\% 
       were spent respectively for {\tt New-Order} and {\tt Payment} transactions on search, update, and insert.
       %This is due to the Masstree traversal.
       These operations need to find a record, and require frequent Masstree traversal. 
       We also observed 44.2\% time of transactions was spent to Masstree traversal.
       %access method in CCBench is Masstree. Thus, they frequently performed Masstree traversal.
       %64.6\% and 75.0\% of execution time were spent for Masstree processing in NewOrder and Payment respectively.
       Since the size of Masstree node is a few hundred bytes, its traversal decreases the spatial locality of memory accesses, so cache miss tends to increases.
       NP can be executed using only hash index without tree-index.
       In that case, the ratio of search, update, and insert to the execution time would be greatly reduced, and the performance of NP would improve.
       
       \subsection{Comment 2}
       \subsubsection{Comment}            
       Your VLDB paper should cite an extended version (e.g., as a technical report or arXiv paper)  “to appear”, which includes the full TPC-C results. The TPC-C implementation should be serializable, meaning that it has B-Trees or other ordered data structures that avoids phantoms and the write skew problem that can occur with snapshot isolation.

       \subsubsection{Response}
       Thank you for your comment.
       We described additional contents about TPC-C in Appendix, and plan to submit it to arXiv.
       Our PVLDB version currently cites the arXiv version as follows.
       If our PVLDB version is accepted, then we will update {\tt XXX.YYY}.
       Besides, after implementing and evaluating TPC-C full-mix, we will update the arXiv paper.
       
        \begin{screen}
	 $\left[ 61 \right]$ T. Tanabe, T. Hoshino, H. Kawashima, and O. Tatebe. An Analysis of Concurrency Control
	 Protocols for In-Memory Database with CCBench (Extended Version). {\tt http://arxiv.org/abs/XXX.YYY}, 2020.
	\end{screen}

==> src/diff.tex <==
In our setting, we applied the RapidGC to ERMIA and SI in all the cases, NoWaitto Silo in Fig. \ref{fig:ycsbA_tuple100m_skew09_slprp0-1000_tps}, and adaptive backoff to TicToc in Fig. \ref{fig:tuple10m_val1k_ycsb_high_tps}


==> src/fullmix_v1.tex <==
\section{Evaluation of a TPC-C Full-mix}
TPC-C full-mix consists of five transactions. They are \\
{\tt New-Order}, {\tt Payment}, {\tt Delivery}, {\tt Stock-Level}, {\tt Order-Status}.
%
The percentages of them are 45, 43, 4, 4, and 4 percent, respectively.
%
We designed and implemented TPC-C full-mix for Silo in CCBench.
%
For that, we designed and implemented a robust and efficient Masstree.
%
We denote our own Masstree implementation as {\sl Yakushima} in this paper.
%
The code for this version of CCBench and {\sl Yakushima} is not publicly available currently at GitHub~\cite{thawkccbench}.
%However, we are working to release them.

\subsection{Yakushima}
We redesigned Masstree~\cite{mao2012cache} to provide robustness and efficiency.
%
We provide two optimizations on {\sl Yakushima}.
%
The first optimization of {\sl Yakushima} is related to the retry processing of tree traversal. When a tree traverse fails due to a write, the traverse can be restarted from the middle of the tree without returning to the root.
This is because, in our performance measurement,
the original implementation of Masstree~\cite{masstree_beta} showed that tree traversal accounted for most of its performance.
%
The second optimization of {\sl Yakushima} is related to scan atomicity. Though Section 3 of the original paper~\cite{mao2012cache} describes that, the original Masstree does not provide atomicity for scan operations.
%
Therefore, concurrency control protocols with optimistic read protocols do not notice phantom occurrences until the validation phase, even if they occur at the time of the scan, which causes performance degradation.
%
In order to avoid this late detection, we designed an atomic scan operation in {\sl Yakushima}.
%

Besides, {\sl Yakushima} API provides {\it enter} and {\it leave} commands for memory protection.
%
Heap memory addresses that can be observed during {\it enter} and {\it leave} are not released.
%
Our transaction engine updates record contents in Copy-on-Write manner.
%
Therefore, the result of get operation no longer needs to be copied to the caller more than the address size,
and it is possible to prevent garbage collection during transaction processing execution.
%We are continuing to make api extensions and performance improvements to meet our needs.

\subsection{Design}
We prepared nine tables that are accessed by primary keys.
They are {\tt WAREHOUSE}, {\tt CUSTOMER}, {\tt NEW-ORDER}, {\tt DISTRICT},
{\tt ORDER}, {\tt ORDERLINE}, {\tt ITEM}, {\tt STOCK}, and {\tt HISTORY}.
%
{\tt HISTORY} table uses surrogate keys, and they are generated in a scalable manner.
%
We provide two bytes for worker thread ID, and increased counters for the {\sl Yakushima} key to avoid contentions.

We prepared secondary tables for {\tt CUSTOMER} and {\tt ORDER}.
%
As for the customer secondary table,
the key consists of warehouse id, district id, and c\_last,
and the value consists of c\_first and the list of primary keys.
%
As for the order secondary table,
the key consists of warehouse id, district id, customer id, and order id, and the value is the primary key for the {\tt ORDER} table.

\subsection{Phantoms}
\label{sec:Phantoms}
In TPC-C full-mix workload, the phantom problem can occur in the following cases.
\begin{itemize}
 \item {\tt ORDER} secondary table. Scan operation in the {\tt Order-Status} transaction and insert operation in the {\tt New-Order} transaction can occur concurrently.

 \item {\tt NEW-ORDER} table. Scan operation in the {\tt Delivery} transaction and insert operation in the {\tt New-Order} transaction can occur concurrently.
\end{itemize}

On the other hand, the phantom problem does not occur in the following cases.
\begin{itemize}

 \item {\tt ORDERLINE} table in the {\tt Stock-Level} transaction. 
   
       The {\tt New-Order} transaction inserts new records into {\tt ORDERLINE} table and the {\tt Stock-Level} transaction scans {\tt ORDERLINE} table.
       %
       %However, the scanning region by the {\tt Stock-Level} transaction is different from the region modified by the {\tt New-Order} transaction. 
       However, the range of keys scanned by the {\tt Stock-Level} transaction is different from the keys inserted by the {\tt New-Order} transaction.
       %
       The {\tt New-Order} transaction increments {\sf d\_next\_id} and a record with the key is inserted into {\tt ORDERLINE} table, while the {\tt Stock-Level} transaction scans keys with less than the {\sf d\_next\_id} from {\tt ORDERLINE} table. 
       %
       The key of {\tt ORDERLINE} table consists of warehouse id, district id, order id, and orderline id.

 \item {\tt ORDERLINE} table in the {\tt Order-Status} transaction. 
       
       The {\tt New-Order} transaction inserts new records into {\tt ORDERLINE} table, and the {\tt Order-Status} transaction scans the table. 
       %
       However, the {\tt Order-Status} transaction scans records inserted by past {\tt New-Order} transactions, not by concurrently running ones. 
       
 \item {\tt ORDERLINE} table in the {\tt Delivery} transaction. 
       
       %{\tt Delivery} transaction reads the oldest records that are not yet delivered by scanning the table. 
       The {\tt Delivery} transaction processes the oldest record that are not yet delivered. Therefore, the scan for the {\tt ORDERLINE} table is executed over the past records.
       %
       %The scan operation is executed over past records. 
       %
       The {\tt New-Order} transaction inserts new records, and thus these scan operation and insert operation does not conflict.
       
 \item {\tt CUSTOMER} secondary table in the {\tt Payment} transaction. 
       
       The transaction does not have insertion.
       
 \item {\tt CUSTOMER} secondary table in the {\tt Order-Status} transaction.

       The transaction does not have insertion.
\end{itemize}

\subsection{Evaluation}
We implemented TPC-C full-mix dealing with phantom problems following the scheme described in Section \ref{sec:Phantoms}.
%
The throughput and abort ratio varying thread count are shown in Figures
 \ref{fig:Varying thread count, throughput, fullmix.} and 
 \ref{fig:Varying thread count, abort ratio, fullmix.}, respectively.
%
We evaluated them varying the warehouse count. 
The warehouse counts are 1, 7, 28, 56, 84, 112, 140, 168, 196, 224, and the thread count. 
%
The same colors in the Figures correspond to the same warehouse count setting.
%
As illustrated in the Figures, the throughput increase as thread count increases if the warehouse count is enough.
%
The performance curve deteriorates when the thread count is larger than 112.
This is because our environment has only 112 physical cores among 224 logical cores.
%
As illustrated in Figure
 \ref{fig:Varying thread count, abort ratio, fullmix.}, 
the abort ratio increases if the warehouse count is not enough.
%
This is because the warehouse count associates with contention ratios.
\begin{figure}[t]
 \centering
 %
 \includegraphics[scale=0.6]{fig/tpcc/fm-tp.pdf}
 \caption{Varying thread count, throughput, fullmix.}
 \label{fig:Varying thread count, throughput, fullmix.}
\end{figure}
%
\begin{figure}[t]
 \centering
 \includegraphics[scale=0.6]{fig/tpcc/fm-abort.pdf}
 \caption{Varying thread count, abort ratio, fullmix.}
 \label{fig:Varying thread count, abort ratio, fullmix.}
\end{figure}
%

%%%%%%%%%%%%%%%%%%%%%%%%

As illustrated in Figure
\ref{fig:Varying warehouse count, fullmix with 224 threads.},
throughput deteriorates as the warehouse count increases when the number of worker threads is fixed to 224.
%
This is because of increasing abort ratios occurred by contentions.
\begin{figure}[t] 
 \centering
 %
 \includegraphics[scale=0.6]{fig/tpcc/fm-wh.pdf}
 \caption{Varying warehouse count, fullmix with 224 threads.}
 \label{fig:Varying warehouse count, fullmix with 224 threads.}
\end{figure}

 \subsection{Summary of TPC-C}
 TPC-C is an important and realistic benchmark that include phantom occurrences by concurrent scan and insert operations.
 %
 CCBench currently supports the TPC-C benchmark with
 the {\sl Yakushima} concurrent index.
 %
 Only the Silo protocol is supported currently.
 %
 This Appendix validates the correctness of its implementation by comparing CCBench with DBx1000~\cite{dbx1000} and \seqsplit{DBx1000(C)}~\cite{dbx1000_cicada_git} for TPC-C NP, and scalability for TPC-C full-mix.
 % Justification.
 The results of the experiments demonstrate that the implementation of CCBench was appropriate.
 %
 In addition, different analysis platforms exhibited different behaviors even for the same workload, depending on the design and the implementation of the systems. 
 % insight 5
 We claim Insight 5 again; it is difficult to find deep knowledge using multiple reference implementations or platforms. We believe that CCBench will help such analysis and related research in the many-core architecture era.

 %
 % Future work 
 %
 An evaluation of the TPC-C full-mix for protocols other than Silo remains as future work.
%
 Furthermore, we plan to implement the phantom avoidance for them soon. 
 %
 For TicToc, Cicada, MOCC, and 2PL-NoWait, we can use the technique presented in this Appendix.
 %
 For 2PL-Wait, we can use next-key locking with Masstree, and we will implement it to {\sl Yakushima}.
 %
 For SI, no extension is necessary for the phantom avoidance since each transaction under SI reads a fixed snapshot and the phantom problem does not occur.


==> src/resp-M1.tex <==
% R3-D2
Thanks for your comment.
To justify the implementations in CCBench, we used a standard benchmark system DBx1000.
%
DBx1000 supports DL\_DETECT, NO\_WAIT, HEKATON, SILO, TICTOC, and we evaluated SILO and TICTOC.
The results are shown in Fig. \ref{fig:tuple10m_val1k_ycsbC_tps} and \ref{fig:tuple10m_val1k_ycsb_medium_tps}.
The results show that CCBench and that of DBx1000 showed similar trends, and
Silo-DBx1000 and TicToc-DBx1000 outperformed those of CCBench.
We consider the reason is the difference in access methods (hash index for DBx1000 and Masstree for CCBench because DBx1000 does not support concurrent index).
It also should be noted that CCBench without index was around 30\% better than DBx1000 (with hash index) at 80 threads in the setting of Fig. \ref{fig:tuple10m_val1k_ycsbC_tps}.
%
Thus we consider the implementations of Silo and TicToc in CCBench are at least as optimized as the original implementations for these workloads.
%

However, we do not know the performance of DBx1000 for RMW workloads because DBx1000 does not support the operations.
Thus, we could not conduct experiments related to Fig. \ref{fig:Reproduction of Cicada experiment. 10M records, payload 100 bytes} since all the results in this Figure required RMW operation.


==> src/resp-M2.tex <==
Thanks for your comment.
TPC-C is a popular and standard benchmark and often used to evaluate the scalability of OLTP systems.
The scalabilities have been well explored, while this paper analyzes different parameter spaces beyond the scalability as shown in Table \ref{tab:Experimental Parameters}.
We conducted all the experiments setting the thread size to 224.
%
Then, unfortunately TPC-C benchmark does not useful for our purpose.
We gained six insights in our analysis with our workload parameter sets.
However, we think it is difficult to gain another insight using TPC-C because the scalability has been well studied and it is simpler than our parameter sets.

%
We described the reason why we do not use TPC-C benchmark in $\S$ \ref{Configurable Workloads} in the manuscript.


==> src/resp-M3.tex <==
Thanks for your comment.
We fully and carefully revised this manuscript, and we also used a proofreading service to improve the quality and readability of this paper.
The revised places are colored in
\color{blue}
blue.
\color{black}


==> src/resp-M4.tex <==
Thanks for your comment.
We revised the related work in $\S$ \ref{sec:Related Work}.
We first summarize conventional studies and then describe the differences between this paper and them.


==> src/resp-M5.tex <==
Thanks for your comment.
To explain how to extend CCBench, we first prepare a guide for the extension~\cite{cc_format}.
We then asked a member of our laboratory to implement a simple OCC protocol in CCBench following the guide.
He easily implemented it~\cite{occ_nemoto} and published the experience for CCBench users~\cite{nemotoccbench}.
%
We described the above contents at the final paragraph of $\S$ \ref{sec:A Platform for Fair Comparison} in the manuscript.


==> src/resp-R1-D3.tex <==
 Thanks for your suggestion.
 %
 It is interesting to find out certain optimizations that perform efficiently for real applications.
 We think it is also interesting to clarify the facets of optimization methods in detail.
 Since there are no silver bullets, each method should have pros and cons.
 The motivation of this paper is to find out such characteristics with unprecedented workload settings.
 %
 Thus, we prefer settings that a method demonstrates both good and bad results to understand the characteristics well.
 %
 However, as you point out, real applications are also impressive, so we will study such workloads in future work.
 Thank you for your great suggestion!


==> src/resp-R3-D1.tex <==
Thank you for your comment.
We fully rewrote this paper so that readers can understand its contributions.
%
We summarized our findings as six insights.
We describe
insight 1 in $\S$~\ref{sec:Cache Miss Mitigation},
insight 2 in $\S$~\ref{sec:Effect of Invisible Read},
insight 3 in $\S$~\ref{sec:Confirmation of Effect of NoWait},
insight 4 in $\S$~\ref{sec:Effect of Extra Read and Read Phase Extension Method},
insight 5 in $\S$~\ref{sec:problem-many-visible-versions} and
insight 6 in $\S$~\ref{sec:discussion-towards-version-lifetime-control}.
%
We mention them in
$\S$ \ref{sec:Contribution} and $\S$ \ref{sec:Conclusion}.


==> src/resp-R3-D6.tex <==
 Thanks for your comment.
 It is interesting to find out certain optimizations that perform efficiently or inefficiently in a variety of settings like centralized data objects.
 It is also interesting to clarify the facets of optimization methods.
 Since there are no silver bullets, each method should have pros and cons.
 The purpose of this paper is to find out such characteristics with unprecedented workload settings.
 %
 Thus, we prefer settings that a method demonstrates both good and bad results to understand the characteristics well.
%
 In this paper, {\sf NoWait} performs well for short transactions while it does not for long transactions as in Fig. \ref{fig:ycsbB_tuple100m_skew08_ope10-100_tps},
 Silo, TicToc, MOCC outperforms Cicada as shown in Fig. \ref{fig:comp_tuple100m_skew0-099} for certain situations, and Silo outperforms TicToc as shown in Fig. \ref{fig:ycsb_rratio10-90_tps} for certain situations.
 These results are not reported in original papers, and it shows that the exploration of concurrency control protocols is still midway.


==> src/tmp/cache-proof.tex <==
\section{Analysis of Cache}
\label{sec:Cache Effect}

In this section, we discuss the following two effects of cache.
{\bf Cache-line conflict} happens when many worker threads access the same cache-line with some writes (e.g., accessing a single shared counter).
%
Then, the cache-line is occupied by a single thread and the other threads are internally blocked.
%
{\bf Cache-line replacement} happens when transactions access a large amount of data (e.g., high cardinality, low skew or large payload).
Then, data accesses incline to replace the contents of L1/L2/L3 cache.
\subsection{Cache-Line Conflict}
\label{sec:changing_database_size}
\input{src/cache_figure.tex}

%
Some protocols adopt centralized ordering (e.g., shared counter)~\cite{jung2013performance,kim2016ermia} while some others do decentralized ordering~\cite{tu2013speedy,yu2016tictoc,wang2016mostly,lim2017cicada}.
We first analyze the negative effect of the centralized ordering.
%
The results are shown in Figs.~\ref{fig:ycsbB_tuple1k-1g}, \ref{fig:ycsbC_tuple1k-1g}, \ref{fig:ycsbB_tuple1k-1g_ar}, and \ref{fig:ycsbC_tuple1k-1g_ca}.
The details of the workload are described in the graph caption. 
% omit?
Since the result of YCSB-A have the same trend as those of YCSB-B, it is omitted.
%YCSB-C is a read-only workload, so the abort rate is 0, and the corresponding result about abort rate is omitted.
%
Fig.~\ref{fig:central_tuple1k-1g} illustrates that the throughput of ERMIA and SI do not scale although their scheduling spaces are wider than that of SVCC serializable protocols.
This is because both protocols depend on a central data object
 %(i.e., a shared counter for the timestamp of both protocols and transaction mapping table of ERMIA), and access to the central data structure
that causes the cache-line conflict, which in turn causes performance degradation.
%This is consistent with the claims in ~\cite{tu2013speedy, wang2016mostly}.
%\cite{tu2013speedy} describes in Section 5.2 that MemSilo + GlobalTID does not scale because it issues a commit tid with a single shared counter.
%\cite{wang2016mostly} states in Section 5.3 that on large machines such as GryphonHawk, ERMIA 's centralized data structure for inter-thread communications used by SSN becomes a major bottleneck.
%\cite{wang2016mostly} also states that interthread communication impedes scalability in Section 2.2.

%
To investigate the degree of the inefficiency, we measured the throughput of {\tt fetch\_add}.
The results are shown in Figs.~\ref{fig:fetch_add_test_tps} and \ref{fig:fetch_add_test_cm}. 
The cache miss rate is measured using the Linux Perf tool, and it is about L3.
Fig.~\ref{fig:fetch_add_test_tps} shows that one thread exhibits the best performance.
This is because frequent reads/writes to the same memory address by multiple threads cause high conflicts of a cache-line.
Fig.~\ref{fig:fetch_add_test_cm} illustrates that the L3 cache miss that rate increases as the number of threads increases.
%
Cache-line conflicts incur L3 cache misses and longer communication delay if the CPU core requiring the cache-line and the another core having it exclusively are running in the different CPU sockets. In the experiment, 28 threads setting used one socket, 56 threads setting used two sockets, 112 or more threads setting used four sockets.
%
Thus, larger L3 cache miss rate ($\geq$ 30\%) indicates occurrence of communication among sockets and it significantly deteriorates the performance of fetch\_add.
%
Consequently, centralized objects should be avoided by the above reason.

\subsection{Cache-Line Replacement}
\label{sec:Cache Miss Mitigation}
In this Section, we first discuss YCSB-B result.
In Figs.~\ref{fig:ycsbB_tuple1k-1g} and \ref{fig:ycsbB_tuple1k-1g_ar}, as cardinality increases,
(1) throughput first improves and then deteriorates, and
(2) abort rate monotonically improves.
%
When cardinality is quite low, the footprint of accessible records are also small so that all of records fit inside L3 cache.
However, it is more likely happen contentions at L1 or L2 cache.
As cardinality increases, such contentions are alleviated since accessible records increase, and performance improves.
%
It is considered that with more cardinality, the total amount of records start to overflow L3 cache.
It attracts L3 cache misses and consecutive accesses of remote socket cache or DRAM, which degrades performance.
%
%The effect of L3 cache miss is stronger than that of L1/L2 cache misses.

% YCSB-C result, cache > contention..
\input{src/read_only_cache_effect.tex}

\if 0
Here we have a hypothesis.
If the performance of a protocol is strongly affected by cache memory utilization, the location of the data to be accessed is either inside (cache-inside) or outside the cache (cache-outside).
The data location is considered to depend greatly on the cardinality.
If the cardinality is small, the data tends to be within the cache, while in the opposite case, the data is less likely to be within the cache.

This situations are evident from ~\ref{fig:ycsbC_tuple1k-1g} and~\ref{fig:ycsbC_tuple1k-1g_ca}.
If the protocol does not update shared meta data, 
the increase in cardinality degrades the throughput and increases the cache miss rate due to using large memory.
Surprisingly, 2PL, SI, and ERMIA which update shared meta data in the read only workload do not show this trend.
2PL uses reader/writer locks and operating read lock updates the shared status of the data.
SI uses centralized counter to define start and end points.
ERMIA uses transaction mapping table.
In these protocols, as it transits from small records to large records, the throughput first improves and then deteriorates, the cache miss rate first improves and then deteriorates.
The reason is considered as follows.
First, even in YCSB-C (read only), when cardinality is quite low, access items are limited, which more likely provides cache contentions.
Second, as cardinality increases, such contentions are alleviated since access items increase.
However, when cardinality increases to some extent, some records are not fit into cache, and the cache evictions incur performance degradation.

Therefore, the above hypothesis holds.
With the cache-inside workload type, more records provide better performance than cache-outside workloads.
\fi

% Invisible read
\input{src/invisible}


==> src/tmp/old_cc_info.tex <==
   \if 0
   Silo~\cite{tu2013speedy} uses all the five transactions on the Silo system~\cite{silo_git}.
 TicToc~\cite{yu2016tictoc} uses only the NewOrder and Payment transactions on the DBx1000 system~\cite{dbx1000}.
 FOEDUS~\cite{kimura2015foedus} uses all the five transactions on the FOEDUS system~\cite{foedus_git}.
 MOCC~\cite{wang2016mostly} uses all the five transactions on the FOEDUS system~\cite{foedus_git}.
 Cicada~\cite{lim2017cicada} uses all the five transactions extending the DBx1000 system~\cite{dbx1000}.
 Latch-free SSN~\cite{wang2017efficiently} uses all the five transactions on the ERMIA system~\cite{ermia_git}.
 STOv2~\cite{STOv2} uses all the five transactions on the STO system~\cite{sto_git}.
 ACC~\cite{DBLP:conf/cidr/TangJE17} uses all the five transactions using the ACC system based on the Doppel system~\cite{Doppel}.
 AOCC~\cite{AOCC_Guo} uses only the the NewOrder, Payment, and the original Reward transactions on the DBx1000 system~\cite{dbx1000}.
 Transaction batching and reordering~\cite{tx_batch} does not use any TPC-C transactions on Cicada system~\cite{cicada_git}.
 %Transaction chopping
 IC3~\cite{IC3} uses all the five transactions extending the Silo system~\cite{silo_git}.
 %
 %
 % Analysis paper
 %
 %
 Abyss paper~\cite{yu2014staring} uses only the NewOrder and Payment transactions on the DBx1000 system~\cite{dbx1000}.
 MVCC evaluation paper~\cite{wu2017empirical} uses all the five transactions extending the Peloton system~\cite{peloton}.
 Trireme paper~\cite{trireme} does not use any TPC-C transactions on Trireme system which is not open source.
 %
 \fi


==> src/tmp/related.tex <==
\input{src/related_core.tex}



==> src/tmp/related_core.tex <==
{\sf

Yu et al.~\cite{yu2014staring} evaluated concurrency control protocols with one thousand cores.
The protocols are three 2PLs and four T/Os.
As for the benchmarks, YCSB and TPC-C are used.
Throughputs and the breakdown of execution time are shown.
Five recent protocols evaluated in this paper~\cite{tu2013speedy}~\cite{kim2016ermia}~\cite{wang2016mostly}~\cite{yu2016tictoc}~\cite{lim2017cicada} were not included.
Wu et al.~\cite{wu2017empirical} empirically evaluated MVCC protocols.
They discussed the theory and techniques superior in some workload situations.
They focused on MVCC and did not evaluate SVCC protocols proposed recently~\cite{wang2016mostly}~\cite{tu2013speedy}~\cite{yu2016tictoc}~\cite{lim2017cicada}
Harding et al.~\cite{10.14778/3055540.3055548} evaluated distributed concurrency control protocols.
No distributed protocols are evaluated in this paper.

Platforms to evaluate transaction processing are important and have been studied.
It includes Trireme~\cite{trireme}, Shore-MT~\cite{10.1145/1516360.1516365}, DBx1000~\cite{dbx1000} and Peloton~\cite{peloton}.
The evaluations of these studies provide users mainly a way to investigate the scalability of protocols, which is significant today for increasing CPU cores.
On the other hand, none of them does not care varying workload parameters at a highly parallel environment.
This paper fixes the number of worker thread to 224, and provides analysis with varying other parameters: skew, payload size, transaction size, and cardinality.
%
Besides, this paper enables to apply optimization techniques to all the protocols even though it has not been applied in the original paper.
%
}


==> src/tmp/repro-proofread.tex <==
\subsection{Reproduction of Prior Work}
	
When evaluating concurrency control protocols, the performance of protocols should be compared under fair conditions.
The meaning of fairness may vary depending on contexts, and we think the following two conditions should be satisfied for a fair comparison.

{\bf Fairness Condition 1.}
Basic modules should be shared: The base modules of an evaluation platform should be shared.
Access methods (e.g., Masstree) and local datasets (read and write sets) need to be shared among protocols.
The effects of memory allocator should be eliminated as much as possible.
The workload should be generated in the same way.
This is important because the performance of a protocol depends on not only the design principle but also engineering details.
The performance of modern protocols is deeply related to the exploitation of underlying hardware, and thus they are sensitive to engineering details.

This above fairness condition may not clearly be satisfied in some cases.
In some papers, we see comparison protocols are not implemented by the authors.
Section 4.2 in Cicada paper [16] states, ”Cicada and existing schemes in DBx1000 share the benchmark code, but have separate data storage and transaction processing engines.”. 
n MOCC paper [27], pure OCC, MOCC, PCC (2PL variants) implementation uses FOEDUS, Dreadlock/WaitDie/BlindDie (2PL variants) uses Orthrus and ERMIA implementation uses ERMIA system.
Three benchmark systems are mixed, In ERMIA paper [14], Silo implementation uses the Silo system while the SI/SSI use the ERMIA system, and the two benchmark systems are mixed.
In these cases, a huge amount of effort by experts is required to avoid unfair comparison.
Such activity is hard for non-experts. Then, we say our fairness condition 1 is not satisfied with their cases.

Wu et al. [29] use the same platform for comparing multiple multi-version protocols, which satisfies the fairness condition 1.
Design philosophy on the platform of CCBench is similar to them.
Their work focuses on evaluating multi-version protocols, and some modern protocols (Cicada, ERMIA, Silo, TicToc, MOCC) are out of scope there.
Yu et al. [30] developed an evaluation platform DBx1000 using a CPU simulator to clarify the scalability impediments of the protocols.
DBx1000 can simulate environments with up to 1024 cores.
Of the seven protocols they targeted, our targets share 2PL, Silo, and TicToc.
On the viewpoint of fairness condition 1, our philosophy is relevant to that of them.

{\bf Fairness Condition 2.}
Applicable optimization techniques should be applied: A protocol consists of a basic method and optimization technique(s).
Sometimes, an optimization technique can be integrated into other basic methods even if a protocol P does not include the optimization technique O at the time of proposal, O can be applied P.
For example, RapidGC is proposed by Cicada [16], and it can be applied to both SI and ERMIA.
NoWait in the validation phase of OCC is proposed by TicToc [31], and it can be applied to Silo.

We think each protocol should be compared with others in the best condition from the viewpoint of fair evaluation.
As described above, the performance of a protocol highly depends on engineering details, and thus applying optimization techniques can improve performance.
One may think such additional optimizations are only laborious and rarely improve performance.
One may have an objection.
By applying an optimization technique to non-original basic methods, the protocol is different from the original one.
However, the application of optimization techniques often improves performance, and we think each protocol should take its best
form in this paper.

Our fairness condition 2 is not satisfied sometimes.
TicToc [31] does not apply NoWait to Silo.
Cicada [16] does not apply RapidGC to ERMIA(SI + SSN) and Hekaton.
Cicada also does not apply adaptive backoff to all protocols used by evaluations in the original paper.

3.2
A Platform for Fair Comparison

We developed CCBench, an evaluation platform for in-memory concurrency control protocols that satisfies the above fairness conditions.
CCBench is publicly available on GitHub [1].
The architecture of CCBench is illustrated in Fig. 1.
To satisfy fairness condition 1, all worker threads in CCBench run in a single node, and it shares the same address space.
Clients and a server run in the same process.
CCBench standardizes the workload generation method.
Client operations (read/write) are generated online.
The generation task is combined with worker threads.
For each transaction execution, workload generation based on the workload setting given before the experiment is performed.
The generated workload information is stored in the STL container, and its memory space reused throughout the experiment.
Allocated memories for a local data structure (read/write set) will be reused for the next transaction, so this improves performance by avoiding memory manager overhead.
We placed record data and concurrency control metadata on the same cache-line.

To fairly provide access methods for protocols in CCBench, all protocols use Masstree [17].
We implemented wrappers for the original implementation [3].
CCBench uses mimalloc [4] for a memory allocator.
We conducted memory allocation evenly in all sockets by using the Linux numactl command for stable results in experiments.
CCBench supports the Yahoo! Cloud Serving Benchmark (YCSB) [9] with flexible configurations on six parameters shown in Table 1.
CCBench currently focuses on read and write operations only, and insert and delete operations are out of scope, which is left as future work.
To determine the skew, CCBench uses a fast approximation method [10].

To satisfy fairness condition 2, CCBench provides seven optimization techniques, as shown in Table 2.
(1) Distributed counter: mitigating simultaneous accesses to a shared single counter.
(2) Invisible read: a read operation that does not pollute the cache memory.
(3) Version inlining: allocating space to keep versions in the record header.
(4) NoWait: immediate abort when detecting a conflict.
(5) Extra Read: retry of the read operation in optimistic protocols.
(6) Adaptive backoff: artificial delay before restarting an aborted transaction.
(7) RapidGC: frequently updating timestamp watermark for garbage collection in multi-version protocols.
CCBench enables additional optimization techniques to 2PL, Silo, TicToc, SI, ERMIA, and Cicada.

It should be noted that CCBench does not support read-only optimization techniques introduced in Silo, FOEDUS, MOCC, and ERMIA.
This is because this optimization improves performance in a specific case (i.e., 99\% read-only transactions, 1\% write transactions, skew at 0.99), and such a workload does not appear in this paper

3.3 Implementing Optimization Techniques
2PL: For efficiency, we implemented the reader/writer lock system used in the protocol from scratch.
Silo: We padded the global epoch (64 bits) into the cache line size (64 bytes) to reduce cache pollution that can be caused by the global epoch state change.
The calculation of commit tid is computationally expensive since it requires loops for both the read set and the write set.
We reduced these two loops by calculation at write lock acquisition and read verification, which leads efficiency.

ERMIA: We adopted the latch-free SSN to avoid expensive SSN serial validation.
This implementation avoided the validation from being a critical section.
We implemented the leveraging existing infrastructure that integrates pstamp and sstamp to reduce memory usage.
We optimized the transaction mapping table.
In a straightforward way, the mapping table is designed as a two-dimensional global array with a thread number, TID, cstamp, and last cstamp, which requires a lock manager for updates and read over the rows.
This clearly causes performance degradation due to serialization and cache pollution.
Therefore, we design a data structure that expresses the rows in a one-dimensional array so that it can be latched with a single atomic compare-and-swap (CAS) operation, and performance was improved by avoiding serialization and cache pollution for row element access.
In our ERMIA implementation, we adopted rapid garbage collection (RapidGC) in Cicada.
CASed transaction mapping table objects and version objects are garbage collected based on calculating a threshold that is not accessed by other workers.
The transaction mapping table object exploits our aggressive version reuse described later in this section, and the load on the memory manager is almost eliminated.

TicToc: We implemented all the three optimization methods (no-wait locking in the validation phase, preemptive aborts, timestamp history).
We also improved the algorithm 5 in the original paper by removing redundant read timestamp updates.
It should be noted that if the recorded read timestamp and updating value is the same, there is no need to perform it.

MOCC: In the original paper, MOCC periodically resets temperature information.
This approach changes many cache lines to the invalid state simultaneously, and performance deteriorates.
We instead perform temperature management only for the record that caused read validation failure.
When resetting the temperature, the epoch at that time is added to the temperature information.
At the time of temperature control, the epoch at that time is compared with the epoch attached to the temperature information.
If the epoch is different, we reset the temperature information.
Therefore, the performance was improved by reducing the cache pollution cost and the resetting cost while finely controlling the temperature.
We did not implement MQL lock since our environment has only 4 NUMA nodes, and its novel effect would be limited.
We instead used the reader/writer lock that is also used by 2PL implementation.

Cicada: We implemented all the six optimization techniques (sort write set by contention, pre-check version consistency, adaptive backoff, early aborts, rapid garbage collection, and best-effort inlining).
In addition, we fixed a logical bug, which is the incomplete version consistency check in the validation phase.
The original paper only confirms that the read version is still the visible version.
However, it needs to check if it is the latest visible version too.
If a newer version exists in the observation range, it means that it should have been read and the transaction view will be broken.

As for the one-sided synchronization, we turned off it to provide higher efficiency.
Aggressive Version Reuse for MVCC: In multi-version protocols (SI, ERMIA, and Cicada), some operations such as creating new versions and deleting old versions provide a load on the memory manager, which also true for memory managers with thread-local memory pools.
So, we worked on a new optimization method, aggressive version reuse that avoids overloading the memory manager in multi-version protocols.
By using the aggressive version reuse, each worker thread maintains a container for future version reuse.
When garbage collection occurs, collected versions are stored in this container.
When a new version is requested, it is taken from this container if this container is not empty.
Otherwise, it requests a memory space to the memory manager as usual.
As an optimization in our experiment, our system expects the necessary memory space for the first garbage collection in advance, and it allocates
them in advance. By this optimization, our multi-version protocols put almost no burden on the memory manager.

3.4 Reproduction of Prior Work
Before introducing the result of the evaluation, we need to validate the correctness of CCBench implementation.
We demonstrate that CCBench successfully reproduces the experimental result in some of the prior work.

3.4.1 MOCC
The first reproduction is MOCC [27].
The MOCC we implemented has two differences, as described in Section 3.3.
In order to confirm the graph shown in the original paper can be reproduced by our implementation, we conduct an experiment with the settings shown in Figs 6 and 7 of the original paper.
The settings are also described in the graph caption.
The experimental results are shown in Fig. 2a that the performance scales with the number of threads in the read-only workload.
It reproduces the result of Fig. 6 in the original paper.
The reason is that there is no interaction between threads.
The reason why the performance improvement rate deteriorates after 112 threads is that there
are only 112 physical cores, and the reason that the MOCC performance is slightly lower than Silo is that there is a new calculation process.
On reading, MOCC calculates the temperature information address.
Also, it performs a process for determining whether the temperature is high, which requires memory access.
This process that not exist in Silo, and it may differentiate their results.
The results shown in Figs. 2b and 2c show that when the write rate increases from 0\% to 10\%, the abort rate rapidly increases, and the performance deteriorates.
This experiment is the reproduction of Fig. 7 in the original paper.
The reason is that write operation produces a large amount of the read validation failures.
In Figure 2b, the performance of Silo deteriorates at a write rate of 0-40\%, but the performance improves at a write rate of 40-60\%.
This is a trade-off between reduced read/write contentions due to reduced write operations and frequent read validation failures due to increased read operations.
Compared to that, MOCC shows stable performance, which is considered to progress steadily by temperature control.

3.4.2 TicToc
The second reproduction is TicToc [31].
To confirm our implementation can reproduce the graph shown in the original paper, we experiment with the settings shown in Figs 6, 7, and 8 of the original paper.
The details of the workload are also described in the graph caption.
We set epoch interval long so that it does not to occur cache line contentions in Silo.

Figure 3a shows that Silo and TicToc show comparable performance in read-only workloads, exceeding 20 M tps, which is consistent with Fig. 6 in the original paper.
In Figure 3b, Silo and TicToc both scale in performance.
This is also consistent with Fig. 7 in the original paper.
On the other hand, we found an impressive result.
In Fig. 3c, TicToc shows different performances from Fig. 8 in the original paper.
The performance of TicToc improves as the number of threads increases, but when the number of threads exceeds a specific number, the performance starts
to deteriorate due to an increase in read/write contention.
Therefore, in the original paper, we considered the possibility of a sort of optimization on TicToc and tried to introduce Cicada backoff optimization.
This is shown as TicToc + BO in Fig. 3c.
In our environment, TicToc + BO showed a similar performance curve of TicToc to that of Fig. 9 in the original paper.
The third reproduction is Cicada [16].
The workload was set almost the same as the original paper.
The details of the workload also are described in the graph caption.
The differences from the original paper and here are as follows: 
(1) Redesign and reimplementation of all protocols by authors.
(2) The backoff optimization that Cicada has is installed in all protocols because this optimization technique can be implemented without using Cicada, and we found it is effective for improving performance.

Figures 4a, 4c, 4b, and 4d illustrate the experimental results.
All the results showed the same tendency as the original paper (Figs 6 and 7).
As a result of applying the backoff optimization techniques fairly to all protocols, MOCC or TicToc won over almost all the given parameters,
which is inconsistent with the original paper.
Evaluation on the original paper compared different systems.
Therefore, it is considered that different designs and implementations between the systems affected the performance in the evaluation of the original paper.


==> src/unknown.tex <==
\section{New Performance Factor}
\input{src/delay}
\input{src/version-lifetime-control}


==> tmp/header.tex <==
\usepackage{graphicx}
\usepackage{balance}  % for  \balance command ON LAST PAGE  (only there!)
\usepackage{caption}
\usepackage{subcaption}
\usepackage{ascmac}

% It should be used on writing.
\usepackage{color}

% It is required to use \url in bibliography for arXiv.
\usepackage{url}

% Include information below and uncomment for camera ready
\vldbTitle{An Analysis of Concurrency Control Protocols for In-Memory Database with CCBench.}
%\title{An Analysis of Concurrency Control Protocols for In-Memory Database with CCBench.}
\vldbAuthors{Takayuki Tanabe, Takashi Hoshino, Hideyuki Kawashima, Osamu Tatebe.}
%\author{Takayuki Tanabe, Takashi Hoshino, Hideyuki Kawashima, Osamu Tatebe.}
\vldbDOI{https://doi.org/10.14778/xxxxxxx.xxxxxxx}
\vldbVolume{13}
\vldbNumber{46}
\vldbYear{2020}

\begin{document}
% ****************** TITLE ****************************************

\title{An Analysis of Concurrency Control Protocols\\ for In-Memory Database with CCBench}

% possible, but not really needed or used for PVLDB:
%\subtitle{[Extended Abstract]
%\titlenote{A full version of this paper is available as\textit{Author's Guide to Preparing ACM SIG Proceedings Using \LaTeX$2_\epsilon$\ and BibTeX} at \texttt{www.acm.org/eaddress.htm}}}

% ****************** AUTHORS **************************************

% You need the command \numberofauthors to handle the 'placement
% and alignment' of the authors beneath the title.
%
% For aesthetic reasons, we recommend 'three authors at a time'
% i.e. three 'name/affiliation blocks' be placed beneath the title.
%
% NOTE: You are NOT restricted in how many 'rows' of
% "name/affiliations" may appear. We just ask that you restrict
% the number of 'columns' to three.
%
% Because of the available 'opening page real-estate'
% we ask you to refrain from putting more than six authors
% (two rows with three columns) beneath the article title.
% More than six makes the first-page appear very cluttered indeed.
%
% Use the \alignauthor commands to handle the names
% and affiliations for an 'aesthetic maximum' of six authors.
% Add names, affiliations, addresses for
% the seventh etc. author(s) as the argument for the
% \additionalauthors command.
% These 'additional authors' will be output/set for you
% without further effort on your part as the last section in
% the body of your article BEFORE References or any Appendices.

\numberofauthors{4} %  in this sample file, there are a *total*
% of EIGHT authors. SIX appear on the 'first-page' (for formatting
% reasons) and the remaining two appear in the \additionalauthors section.

\author{
% You can go ahead and credit any number of authors here,
% e.g. one 'row of three' or two rows (consisting of one row of three
% and a second row of one, two or three).
%
% The command \alignauthor (no curly braces needed) should
% precede each author name, affiliation/snail-mail address and
% e-mail address. Additionally, tag each line of
% affiliation/address with \affaddr, and tag the
% e-mail address with \email.
%
% 1st. author
\alignauthor
Takayuki Tanabe\titlenote{Work done while at University of Tsukuba}\\
       \affaddr{NAUTILUS Technologies, Inc}\\
       \email{tanabe@nautilus-technologies.com}
% 2nd. author
\alignauthor
Takashi Hoshino\\
       \affaddr{Cybozu Labs}\\
       \email{hoshino@labs.cybozu.co.jp}
% 3rd. author
\alignauthor
Hideyuki Kawashima\\
       \affaddr{Keio University}\\
       \email{river@sfc.keio.ac.jp}
\and  % use '\and' if you need 'another row' of author names
% 4th. author
\alignauthor
Osamu Tatebe\\
       \affaddr{University of Tsukuba}\\
       \email{tatebe@cs.tsukuba.ac.jp}
}
% There's nothing stopping you putting the seventh, eighth, etc.
% author on the opening page (as the 'third row') but we ask,
% for aesthetic reasons that you place these 'additional authors'
% in the \additional authors block, viz.
%\additionalauthors{Additional authors: John Smith (The Th{\o}rv\"{a}ld Group, {\texttt{jsmith@affiliation.org}}), Julius P.~Kumquat
%(The \raggedright{Kumquat} Consortium, {\small \texttt{jpkumquat@consortium.net}}), and Ahmet Sacan (Drexel University, {\small \texttt{ahmetdevel@gmail.com}})}
%\date{1 March 2020}
% Just remember to make sure that the TOTAL number of authors
% is the number that will appear on the first page PLUS the
% number that will appear in the \additionalauthors section.


==> tmp/src/abst.tex <==
\begin{abstract}
 This paper proposes yet another concurrency control analysis platform CCBench.
 CCBench supports seven protocols (Silo, TicToc, MOCC, Cicada, SI, SI with latch-free SSN, 2PL) and seven versatile optimization methods and enables them to configure seven workload parameters.
 %(skew, cardinality, payload size, transaction size, read ratio, thread size, read-modify-write).
 %
 We analyze the protocols and optimization methods varying workload parameters setting the thread size to 224.
 %
Conventional studies focus on thread scalability, and none of them explore the space this paper analyzes.
%
We classify a variety of methods into three classes of performance factors: CPU cache, delay on conflict, and version lifetime.
Through the analyses with CCbench for 224 threads, we gain six insights.
(I1) The performance of optimistic protocols at read-only workload rapidly degrades as cardinality increases even without L3 cache misses.
(I2) Silo can outperform TicToc for write-intensive workloads by invisible read.
(I3) Extra read at optimistic protocols regulates contentions for certain situations, and we define read phase extension method.
(I4) The effectiveness of a waiting policy depends on situations.
(I5) To find deep knowledge of protocols, analysis must be done at the same platform.
(I6) Even state-of-the-art garbage collection cannot improve the performance of multi-version protocols if a single long transaction exists, and we define aggressive garbage collection method.
%
 The code for CCBench and all the data in this paper are available online at GitHub.
%
\end{abstract}


==> tmp/src/ack.tex <==
\section*{Acknowledgments}
We thank Masahiro Tanaka, Takuma Ojiro, Sho Nakazono, Jun Nemoto for thoughtful supports on drafts.
%
We are grateful to the anonymous reviewers for their valuable feedbacks.
%
%This work is partially supported by JST CREST JPMJCR1414, JSPS Kakenhi 19H04117, and Project commissioned by the New Energy and Industrial Technology Development Organization (NEDO).
%
This work is partially supported by JST CREST JPMJCR1414, JSPS Kakenhi 19H04117, and Project commissioned by the New Energy and Industrial Technology Development Organization (NEDO).
%We’re grateful toJun Nemoto, Masahiro Tanaka, Sho Nakazono, and Takuma Ojiro for thoughtful comments on drafts.
%
%Thanks also to anonymous reviewers of the work.
%

==> tmp/src/analyzed_space.tex <==
%\color{blue} %REVISED_COLOR_BEGIN
CCBench supports the seven parameters shown in Table~\ref{tab:Experimental Parameters}.
%
Skew is the access pattern, which follows Zipf distribution.
Cardinality is the number of records in the database.
The payload is the size of a record (key plus value).
Transaction size is the number of operations in a transaction.
Read ratio is the ratio of reads in a transaction.
Write model is whether read modify write or not.
Thread size is the number of worker threads (though it is fixed to 224 in this paper except for reproduction).
%
To determine the skew, CCBench uses a fast approximation method~\cite{gray1994quickly}.
%
We analyzed CC protocols by using 224 threads with CCBench.
Most of the benchmarks were YCSB, and some were its variants of YCSB.
The analyzed parameter sets are summarized in Table \ref{tab:Experimental Parameters}.
We varied the skew, cardinality, payload, transaction size, and read ratio and fixed the thread size at 224.
%
The caption in Table \ref{tab:Experimental Parameters} describes the variance in parameters using $\alpha \ldots \zeta$\footnote{More parameter spaces are explored, but they are omitted due to the page length. All the results are found at \cite{thawkccdata}}.
%\color{black} %REVISED_COLOR_END

\begin{table}[tb]
 \begin{center}
  %  \begin{scriptsize}
    \begin{small}
   \caption{Analyzed Parameter Sets in this paper.
   ($\alpha$) Cardinality (from $10^3$ to $10^9$ records);
   ($\beta$) Cardinality ($10^3$ or $10^6$ records);
   ($\gamma$) Read ratio (from 0\% to 100\%);
   ($\delta$) Transaction size (from 10 to 100);
   ($\epsilon$) Payload size (from 4 to 1000 bytes);
   ($\zeta$) Skew (from 0.6 to 0.99).
   }
 \label{tab:Experimental Parameters}
 \begin{tabular}[tb]{l|cccccc}
  & \multicolumn{2}{c}{Cache}& \multicolumn{2}{c}{Delay}& \multicolumn{1}{c}{Version}\\
  \hline
  Figure Number
  &
  \color{blue} 
      $\mathcal{F}$\ref{fig:central_tuple1k-1g}
      \color{black} 
  & $\mathcal{F}$\ref{fig:Analysis of Invisible Read: YCSB, 224 Threads, Payload 4 bytes, Skew 0, 10 ops/trans.}

  & $\mathcal{F}$\ref{fig:Impact of Transaction Size: YCSB-B, 100M Records, 224 Threads, Payload 4 bytes, Skew 0.8.}
  & $\mathcal{F}$\ref{fig:Effect of Delay provided by Extra Read: YCSB-A, 100M records, 224 threads, skew 0.9, 10 ops/trans.}
  & $\mathcal{F}$\ref{fig:comp_tuple100m_skew0-099}\\
  \hline
  Skew            &0   &0   &0.8   &0.9  &$\zeta$ \\
  Cardinality     &$\alpha$ &$\beta$ &$10^8$&$10^8$&$10^8$\\
  Payload (byte)  &4   &4   &4     &$\epsilon$  &4\\
  Xact size       &10  &10  &$\delta$   &10   &10\\
  Read ratio (\%) &0,5 &$\gamma$ &50,95 &50   &50,95\\ \hline
  Thread size      &\multicolumn{5}{l}{Always 224 except from reproduction}\\
  Read modify write&\multicolumn{5}{l}{Always off except from reproduction}\\
 \end{tabular}
     %     \end{scriptsize}
     \end{small}
 \end{center}
\end{table}

\if 0 % backup
\begin{table}[tb]
 \begin{center}
  \begin{scriptsize}
 \caption{Analyzed Parameter Sets.
   \$1: Cardinality: range from $10^3$ records to $10^9$ records.
   \$2: Cardinality: points $10^3$ records or $10^6$ records.
   \$3: Read ratio: range from 0\% to 100\%.
   \$4: Transaction size: range from 10 to 100.
   \$5: Payload size: range from 4 bytes to 1000 bytes.
   \$6: Skew: range from 0.6 to 0.99.
   }
 \label{tab:Experimental Parameters}

 \begin{tabular}[tb]{l|cccccc}
  Parameter
  & Fig. \ref{fig:central_tuple1k-1g}
  & Fig. \ref{fig:Analysis of Invisible Read: YCSB, 224 Threads, Payload 4 bytes, Skew 0, 10 ops/trans.}
  & Fig. \ref{fig:Impact of Transaction Size: YCSB-B, 100M Records, 224 Threads, Payload 4 bytes, Skew 0.8.}
  & Fig. \ref{fig:Effect of Delay provided by Extra Read: YCSB-A, 100M records, 224 threads, skew 0.9, 10 ops/trans.}
  & Fig. \ref{fig:comp_tuple100m_skew0-099}\\
 \hline
  Skew            &0   &0   &0.8   &0.9  &\$6 \\
  Cardinality     &\$1 &\$2 &$10^8$&$10^8$&$10^8$\\
  Payload  (Byte) &4   &4   &4     &\$5  &4\\
  Xact Size       &10  &10  &\$4   &10   &10\\
  Read Ratio(\%)  &0,5 &\$3 &50,95 &50   &50,95\\
  \# Threads      &224 &224 &224   &224  &224\\
 \end{tabular}
  \end{scriptsize}
 \end{center}
\end{table}
\fi


==> tmp/src/appen.tex <==
\appendix
 This section describes the result related to TPC-C.
 %
 CCBench currently supports TPC-C benchmark partially.
 Among protocols, CCBench supports only Silo.
 CCBench supports only two (Payment and NewOrder) out of five transctions in TPC-C.
 We denote the workload as TPC-C-NP.
 %
 
 TPC-C or a subset of TPC-C has been used to evaluate concurrency control protocols.
 %
 % New proposal papers
 Silo~\cite{tu2013speedy} uses all the five transactions on the Silo system~\cite{silo_git}.
 TicToc~\cite{yu2016tictoc} uses only the NewOrder and Payment transactions on the DBx1000 system~\cite{dbx1000}.
 FOEDUS~\cite{kimura2015foedus} uses all the five transactions on the FOEDUS system~\cite{foedus_git}.
 MOCC~\cite{wang2016mostly} uses all the five transactions on the FOEDUS system~\cite{foedus_git}.
 Cicada~\cite{lim2017cicada} uses all the five transactions extending the DBx1000 system~\cite{dbx1000}.
 Latch-free SSN~\cite{wang2017efficiently} uses all the five transactions on the ERMIA system~\cite{ermia_git}.
 STOv2~\cite{STOv2} uses all the five transactions on the STO system~\cite{sto_git}.
 ACC~\cite{DBLP:conf/cidr/TangJE17} uses all the five transactions using the ACC system based on the Doppel system~\cite{Doppel}.
 AOCC~\cite{AOCC_Guo} uses only the the NewOrder, Payment, and the original Reward transactions on the DBx1000 system~\cite{dbx1000}.
 Transaction batching and reordering~\cite{tx_batch} does not use any TPC-C transactions on Cicada system~\cite{cicada_git}.
 % Transaction chopping
 IC3~\cite{IC3} uses all the five transactions extending the Silo system~\cite{silo_git}.

% analysis paper
 Abyss paper~\cite{yu2014staring} uses only the NewOrder and Payment transactions on the DBx1000 system~\cite{dbx1000}.
 MVCC evaluation paper~\cite{wu2017empirical} uses all the five transactions extending the Peloton system~\cite{peloton}.
 Trireme paper~\cite{trireme} does not use any TPC-C transactions on Trireme system which is not open source.
%



==> tmp/src/cache-proof.tex <==
\section{Analysis of Cache}
\label{sec:Cache Effect}

In this section, we discuss the following two effects of cache.
{\bf Cache-line conflict} happens when many worker threads access the same cache-line with some writes (e.g. accessing a single shared counter).
%
Then, the cache-line is occupied by a single thread and the other threads are internally blocked.
%
{\bf Cache-line replacement} happens when transactions access a large amount of data (e.g. high cardinality, low skew or large payload).
Then, data accesses incline to replace the contents of L1/L2/L3 cache.
\subsection{Cache-Line Conflict}
\label{sec:changing_database_size}
\input{src/cache_figure.tex}

%
Some protocols adopt centralized ordering (e.g., shared counter)~\cite{jung2013performance,kim2016ermia} while some others do decentralized ordering~\cite{tu2013speedy,yu2016tictoc,wang2016mostly,lim2017cicada}.
We first analyze the negative effect of the centralized ordering.
%
The results are shown in Figs.~\ref{fig:ycsbB_tuple1k-1g}, \ref{fig:ycsbC_tuple1k-1g}, \ref{fig:ycsbB_tuple1k-1g_ar}, and \ref{fig:ycsbC_tuple1k-1g_ca}.
The details of the workload are described in the graph caption. 
% omit?
Since the result of YCSB-A have the same trend as those of YCSB-B, it is omitted.
%YCSB-C is a read-only workload, so the abort rate is 0, and the corresponding result about abort rate is omitted.
%
Fig.~\ref{fig:central_tuple1k-1g} illustrates that the throughput of ERMIA and SI do not scale although their scheduling spaces are wider than that of SVCC serializable protocols.
This is because both protocols depend on a central data object
 %(i.e., a shared counter for the timestamp of both protocols and transaction mapping table of ERMIA), and access to the central data structure
that causes the cache-line conflict, which in turn causes performance degradation.
%This is consistent with the claims in ~\cite{tu2013speedy, wang2016mostly}.
%\cite{tu2013speedy} describes in Section 5.2 that MemSilo + GlobalTID does not scale because it issues a commit tid with a single shared counter.
%\cite{wang2016mostly} states in Section 5.3 that on large machines such as GryphonHawk, ERMIA 's centralized data structure for inter-thread communications used by SSN becomes a major bottleneck.
%\cite{wang2016mostly} also states that interthread communication impedes scalability in Section 2.2.

%
To investigate the degree of the inefficiency, we measured the throughput of {\tt fetch\_add}.
The results are shown in Figs.~\ref{fig:fetch_add_test_tps} and \ref{fig:fetch_add_test_cm}. 
The cache miss rate is measured using the Linux Perf tool, and it is about L3.
Fig.~\ref{fig:fetch_add_test_tps} shows that one thread exhibits the best performance.
This is because frequent reads/writes to the same memory address by multiple threads cause high conflicts of a cache-line.
Fig.~\ref{fig:fetch_add_test_cm} illustrates that the L3 cache miss that rate increases as the number of threads increases.
%
Cache-line conflicts incur L3 cache misses and longer communication delay if the CPU core requiring the cache-line and the another core having it exclusively are running in the different CPU sockets. In the experiment, 28 threads setting used one socket, 56 threads setting used two sockets, 112 or more threads setting used four sockets.
%
Thus, larger L3 cache miss rate ($\geq$ 30\%) indicates occurrence of communication among sockets and it significantly deteriorates the performance of fetch\_add.
%
Consequently, centralized objects should be avoided by the above reason.

\subsection{Cache-Line Replacement}
\label{sec:Cache Miss Mitigation}
In this Section, we first discuss YCSB-B result.
In Figs.~\ref{fig:ycsbB_tuple1k-1g} and \ref{fig:ycsbB_tuple1k-1g_ar}, as cardinality increases,
(1) throughput first improves and then deteriorates, and
(2) abort rate monotonically improves.
%
When cardinality is quite low, the footprint of accessible records are also small so that all of records fit inside L3 cache.
However, it is more likely happen contentions at L1 or L2 cache.
As cardinality increases, such contentions are alleviated since accessible records increase, and performance improves.
%
It is considered that with more cardinality, the total amount of records start to overflow L3 cache.
It attracts L3 cache misses and consecutive accesses of remote socket cache or DRAM, which degrades performance.
%
%The effect of L3 cache miss is stronger than that of L1/L2 cache misses.

% YCSB-C result, cache > contention..
\input{src/read_only_cache_effect.tex}

\if 0
Here we have a hypothesis.
If the performance of a protocol is strongly affected by cache memory utilization, the location of the data to be accessed is either inside (cache-inside) or outside the cache (cache-outside).
The data location is considered to depend greatly on the cardinality.
If the cardinality is small, the data tends to be within the cache, while in the opposite case, the data is less likely to be within the cache.

This situations are evident from ~\ref{fig:ycsbC_tuple1k-1g} and~\ref{fig:ycsbC_tuple1k-1g_ca}.
If the protocol does not update shared meta data, 
the increase in cardinality degrades the throughput and increases the cache miss rate due to using large memory.
Surprisingly, 2PL, SI, and ERMIA which update shared meta data in the read only workload do not show this trend.
2PL uses reader/writer locks and operating read lock updates the shared status of the data.
SI uses centralized counter to define start and end points.
ERMIA uses transaction mapping table.
In these protocols, as it transits from small records to large records, the throughput first improves and then deteriorates, the cache miss rate first improves and then deteriorates.
The reason is considered as follows.
First, even in YCSB-C (read only), when cardinality is quite low, access items are limited, which more likely provides cache contentions.
Second, as cardinality increases, such contentions are alleviated since access items increase.
However, when cardinality increases to some extent, some records are not fit into cache, and the cache evictions incur performance degradation.

Therefore, the above hypothesis holds.
With the cache-inside workload type, more records provide better performance than cache-outside workloads.
\fi

% Invisible read
\input{src/invisible}


==> tmp/src/cache.tex <==
\section{Analysis of Cache}
\label{sec:Cache Effect}

In this section, we discuss the following two effects of the cache.
{\bf Cache-line conflict} happens when many worker threads access the same cache-line with some writes (e.g. accessing a single shared counter).
%
Then, the cache-line is occupied by a single thread and the other threads are internally blocked.
%
{\bf Cache-line replacement} happens when transactions access a large amount of data (e.g. high cardinality, low skew, or large payload).
Then, data accesses incline to replace the contents of the L1/L2/L3 cache.

\subsection{Cache-Line Conflict}
\label{sec:changing_database_size}
\input{src/cache_figure.tex}

%
Some protocols adopt centralized ordering (e.g., a shared counter)~\cite{jung2013performance,kim2016ermia} while others have a decentralized ordering~
\cite{
  lim2017cicada,
  tu2013speedy,
  wang2016mostly,
  yu2016tictoc}.
We first analyzed the negative effect of centralized ordering.
%
The results are shown in Fig.~\ref{fig:central_tuple1k-1g}
Since the results for YCSB-A have the same tendency as those for YCSB-B, they are omitted.
%
Fig.~\ref{fig:central_tuple1k-1g} shows that the throughputs of ERMIA and SI do not scale although their scheduling spaces are wider than those of single-version concurrency control (SVCC) serializable protocols.
This is because both protocols depend on a centralized data structure that causes cache-line conflicts, which in turn degrade performance.
This is consistent with the claims in ~\cite{tu2013speedy, wang2016mostly}.

%
To investigate the cause of the inefficiency, we measured the throughput of {\tt fetch\_add}.
The results are shown in Figs.~\ref{fig:fetch_add}.
The L3 cache miss rate was measured using the Linux Perf tool.
Fig.~\ref{fig:fetch_add_test_tps} shows that one thread exhibits the best performance.
This is because frequent reads/writes to the same memory address by multiple threads cause many cache-line conflicts.
Fig.~\ref{fig:fetch_add_test_cm} shows that the L3 cache miss rate increases with the number of threads.
%
\color{blue} %%% begin
Cache-line conflicts result in L3 cache misses and longer communication delay because this is a situation that  a CPU core uses a cache-line and the other cores running in different CPU sockets also require the line.
\color{black} %%% end
In the experiment setting, 28 threads used one socket, 56 threads used two sockets, and 112 or more threads used four sockets.
%
Thus, a higher L3 cache miss rate ($\geq$ 30\%) indicates communication among sockets, which greatly degrades the performance of {\tt fetch\_add}.
%
That is, centralized ordering should be avoided.

\subsection{Cache-Line Replacement}
\label{sec:Cache Miss Mitigation}
Here, we first discuss the result for YCSB-B.
In Figs.~\ref{fig:ycsbB_tuple1k-1g} and \ref{fig:ycsbB_tuple1k-1g_ar}, as cardinality increases,
(1) throughput first improves and then deteriorates, and
(2) the abort ratio monotonically improves.
%
When cardinality is quite low, the footprint of accessible records is also small so that all the records fit inside the L3 cache.
The contention is more likely with L1 or L2 cache.
As cardinality increases, such contentions are alleviated since the number of accessible records increases, and performance improves.
%
It is likely that with more cardinality, the total number of records starts to overflow L3 cache.
This result in L3 cache misses and consecutive accesses to remote socket cache or DRAM degrades performance.
%

% YCSB-C result, cache > contention..
\input{src/read_only_cache_effect.tex}

% Invisible read
\input{src/invisible}


==> tmp/src/cache_figure.tex <==
\begin{figure*}[tb]
 \begin{tabular}{cccc}
  \begin{minipage}{0.23\hsize}
   \subcaptionbox{YCSB-B \label{fig:ycsbB_tuple1k-1g}}
   {\includegraphics[scale=0.7]{fig/central/comp_tuple1k-1g_ycsbB_tps.pdf}}
  \end{minipage}
  &
  \begin{minipage}{0.23\hsize}
   \subcaptionbox{YCSB-C \label{fig:ycsbC_tuple1k-1g}}
   {\includegraphics[scale=0.7]{fig/central/comp_tuple1k-1g_ycsbC_tps.pdf}}
  \end{minipage}
  &
  \begin{minipage}{0.23\hsize}
   \subcaptionbox{YCSB-B \label{fig:ycsbB_tuple1k-1g_ar}}
   {\includegraphics[scale=0.7]{fig/central/comp_tuple1k-1g_ycsbB_ar.pdf}}
  \end{minipage}
  &
  \begin{minipage}{0.23\hsize}
   \subcaptionbox{YCSB-C \label{fig:ycsbC_tuple1k-1g_ca}}
   {\includegraphics[scale=0.7]{fig/central/comp_tuple1k-1g_ycsbC_ca.pdf}}
 \end{minipage}
 \end{tabular}
 \caption{Varying Cardinality: payload 4 bytes, 224 threads, skew 0, 10 ops/trans.}
 \label{fig:central_tuple1k-1g}
\end{figure*}

% centralized counter
\begin{figure}[t]
  \begin{tabular}{cc}
    \begin{minipage}{0.45\hsize}
      \subcaptionbox{Throughput \label{fig:fetch_add_test_tps}}
      {\includegraphics[scale=0.8]{fig/central/fetch_add_tps.pdf}}
    \end{minipage}
    &
    \begin{minipage}{0.45\hsize}
      \subcaptionbox{Cache miss ratio \label{fig:fetch_add_test_cm}}
      {\includegraphics[scale=0.8]{fig/central/fetch_add_cm.pdf}}
    \end{minipage}
  \end{tabular}
  \caption{Scalability of fetch\_add}
  \label{fig:fetch_add}
\end{figure}


==> tmp/src/ccbench.tex <==
\section{CCBench}
\label{sec:Platform}

\begin{figure}[tb]
 \begin{center}
  \includegraphics[scale=0.48]{fig/CCBench-arch-update.eps}
  \caption{CCBench Architecture}
  \label{figure::CCBench Architecture}
 \end{center}
\end{figure}

\subsection{Fairness Condition}
When analyzing concurrency control protocols, their performance should be evaluated under
a fairness condition.
%
The meaning of fairness depends on the situation.
In this paper, fairness means that {\bf basic modules are shared in the analysis}.
This is because the performance of modern protocols is closely related to the exploitation of the underlying hardware; i.e., they are sensitive to the engineering details.
Therefore, the basic modules of an evaluation platform should be shared for a fair evaluation.
%
Access methods (e.g., Masstree) and local data structures (read and write sets) need to be shared among protocols.
The effects of memory allocator should be eliminated as much as possible.
The workload should be consistent among experiments.

%
% conventional platforms
%
Several analysis studies satisfy our fairness condition.
%
Yu et al.~\cite{yu2014staring} developed DBx1000~\cite{dbx1000}.
It was used to analyze multiple protocols, to evaluate TicToc~\cite{yu2016tictoc}, and to evaluate protocols on a real 1568 core machine~\cite{10.1145/3399666.3399910}.
DBx1000 currently does not support some modern protocols (Cicada, MOCC, ERMIA).
%
Wu et al.~\cite{cavalia_paper} developed Cavalia~\cite{cavalia} to compare the
HTM-assisted OCC-style protocol (HTCC) with conventional protocols. Several modern protocols (Cicada, ERMIA, Silo, TicToc, MOCC) were beyond their scope.
%
Wu et al.~\cite{wu2017empirical} developed Peloton~\cite{peloton} to compare MVCC protocols.
Several modern protocols (Cicada, ERMIA, Silo, TicToc, MOCC) were beyond their scope.
%
Appuswamy et al.~\cite{trireme} developed Trireme to compare protocols in four architecture classes including shared everything.
Several modern protocols (TicToc, Cicada, MOCC, ERMIA) were beyond their scope.

A protocol offers a variety of optimization methods.
Even if protocol {\sf P} does not initially include optimization method {\sf O},
a platform should be able to provide {\sf O} to {\sf P} if users request it
because the performance of a protocol greatly depends on the optimization method.
%
For example, {\sf RapidGC} included in Cicada can also be applied to both SI and ERMIA.
{\sf NoWait}~\cite{10.1145/356842.356846} can be applied to Silo to improve performance,
as shown in Fig. \ref{fig:ycsbA_tuple100m_skew09_slprp0-1000_tps}.
%
All of the conventional platforms do not support this concept.

Our fairness condition was not satisfied in several studies.
% Cicada
The Cicada paper ($\S$ 4.2)~\cite{lim2017cicada} states,
``Cicada and existing schemes in DBx1000 share the benchmark code,
but have separate data storage and transaction processing engines.''.
% MOCC
The MOCC paper~\cite{wang2016mostly} states that pure OCC, MOCC, and PCC (2PL variants) implementations used the FOEDUS system, the Dreadlock/WaitDie/BlindDie (2PL variants) implementations used the Orthrus system, and the ERMIA implementation used the ERMIA system, which means three benchmark systems are mixed.
% ERMIA
The ERMIA paper~\cite{kim2016ermia} states that the Silo implementation used the Silo system while the SI/SSI implementation used the ERMIA system, which means two benchmark systems were mixed.
In such studies, a huge amount of effort by experts is required to conduct a fair comparison, and this would not be easy, especially studies proposing a novel protocol or optimization.
%\color{black} %REVISED_COLOR_END

%
%
%
%
%
\subsection{CCBench: A Platform for Fair Analysis}
\label{sec:A Platform for Fair Comparison}
\input{src/opt_table}
Our CCBench analysis platform for in-memory CC protocols satisfies our fairness condition
because it shares the basic modules among protocols. The architecture of CCBench is illustrated in Fig. \ref{figure::CCBench Architecture}.
% publicly available
The code for CCBench is available on GitHub~\cite{thawkccbench}.

In CCBench, each thread executes both the client and the server logic.
The client generates a transaction with read/write operations using the workload parameters at runtime.
The server provides APIs as C++ functions, such as read, write, commit, and abort.
The client calls the APIs to run transactions.
The server runs the transactions requested from the client inside a worker thread.
The code of client is separated from that for a server the codes for both are compiled into a single executable binary.
The memory allocator, mimalloc~\cite{mimalloc}, allocates interleaved memory among CPU sockets
by using the Linux {\tt numactl} command.
Memory allocation is avoided as much as possible so that the penalty~\cite{clements2013radixvm} imposed by the Linux virtual memory system can be ignored and so that the execution performance of protocols is not degraded due to undesirable side-effects of memory allocation.
%
CCBench initializes the database for each experiment,
pre-allocates the memory for objects, and reuses the memory during the experiment.
Allocated memory for local data structures (read/write sets)
and the generated operations for a transaction are reused for the next transaction.
We properly aligned the metadata and record data to reduce false sharing.
We implemented a wrapper of Masstree~\cite{masstree_beta}, and all protocols used it as the access methods.

CCBench supports seven versatile optimization methods, as shown in Table~\ref{table::protocol_opt}.
%
(1) {\sf DecentralizedOrdering}: prevents contended accesses to a shared single counter.
(2) {\sf InvisibleReads}: read operations that do not update memory at all and cache-line conflicts do not occur.
(3) {\sf NoWait} or {\sf Wait}: immediate abort upon detection of a conflict followed by retry, or waiting for lock release.
(4) {\sf ReadPhaseExtension}: an artificial delay in the read phase inspired by the extra read process that retries the read operation.
(5) {\sf AdaptiveBackoff}: an artificial delay before restarting an aborted transaction.
(6) {\sf AssertiveVersionReuse}: allocates thread-local space denoted as version cache in Fig. \ref{figure::CCBench Architecture} to keep versions for eliminating the need for memory manager access.
(7) {\sf RapidGC}: frequent updating of timestamp watermark for GC in MVCC protocols.
%
(4) and (6) are proposed in this paper.
%

CCBench enables the use of additional optimization methods for 2PL, Silo, TicToc, SI, ERMIA, and Cicada.
%
%\color{black} %REVISED_COLOR_END
It does not support read-only optimization methods introduced in Silo, FOEDUS, MOCC, and ERMIA  because this optimization improves performance only in a specific case
(i.e., 99\% read-only transactions, 1\% write transactions, skew at 0.99),
and such a workload is not considered here.

%
% Extend CCBench
%
\input{src/extend_ccbench.tex}

%\color{blue} %REVISED_COLOR_BEGIN
\subsection{Details of Optimization Method Implementations}
\label{sec:Implementing Optimization Techniques}
%\color{black} %REVISED_COLOR_END
{\bf 2PL:~}
For efficiency, we implemented from scratch the reader/writer lock system with the compare-and-swap (CAS) operation used in the protocol.

{\bf Silo:~} We padded the global epoch (64 bits) into the cache-line size to reduce the false sharing that can be caused by a global epoch state change.
Calculation of the commit transaction id (TID) is expensive since it requires loops for both the read set and the write set.
We reduced the length of these two loops by implementing calculation at write lock acquisition and read verification.
%, which leads to more efficient processing.

{\bf Latch-Free SSN or ERMIA:~}
We used latch-free SSN to prevents expensive SSN serial validation.
This implementation avoids the validation from being a critical section.
We integrated pstamp and sstamp to reduce memory usage.
We optimized the transaction mapping table.
Straightforwardly, the mapping table is designed as a two-dimensional global array with a thread number, transaction ID (TID), cstamp, and last cstamp, which requires a lock manager for updates and read over the rows.
%
This degrades performance due to serialization.
Therefore, we designed a data structure that expresses the rows in a one-dimensional array
so that it can be latched with a CAS operation.
The performance was improved by avoiding serialization and cache-line conflicts for row element access.
We used {\sf RapidGC}~\cite{lim2017cicada}.
The transaction mapping table objects exploited our {\sf AssertiveVersionReuse}, and the memory manager almost did not work during experiments.

{\bf TicToc:~}
We implemented all three optimization methods ({\sf NoWaitTT}, {\sf PreemptiveAbort}, {\sf TimestampHistory}).
We also improved algorithm 5 in the original paper~\cite{yu2016tictoc} by removing the redundant read timestamp updates.
This is effective because if the recorded read timestamp is the same to the old one, an update of it is not necessary.

{\bf MOCC:~}
MOCC periodically resets temperature information~\cite{wang2016mostly}, which switches many cache-lines to the invalid state simultaneously and thereby degrades performance.
% hoshino
In contrast, our implementation stores the epoch ID of the latest reset timing and temperature together and thereby avoids multiple resets in the same epoch.
%
This reduces the cost of cache-line conflicts and the number of reset operations, keeping fine control of the temperature.
We did not implement MQL since our environment had only four NUMA nodes, and so its effect would be limited.
We instead used the reader/writer lock that was used in our 2PL implementation.


{\bf Cicada:~}
We implemented all six optimization methods.
({\sf SortWriteSetByContention},
{\sf PrecheckVersionConsistency},
{\sf AdaptiveBackoff},
{\sf EarlyAborts},
{\sf RapidGC},
and {\sf BestEffortInlining}).
Moreover, we fixed a logical bug, i.e., the incomplete version consistency check in the validation phase.
In the original paper~\cite{lim2017cicada}, only the read version is confirmed to still be the visible version.
However, whether the latest version is still the visible version needs to be confirmed as well.
The existence of a newer version in the observable range means that it should have been read and the transaction view will thus be broken.
We turned off the one-sided synchronization to improve throughput.

%\color{blue} %REVISED_COLOR_BEGIN
{\bf CCBench:~}
In the MVCC protocols (SI, ERMIA, and Cicada),
creating new versions and deleting old versions put a load on the memory manager.
%which is also true for memory managers with thread-local memory pools.
We, therefore, developed a new optimization method, {\sf AssertiveVersionReuse} that avoids overloading the memory manager in MVCC protocols.
This method enables each worker thread to maintain a container for future version reuse.
When GC begins, the versions collected are stored in this container.
A new version is taken from this container except if it is empty.
If it is empty, a request for space is sent to the memory manager as usual.
%
The space needed for GC is estimated before the experiment,
and memory space is allocated in advance.
This optimization minimizes the burden on the memory manager for the MVCC protocols.
%
Moreover, we introduce the use of {\sf ReadPhaseExtension} which delays execution. It was inspired by the extra read process described in $\S$ \ref{sec:Effect of Extra Read and Read Phase Extension Method}.
We also introduce {\sf AggressiveGC} optimization, which collects even visible versions, described in $\S$ \ref{sec:discussion-towards-version-lifetime-control}.
%\color{black} %REVISED_COLOR_END


%\color{blue} %REVISED_COLOR_BEGIN
\subsection{Configurable Workloads}
\label{Configurable Workloads}
%\color{black} %REVISED_COLOR_END

\input{src/analyzed_space}
% Why not tpcc
\input{src/tpcc}


==> tmp/src/cicada_repro_comment.tex <==
In Figs.~\ref{fig:ycsbA_tuple10m_ope16_rmw_skew0-099_th28_tps},
\ref{fig:ycsbB_tuple10m_ope16_rmw_skew0-099_th28_tps},
and \ref{fig:ycsbB_tuple10m_ope1_rmw_skew099_tps}, the tendencies in our results for Silo, TicToc, MOCC, ERMIA, and 2PL are
the same as those in the corresponding figures in the original paper.
%
In contrast, the results for Cicada differ.
Fig.~\ref{fig:ycsbB_tuple10m_ope1_rmw_skew099_tps} shows that Cicada has worse performance than Silo and TicToc for a read intensive workload, and this is inconsistent with the results shown in Fig.~7 in~\cite{lim2017cicada}.
%
We discuss this inconsistency at {\bf Insight 5} in $\S$~\ref{sec:problem-many-visible-versions}.
%


==> tmp/src/concl.tex <==
\section{Conclusion}
\label{sec:Conclusion}
Our CCBench concurrency control analysis platform offers seven protocols and seven versatile optimization methods, and enables the configurations of seven workload parameters.
We analyzed the protocols and optimization methods for various settings of the workload parameters with the number of threads fixed at 224 whereas previous studies~\cite{dbx1000,peloton,trireme} mostly focused on thread scalability, and none of them explored the space we analyzed.

% takeaway 
\input{src/key_takeaway.tex}

Future work includes the extension of CCBench.
\color{blue} %REVISED_COLOR_BEGIN
We will implement insertion/deletion operations, phantom avoidance, and tree indexes so that CCBench will support the TPC-C fullmix.
\color{black} %REVISED_COLOR_BEGIN
We plan to add recovery modules based on our preliminary studies~\cite{tanabe2018cicada-pwal2,nakamuraTicToc}.
%
The code for CCBench and all the data in this paper are available online at GitHub~\cite{thawkccbench}.
We expect that CCBench will help to advance transaction processing research in the many-core architecture era.


==> tmp/src/delay.tex <==
\section{Analysis of Delay}
\label{sec:Delay Control}

\input{src/delay_figure}

\subsection{Effect of NoWait}
\label{sec:Confirmation of Effect of NoWait}

One optimization method for mitigating performance degradation caused by conflicts is to place an additional artificial delay before a retry, such as with {\sf NoWaitTT}~\cite{yu2016tictoc} and {\sf AdaptiveBackoff}~\cite{lim2017cicada}.
%
In contrast to waiting for a lock release, the {\sf NoWait} method immediately releases locks when a conflict is detected and immediately retries. 
%
The question then in dealing with contention, is whether we should choose, 
{\sf NoWait} or {\sf Wait}.

To answer this question, we compared the performance of three methods for various degrees of skew: 2PL-Wait, 2PL-NoWait, and MOCC that is the mix of OCC and 2PL-Wait.
%
All operations of each transaction for 2PL-Wait were sorted in advance to avoid deadlock.
%
As shown in Fig.~\ref{fig:ycsbB_tuple100m_skew06-085_tps},
performance starts to degrade at a skew of 0.7 due to a large number of conflicts for all three protocols.
%
%We compare 2PL-Wait, 2PL-NoWait, and MOCC,  which performs similarly to 2PL-Wait for a highly conflicted situation.


MOCC demonstrated excellent performance, as shown in Fig.~\ref{fig:ycsbB_tuple100m_skew06-085_tps}. This is because MOCC manages fewer lock objects for the workloads with less skew.
%
It should be noted that 2PL-Wait and 2PL-NoWait show similar performances at skews of 0.6-0.85, so the cost of abort-retry and the cost of waiting for lock were almost the same for this workload.
Therefore, we need more contention to answer the question.

To provide more contentions, we increased the transaction size.
The cost of aborts should be smaller for short transactions and larger for long ones.
Therefore, with long transactions, the abort-retry cost is higher and may exceed the lock waiting cost.
%
%% We used YCSB-B benchmark, setting the cardinality to 100 million, skew to 0.8, and varied the number of operations.
%% Operations are sorted due to the same reason in the above.
%
% problem,
Fig.~\ref{fig:skew_on_large_records} illustrates that the lock waiting cost of {\sf Wait} and the abort-retry cost of {\sf NoWait} are similar.
Fig.~\ref{fig:ycsbB_tuple100m_skew08_ope10-100_tps} shows that {\sf Wait} comes to outperform {\sf NoWait} as the transaction size increases.
%
% Summary
%
%% {\sf NoWait} demonstrates efficiency only for small size transactions.
%
In contrast, Silo-NoWait outperformed Silo(-Wait) in
Fig.~\ref{fig:Effect of Delay provided by Extra Read: YCSB-A, 100M records, 224 threads, skew 0.9, 10 ops/trans.} (described in $\S$ \ref{sec:Effect of Extra Read and Read Phase Extension Method}).
The answer of the question is that it depends on situation.
Therefore, the control of waiting time is important for efficiency.

%\color{blue} %REVISED_COLOR_BEGIN
\underline{\bf Insight 3:}
One cannot give a general statement about which is better, {\sf NoWait} or {\sf Wait} since it depends on the situations.
%
As illustrated in Fig.~\ref{fig:ycsbB_tuple100m_skew08_ope10-100_tps}, {\sf Wait} comes to outperform {\sf NoWait} as transaction size increases.
%
On the other hand, as illustrated in Fig.~\ref{fig:ycsbA_tuple100m_skew09_slprp0-1000_tps}, Silo with {\sf NoWait} comes to outperform original Silo.
%
It suggests the importance of the adaptive behavior.
Adaptive concurrency controls have been studied in~\cite{wang2016mostly,adaptiveCC,abortML,PelotonConcept}.
%
However, the importance has not discussed in the depth of optimization method except {\it backoff} optimization such as {\sf AdaptiveBackoff}~\cite{lim2017cicada}.
%
We consider studies on adaptive optimization method is still a frontier.

%
% Payload size, Extra Read
%
\subsection{Effect of Payload Size}
\label{sec:Effect of Extra Read and Read Phase Extension Method}
%
We analyzed the effect of payload size, which has not yet done so far, to our knowledge.
Fig.~\ref{fig:ycsbA_tuple100m_skew09_val4-1k_tps} shows the relationship between the throughput and the payload size about Silo and TicToc.
The result that throughput first increases as payload size increases, and then it starts to decrease after passing a certain point.
%
The increase of payload size would likely cause performance degradation in OCC, and this is consistent with the right half of the graph.
However, the performance improvement in the left half of the graph is counter intuitive.
%
We hypothesize that this improvement was due to by the delay caused by the extra reads process that reads two or more times if there is an interruption in the concurrent update transactions.
%
An increase in payload size lengthens the time to read the payload.
%
This increases possibility of an interruption due to an update transaction,
which increases the number of extra reads.
%
This behavior extends the read phase and reduces the number of transactions that run through the validation phase in parallel.
%
As the number of committed update transactions decreases, the number of read validation failures also decreases, which leads to performance improvement.
%
Delaying the retry of atomic reads reduces the number of concurrent worker threads involved in the validation phase for the entire system, which also reduces contentions.
%

% Read phase extension
\input{src/read_phase_extension.tex}


==> tmp/src/delay_figure.tex <==
\begin{figure}[t]
  \begin{tabular}{cc}
    \begin{minipage}{0.45\hsize}
     \begin{flushleft}
      \subcaptionbox{Throughput \label{fig:ycsbB_tuple100m_skew06-085_tps}}
      {\includegraphics[scale=0.9]{fig/delay/comp_ycsbB_tuple100m_skew06-085_tps.pdf}}
     \end{flushleft}
    \end{minipage}
    &
    \begin{minipage}{0.45\hsize}
      \subcaptionbox{Abort Ratio \label{fig:ycsbB_tuple100m_skew06-085_ar}}
      {\includegraphics[scale=0.9]{fig/delay/comp_ycsbB_tuple100m_skew06-085_ar.pdf}}
    \end{minipage}
  \end{tabular}
  \caption{Wait or NoWait: YCSB-B, 100 M Records, 224 Threads, Payload 4 bytes, 10 ops/trans.}
  \label{fig:skew_on_large_records}
\end{figure}


%
% Wait outperforms NoWait
%
\begin{figure}[t]
  \begin{tabular}{cc}
    \begin{minipage}{0.45\hsize}
     \subcaptionbox{Throughput.\label{fig:ycsbB_tuple100m_skew08_ope10-100_tps}}
     {\includegraphics[scale=0.9]{fig/delay/comp_ycsbB_tuple100m_skew08_ope10-100_tps.pdf}}
    \end{minipage}
    &
    \begin{minipage}{0.45\hsize}
     \subcaptionbox{Abort ratio.\label{fig:ycsbB_tuple100m_skew08_ope10-100_ar}}
     {\includegraphics[scale=0.9]{fig/delay/comp_ycsbB_tuple100m_skew08_ope10-100_ar.pdf}}
    \end{minipage}
  \end{tabular}
 \caption{Impact of Transaction Size: YCSB-B, 100M Records, 224 Threads, Payload 4 bytes, Skew 0.8.}
 \label{fig:Impact of Transaction Size: YCSB-B, 100M Records, 224 Threads, Payload 4 bytes, Skew 0.8.}
\end{figure}


%
% Read Phase Extension
%
\begin{figure*}[t]
  \begin{tabular}{ccc}
    \begin{minipage}{0.3\hsize}
     \subcaptionbox{Throughput \label{fig:ycsbA_tuple100m_skew09_val4-1k_tps}}
      {\includegraphics[scale=1.15]{fig/delay/comp_ycsbA_tuple100m_skew09_val4-1k_tps.pdf}}
    \end{minipage}
   &
    \begin{minipage}{0.3\hsize}
     \subcaptionbox{Extra Reads \label{fig:ycsbA_tuple100m_skew09_val4-1k_er}}
     {\includegraphics[scale=1.15]{fig/delay/comp_ycsbA_tuple100m_skew09_val4-1k_er.pdf}}
    \end{minipage}
   &
    \begin{minipage}{0.3\hsize}
     \subcaptionbox{Read Phase Extension Method\label{fig:ycsbA_tuple100m_skew09_slprp0-1000_tps}}
     {\includegraphics[scale=1.15]{fig/delay/comp_ycsbA_tuple100m_skew09_slprp0-1000_tps.pdf}}
    \end{minipage}
  \end{tabular}
 \caption{Effect of Delay provided by Extra Read: YCSB-A, 100M records, 224 threads, skew 0.9, 10 ops/trans.}
 \label{fig:Effect of Delay provided by Extra Read: YCSB-A, 100M records, 224 threads, skew 0.9, 10 ops/trans.}
\end{figure*}



==> tmp/src/diff.tex <==
In our setting, we applied the RapidGC to ERMIA and SI in all the cases, NoWaitto Silo in Fig. \ref{fig:ycsbA_tuple100m_skew09_slprp0-1000_tps}, and adaptive backoff to TicToc in Fig. \ref{fig:tuple10m_val1k_ycsb_high_tps}


==> tmp/src/environment.tex <==
\subsection{Environment}
% Machine
The evaluation environment consisted of a single server with four Intel (R) Xeon (R) Platinum 8176 CPUs @ 2.10GHz processors.
%
Each CPU had 28 physical cores with hyper-threading, and the server had 224 logical cores.
%
Each physical core had 32 KB private L1d cache and 1 MB private L2 cache.
%
The 28 cores in each processor shared a 39 MB L3 cache.
%
The total cache size was about 160 MB.
Forty-eight DDR4-2666 DIMM were connected, each 32 GB, so the total size was 1.5 TB.

% Result
In all graphs in this paper showing the results of CCBench, each plot point shows the average for 5 runs, each with a duration of 3 sec.
We confirmed that these numbers produce stable CCBench results.
%
The error bars indicate the range between the maximum and minimum values.
We counted the number of committed and aborted transactions to calculate average throughput.
We used the \texttt{rdtscp} instruction to measure the latency of the transitions and their portions.
Each worker thread was pinned to a specific CPU core in every experiment.
%


==> tmp/src/extend_ccbench.tex <==
%\color{blue} %REVISED_COLOR_BEGIN
Users of CCBench can easily add new protocols to the platform.
After replicating a directory that has an existing protocol, the user rewrites the functions corresponding to the transactions with begin/read/write/commit/abort operations in the transaction executor class.
The user can then reuse the basic modules in the platform: workload generator, memory management, and so on.
%
Users easily attach or detach optimization methods provided by CCBench to their protocols simply by rewriting the preprocessor definition in the Makefile.
A developer guide for CCBench users is available~\cite{cc_format}.
%
One of our team members implemented a simple OCC protocol following this guide~\cite{occ_nemoto}; and published the experience for other users~\cite{nemotoccbench}.
%
Users can also switch the configuration of the optimization methods, key-value size, and protocol details in the same way as done in the online example.
%
In an experiment, the user can set the workload by specifying the runtime arguments using the seven workload parameters listed in Table \ref{tab:Experimental Parameters}.
%
% try to reduce
%
This design makes it easier to conduct experiments compared with DBx1000~\cite{dbx1000}, which manages these values as preprocessor definitions in a file {\tt config.h}.

%\color{black} %REVISED_COLOR_END


==> tmp/src/intro.tex <==
\section{Introduction}
\subsection{Motivation}
%
Transacting processing systems for thousands of CPU cores in a single server
have been emulated~\cite{yu2014staring}, implemented~\cite{kimura2015foedus},
or analyzed~\cite{10.1145/3399666.3399910}.
%
Along with these systems, a variety of concurrency control protocols for a single server~
\cite{
  kim2016ermia,   % ERMIA
  lim2017cicada,  % Cicada
  tu2013speedy,   % Silo
  wang2016mostly, % MOCC
  yu2016tictoc}    % TicToc
have been proposed in recent years for use on many-core architecture.
%
These modern protocols use a variety of optimization methods, and their behaviors depend on the workload characteristics (e.g., skew, read ratio, cardinality).
%
Recent protocol studies have compared these protocols with conventional ones~
\cite{
  kim2016ermia,   % ERMIA
  lim2017cicada,  % Cicada
  tu2013speedy,   % Silo
  wang2016mostly, % MOCC
  yu2016tictoc}   % TicToc
, and recent analytic studies have compared the performance of conventional protocols on a common platform~
\cite{
  trireme,                 % Trireme
  10.1145/3399666.3399910, % Supredome
  wu2017empirical,         % MVCC
  yu2014staring}.          % DBx1000 or Abyss
%
These studies mostly evaluated the scalability of the protocols.
This paper takes the standpoint that it is already known that modern protocols are scalable,
and focuses on other factors that contribute to performance on many-core environment.
%
This sort of analysis has not yet been conducted, to our knowledge.
%

To conduct such an analysis, some of recent studies have a problem that
they compare their new protocols with others using multiple different platforms.
%
For example, evaluation in ERMIA~\cite{kim2016ermia}, MOCC~\cite{wang2016mostly}, and Cicada~\cite{lim2017cicada} used two or three platforms.
%
The experiments using mixed platforms can produce approximate or inaccurate results because the performance of protocols on many-core architecture is highly associated with the exploitation of underlying hardware.
%
In such experimental conditions, it is only possible to conduct macroscopic evaluation (i.e. scalability), but detailed analysis is difficult.
%
The conduct of such a detailed analysis requires a single unified comparison platform.

%
% Platform
%
To conduct a fair comparison, a common analysis platform is necessary.
It should provide shared core modules such as access methods (concurrent index) and thread-local data structures (read and write sets) for any of the protocols.
It should also provide a variety of optimization methods to support a way to deeply understand the protocols.
%
%
Finally, the platform should be publicly available for reproduction experiments.
% 3. Modern protocols
There are open source platforms, including DBx1000~\cite{dbx1000}, Peloton~\cite{peloton}, and Cavalia~\cite{cavalia}.
Unfortunately, they do not provide certain modern protocols~\cite{
  kim2016ermia,   % ERMIA
  lim2017cicada,  % Cicada
  tu2013speedy,   % Silo
  wang2016mostly, % MOCC
  yu2016tictoc}.  % TocToc

%
%
%
\subsection{Contributions}
\label{sec:Contribution}
The first contribution of the paper is {\bf CCBench}: a platform for evaluating and fairly comparing concurrency control protocols.
It provides flexible configurations for both optimizations and workloads.
%
The protocols currently implemented in CCBench are two-phase locking (2PL), Silo, MOCC, TicToc, snapshot isolation (SI), latch-free serial safety net (SSN), and Cicada.
%
CCBench supports five versatile optimization methods used in conventional protocols and two identified in this work (Table \ref{table::protocol_opt}, $\S$\ref{sec:A Platform for Fair Comparison}).
Optimization methods can thus be applied to non-original protocols.
For example, {\sf NoWait}~\cite{bernstein1987concurrency} can be applied to Silo, rapid garbage collection (GC)~\cite{lim2017cicada} can be applied to multi-version protocols, and {\sf AdaptiveBackoff}~\cite{lim2017cicada} can be applied to all protocols.
%
Fairness in analyzing protocols is achieved through shared modules including a workload generator, access methods (Masstree~
\cite{
  masstree_beta,
  mao2012cache}
), local datasets (read/write sets), and a memory manager (the mimalloc~\cite{mimalloc} and {\sf AssertiveVersionReuse} proposed in this paper).
Evaluation of protocols under various conditions is enabled by the provision of seven workload configuration parameters: skew, payload size, transaction size, cardinality, read ratio, read-modify-write (RMW) or not, and the number of worker threads.
%
CCBench and all of the data in this paper are available online at GitHub~\cite{thawkccbench}.

The second contribution of the paper is the {\bf analysis of cache, delay, and version lifetime for 224 threads.}
We clarified the effects of the protocols on the performance factors by configuring the optimization methods and workload settings.
%
As suggested elsewhere~\cite{yu2014staring} and \cite{kimura2015foedus}, the era of a thousand cores is just around the corner, so conventional analysis studies have focused on evaluating thread scalability~
\cite{
  10.14778/3055540.3055548,
  wu2017empirical,
  yu2014staring}.
However, we performed all of analyses with {\it 224 threads on 224 cores}.

% Cache
We first investigated the effects of optimization methods related to {\bf cache}.
By determining that a centralized counter increases cache-line conflicts and
degrades performance, we gained two insights.
% Insight 1.
{\bf I1:} The performance of optimistic concurrency control (OCC) for a read-only workload rapidly degrades as cardinality increases even without L3 cache misses ($\S$\ref{sec:Cache Miss Mitigation}).
% Insight 2.
{\bf I2:} Silo outperforms TicToc for some write-intensive workloads due to {\sf InvisibleRead} ($\S$\ref{sec:Effect of Invisible Read}).

%
% Delay
%
We then investigated the effects of optimization methods related to {\bf delay},
and gained two more insights.
% Insight 3.
{\bf I3:} The effectiveness of two approaches to coping with conflict ({\sf Wait} and {\sf NoWait}) depends on the situation. ($\S$\ref{sec:Confirmation of Effect of NoWait}).
%
% Insight 4.
{\bf I4:} OCC reads the same record two or more times due to concurrent transaction interruption.
Surprisingly, it can improve performance in certain situations, and we have defined a new optimization method {\sf ReadPhaseExtension} based on it ($\S$\ref{sec:Effect of Extra Read and Read Phase Extension Method}).

%
% Version lifetime
%
Finally, we investigated the effects of optimization methods related to {\bf version lifetime}
 for multi-version concurrency control (MVCC) protocols, and gained two last insights.
{\bf I5:} Mixing different implementations are inappropriate.
Silo outperformed Cicada for the YCSB-B workload in an unskewed environment,
which is inconsistent with previously reported results where different systems are used~\cite{lim2017cicada}.
% Insight 6
{\bf I6:} Even state-of-the-art GC technique cannot improve the performance of MVCC if only a single long transaction is mixed into the workload.
To overcome this problem, we defined a new optimization method, {\sf AggressiveGC}.
It requires an unprecedented protocol that weaves GC into MVCC beyond the current assumption that
versions can not be collected if they may be read by transactions ($\S$\ref{sec:discussion-towards-version-lifetime-control}).

\subsection{Organization}
The rest of this paper is organized as follows.
$\S$\ref{sec:Preparation} describes the existing concurrency control protocols and the evaluation environment.
$\S$\ref{sec:Platform} describes the fairness condition, CCBench, implementation of the optimization methods, and workloads.
$\S$\ref{sec:Reproduction of Prior Work} describes the reproduction of experiments performed in prior work using CCBench.
$\S$\ref{sec:Cache Effect} describes the effect of cache exploitation.
$\S$\ref{sec:Delay Control} describes the effect of delay control.
$\S$\ref{sec:version-lifetime-control} describes the effect of version lifetime management.
$\S$\ref{sec:Related Work} describes related work, and
$\S$\ref{sec:Conclusion} concludes the paper with a summary of the key points and a mention of future work.


==> tmp/src/invisible.tex <==
\input{src/invisible_figure}
\subsection{Effect of Invisible Read}
\label{sec:Effect of Invisible Read}
%
Updating shared data among threads running in different CPU sockets trigger L3 cache misses due to cache-line conflicts mainly, leading to performance degradation.
The read operation in Silo does not update the corresponding metadata, which can avoid cache-line conflicts.
%
This method is referred to as {\sf InvisibleRead}~\cite{marathe2004design}.
%
{\sf InvisibleReads} effectively improve performance for read-intensive workloads; however, its behaviors have not been explored yet.
% TicToc
The read operations of TicToc typically update the read timestamp, so they are not {\sf InvisibleRead}.

%
% Result
To investigate the details of {\sf InvisibleReads}, we measured the performance of Silo and TicToc
for various read ratios and cardinalities.
The results are shown in Figs.~\ref{fig:ycsb_rratio10-90_tps}-\ref{fig:ycsb_rratio10-90_ca}.
% highly contended
Fig.~\ref{fig:ycsb_rratio10-90_tps} shows that for low cardinality
and write-intensive workloads, TicToc-1K (where 1K means 1000 records) outperforms Silo-1K.
%
% here
%
The abort ratio of TicToc-1K is much worse than that of Silo-1K in this case, as illustrated in Fig.~\ref{fig:ycsb_rratio10-90_ar}.
As shown in Fig.~\ref{fig:ycsb_rratio10-90_tps}, in the read-most (90\%) case,
Silo-1K outperforms TicToc-1K, as evidenced by the rapidly increasing abort ratio (Fig.~\ref{fig:ycsb_rratio10-90_ar}).
{\sf InvisibleRead} method contributes the performance in this case.
% low contended
For high cardinality workloads, Silo-1M (where 1M means 1 million records) always outperforms TicToc-1M.
The abort ratios of Silo-1M and TicToc-1M are both zero, as illustrated in Fig.~\ref{fig:ycsb_rratio10-90_ar}.
This is seemingly a mysterious finding since the abort ratios for both Silo and TicToc are almost zero, and their L3 cache miss ratios are almost the same as illustrated in Fig.~\ref{fig:ycsb_rratio10-90_ca}.
%
This is because dealing with contention resolution processing in TicToc
requires three functions: timestamp history management, early abort judgment, and read timestamp update.
These functions require executing additional instructions and thus degraded performance.
When weaving {\sf InvisibleReads} into the process, a protocol is difficult to exploit them.
%

\underline{\bf Insight 2:}~
For a detailed analysis of protocols, contention should be carefully considered.
Contentions are caused by not only read ratio but also cardinality and skew.
%
We observed that Silo outperformed TicToc not only for read-only but also for write-intensive workloads.
This has not been reported yet in conventional studies~\cite{yu2016tictoc, lim2017cicada, trireme}.
%except that OSTO outperforms TSTO slightly~\cite{STOv2}.
%
These results are provided by {\sf InvisibleReads} that prevent cache misses for low contention cases, and by its simple design that does not require computations for conflict resolution nor track anti-dependencies.


==> tmp/src/invisible_figure.tex <==
\begin{figure*}[tb]
  \begin{tabular}{ccc}
    \begin{minipage}{0.33\hsize}
      \subcaptionbox{Throughput \label{fig:ycsb_rratio10-90_tps}}
      {\includegraphics[scale=1]{fig/invisible/comp-silo-tictoc_rratio10-90_tps.pdf}}
    \end{minipage}
    &
    \begin{minipage}{0.33\hsize}
      \subcaptionbox{Abort Ratio \label{fig:ycsb_rratio10-90_ar}}
      {\includegraphics[scale=1]{fig/invisible/comp-silo-tictoc_rratio10-90_ar.pdf}}
    \end{minipage}
    &
    \begin{minipage}{0.33\hsize}
      \subcaptionbox{Cache-Miss Ratio \label{fig:ycsb_rratio10-90_ca}}
      {\includegraphics[scale=1]{fig/invisible/comp-silo-tictoc_rratio10-90_ca.pdf}}
    \end{minipage}
  \end{tabular}
  \caption{Analysis of Invisible Read. 224 Threads, Payload 4 bytes, Skew 0, 10 ops/trans. Cardinality $10^3$ or $10^6$ records}
  \label{fig:Analysis of Invisible Read: YCSB, 224 Threads, Payload 4 bytes, Skew 0, 10 ops/trans.}
\end{figure*}



==> tmp/src/key_facets.tex <==
The concurrency control protocols we analyzed are classified as follows.
(1) Pessimistic (2PL~\cite{eswaran1976notions}).
(2) Optimistic (Silo~\cite{tu2013speedy} and TicToc~\cite{yu2016tictoc}).
(3) Multi-version (SI~\cite{jung2013performance} and ERMIA~\cite{kim2016ermia}).
(4) integration of optimistic and pessimistic (MOCC~\cite{wang2016mostly}).
(5) integration of optimistic and multi-version (Cicada~\cite{lim2017cicada}).
We explain the details in the below.


==> tmp/src/key_takeaway.tex <==
%
% Difference
%
We classified versatile optimization methods into three class of factors: cache, delay, and version lifetime.
Through the analysis of protocols with CCbench, we gained six insights.
{\bf I1:}~As cardinality increases, OCC for read-only workloads deteriorated without L3 cache misses.
{\bf I2:}~Silo outperformed TicToc for write-intensive workloads attributed to {\sf InvisibleRead} for unskewed and high cardinality cases.
{\bf I3:}~Extra read regulated contentions, and we defined {\sf ReadPhaseExtension} based on it.
{\bf I4:}~Effectiveness of {\sf Wait} or {\sf NoWait} depended on situations.
{\bf I5:}~Results produced from mixed different implementations may be inconsistent with theory.
%Silo and TicToc can outperform Cicada under a high skew situation (0.99) and Cicada underperforms Silo under YCSB-A/B with skewless environment, which is superficially inconsistent with \cite{lim2017cicada}.
{\bf I6:}~Even {\sf RapidGC } cannot improve performance of MVCC if only a single long transaction exists, and we defined {\sf AggressiveGC} for a solution.


==> tmp/src/letter.tex <==
\setcounter{page}{1}

\section*{Our Thanks to Meta Reviewer and Reviewers from the Heart}
 Dear meta reviewer, thank you for inviting us to submit a revised draft of our manuscript entitled,
 ``An Analysis of Concurrency Control Protocols for In-Memory Database with CCBench''
 to {\it PVLDB}. We also appreciate the time and effort you and each of the reviewers have dedicated to providing insightful feedback on ways to strengthen our paper.
 Thus, it is with great pleasure that we resubmit our paper for further consideration.
 %
 We have incorporated changes that reflect the detailed suggestions and comments you have graciously provided.
 %
 We also hope that our edits are written in
\color{blue}
 blue color
\color{black}
 and the responses we provide below satisfactorily address all the issues and concerns you and the reviewers have noted.
 %
 To facilitate your review of our revisions, the following is a point-by-point response to the questions and comments delivered in your letter.

\section{Response to Meta Reviewer}
\subsection{Meta-1}
\begin{screen}
 For each algorithm include a performance comparison to results reported in the paper that introduced the algorithm.
\end{screen}

\input{src/resp-M1}

\subsection{Meta-2}
\begin{screen}
Include TPC-C results for all algorithms.
\end{screen}

\input{src/resp-M2}

\subsection{Meta-3}
\begin{screen}
Greatly improve the writing clarity.
This is very important since part of the paper’s value is as a tutorial.
There are many grammar errors, which is a distraction, but the bigger problem is the vague sentences where the reader has to guess what is meant.
\end{screen}

\input{src/resp-M3}

\subsection{Meta-4}
\label{sec:Meta-4}
\begin{screen}
Expand the Related Work section, which is too sketchy. In particular, do not simply list related papers but compare your work to theirs.
\end{screen}

\input{src/resp-M4}

\subsection{Meta-5}
 \label{sec:Meta-5}
\begin{screen}
Explain how to extend the framework with other CC algorithms, storage mechanisms, and optimizations.
\end{screen}

\input{src/resp-M5}

\section{Response to Reviewer-1}
\subsection{Review1-D1}

\begin{screen}
This paper is better suited as an experiment paper since the novel research contributions of the paper are low.
Even though it is not tagged as an experiment paper, I evaluate it as one, and my evaluation is based on that characterization.
\end{screen}

Thanks for your kind comments. As you suggested, we intended to submit this paper to the Experiment and Analysis category.
We are surprised to know that this paper is not categorized in the section. We really appreciate your kind evaluation!


\if 0
Thanks for your comment.
First, to inform the features of many protocols analyzed in this paper,
We add a brief explanation of protocols at the beginning of $\S$ \ref{sec:Cache Effect}. Please see there in the paper.

Second, we summarized the result of our analysis as 6 insights, and describe them at $\S$ \ref{sec:Contribution} and \ref{sec:Conclusion}.
\fi

\subsection{Reviewer1-D2}
\begin{screen}
Since the paper starts with a summary of the different protocol, it would be good to summarize the key facets of each protocol in one table that allows the reader to grasp them at once and better understand the key results presented in the experiments.
Much like Table 2, but for the original approaches.
Similarly, since there are a lot of experiments presented, it would be good to provide a section/table that summarizes the key takeaways.
\end{screen}

Thanks for your suggestion.
%
As for the summary of key facets of protocols, we add a brief explanation of the characteristics of protocols in $\S$ \ref{sec:Concurrency Control Protocols}.
%
We also add Table \ref{tab:Experimental Parameters} so that reader can grasp analyzed spaces in this paper.

To present the key takeaways, we summarized our findings as six insights.
%
We describe
insight 1 in $\S$~\ref{sec:Cache Miss Mitigation},
insight 2 in $\S$~\ref{sec:Effect of Invisible Read},
insight 3 in $\S$~\ref{sec:Confirmation of Effect of NoWait},
insight 4 in $\S$~\ref{sec:Effect of Extra Read and Read Phase Extension Method},
insight 5 in $\S$~\ref{sec:problem-many-visible-versions} and
insight 6 in $\S$~\ref{sec:discussion-towards-version-lifetime-control}.
%
We mention them in
$\S$ \ref{sec:Contribution} and $\S$ \ref{sec:Conclusion}.


\subsection{Reviewer1-D3}

\begin{screen}
All the experiments are with YCSB.
Even though YCSB is pretty configurable, it is still very simple transactions not very representative of realistic applications.
It would be good to add a bit more diversity with the benchmarks, e.g., consider the suite of benchmarks supported by OLTPBench
%(https://github.com/oltpbenchmark/oltpbench/tree/master/src/com/oltpbenchmark/benchmarks)
 and pick one or two from there that adds diversity in the workloads, potentially making the analysis more interesting.
\end{screen}

\input{src/resp-R1-D3}

\subsection{Reviewer1-D5}

\begin{screen}
How extensible is this framework for the addition of other algorithms or implementations of storage engines or other configurations?
\end{screen}

%Thanks for your comment.
%We revised the related work in $\S$ \ref{sec:A Platform for Fair Comparison}.
%Please see $\S$ \ref{sec:Meta-5} (Meta-5).
\input{src/resp-M5}

\subsection{Reviewer1-D6}

\begin{screen}
The language of the paper needs significant improvements. For instance,\\
-- ``We second organize two performance factors that have not been fully organized yet.'' What does this sentence mean?\\
-- ``The rapid garbage collection at Cicada demonstrates''\\
-- ``We show these optimizations harness the version lifetime factor with limitations.''\\
and many more..\\
\end{screen}

\input{src/resp-M3}

\subsection{Reviewer1-D7}
\begin{screen}
The related work section needs more work. Related work is more than just a list of papers as the current section presents. It would be good to better compare and contrast with similar related work studying performance characteristics.
\end{screen}

%Thanks for your comment.
%We revised the related work in $\S$ \ref{sec:Related Work}.
%Please see $\S$ \ref{sec:Meta-4} (Meta-4).

\input{src/resp-M4}

\section{Response to Reviewer-3}
\subsection{Reviewer3-D1}

\begin{screen}
It can be a nice contribution to evaluate state-of-the-art concurrency control protocols with a fair performance comparison among them and demonstrate what
insights are learned from the study and how we should design concurrency control protocols in the future. This paper tries the first step (fair performance evaluation) but does not give many insights to the readers. Therefore, not much can be learned from this paper besides what has been learned in the original papers describing these concurrency control protocols.
\end{screen}


\input{src/resp-R3-D1}

\subsection{Reviewer3-D2}

\begin{screen}
Given that all of these state-of-the-art protocols have their own optimized implementations. The paper needs to justify that the implementations in CCBench are at least as optimized as the original implementations. An evaluation of both original protocols and CCBench on standard benchmarks is necessary.
\end{screen}

\input{src/resp-M1}

\subsection{Reviewer3-D3}

\begin{screen}
 There are some factual errors in the paper.

 - $\S$ 2.1: The description of TicToc says: ``NoWait in validation does not wait for lock releasing at validation phase.
 It instead immediately aborts and retries the
transaction.'' The NoWait optimization in TicToc does not abort and retry the entire transaction, it only retries the lock acquiring process.
This leads to a significant performance difference.

 - End of $\S$ 2.1: ``For the deadlock resolution, our 2PL adopts the NoWait optimization technique introduced by TicToc that immediately aborts when conflict
is detected.''. NoWait is not introduced by TicToc, NoWait has existed decades before TicToc, TicToc is just reusing the idea for the lock acquiring process...
Furthermore, NoWait is not an ``optimization'' with respect to other deadlock resolution schemes. It is just one scheme with its own properties. Many previous papers
have shown that NoWait can underperform other 2PL protocols under certain scenarios (e.g., [29]).
\end{screen}

Thanks for your comment, and we are sorry that we misunderstand the NoWait optimization of TicToc.
We revised our implementation and describe the optimization as {\sf NoWaitTT} in the paper so that it can be clearly distinguished from the conventional {\sf NoWait}.
We re-implemented the optimization method and redraw the graph in Fig. \ref{fig:tuple10m_val1k_ycsb_high_tps} indicating as {\tt Torg}.

\subsection{Reviewer3-D4}

\begin{screen}
Most of the findings discussed in the evaluation of this paper have already been known.
Some were discussed in the original papers of these protocols.
The discussion in this paper restates these findings but there is little deeper discussion.
\end{screen}

Thanks for your comments.
Since our writing quality in the first version was not enough, we summarized our findings as insights as mentioned in the response to Reviewer3-D1.
It includes three new optimization methods.
We are happy if you kindly see it and judge the quality again.

\subsection{Reviewer3-D5}

\begin{screen}
The evaluation tries to cover a large multi-dimensional space of parameters.
But clearly not all the configurations are shown. Please explain which part of the space is evaluated and which part is not.
\end{screen}

Thank you for your suggestion.
We describe a parameter space in Table \ref{tab:Experimental Parameters} so that readers can understand the analyzed space.

\subsection{Reviewer3-D6}

\begin{screen}
Related to D5, In Figure 7 when showing the effect of invisible read, Silo (with invisible read) outperforms TicToc (without invisible read).
In Figure 10, when showing the effect of extra read, TicToc (without extra read) outperforms Silo (with extra read).
The two experiments use different parameters and different conclusions can be drawn.
Clearly, it is possible to pick a specific parameter setting to show one protocol better than another; it is important to demonstrate the effectiveness of certain optimizations in a more general setting.
\end{screen}

\input{src/resp-R3-D6}
%
 %and as illustrated in Fig. \ref{fig:ycsbA_tuple100m_skew09_slprp0-1000_tps}, Silo with {\sf NoWait} outperforms original Silo.
%
% delete
%
% Aside from this paper, an interesting example is timestamp history optimization in TicToc.
Its effect is not observed by original paper \cite{yu2016tictoc}, while it has been confirmed by a recent one \cite{STOv2}\footnote{need revision}.

\subsection{Reviewer3-D7}

\begin{screen}
There is no evaluation of TPC-C.
\end{screen}

\input{src/resp-M2}

\section{Response to Reviewer-4}
\subsection{Reviewer4-D1}

\begin{screen}
This paper has several language issues.
Starting from the very first sentence (“... concurrency control protocols have [been] proposed for in-memory database
systems.”), it contains numerous syntactic and semantic errors.
Some of the errors even make the meaning of sentences opposite.
For instance: “... causes optimistic protocols to read excessively \_by interrupting\_ the updating transaction...” should be “as getting interrupted by”.
“... the possibility of being interrupted by the update transaction \_improves\_,...” should be “increases”.Combined with the above issue is the presentation of this paper. For instance, it took a while for this reviewer to capture the overview of this work from the first section.
Its narrative is not easy to follow.
This paper should go through substantial edits aided by native speakers.
\end{screen}

\input{src/resp-M3}

\subsection{Reviewer4-D2}

\begin{screen}
If CCBench is only to compare a couple of CC schemes evaluated in this paper, its value is quite limited.
It is unclear whether/how one can extend CCBench for a new, yet-to-come CC scheme that might be drastically different from existing ones.
Are the authors committed to keeping extending CCBench for future CC schemes?
If not, it has to be easy for \_others\_ to extend it for their new CC scheme. So far it is unclear whether that is the case.
\end{screen}

%Thanks for your comment.
%We add the procedure at the end of $\S$ \ref{sec:A Platform for Fair Comparison}. Please see $\S$ \ref{sec:Meta-5} (Meta-5).
\input{src/resp-M5}

\subsection{Reviewer4-D3}

\begin{screen}
The paper has various observations that make sense, such as the effects of cache-miss and dirtying additional cache-lines.
However, they do not look significant enough to motivate yet another optimization to exploit the effects, at least for general cases.
For example, the effect of “Extra Read” reported in $\S$ 5.2 is hard to exploit.
One cannot blindly place waits to reduce contention although it improved the throughput in this particular case.
Unless there is some finding to distill a generally-applicable optimization, the value of these findings is limited.
\end{screen}

Thanks for your comment.
We defined three new optimization methods in this revised manuscript.
%
They are the {\sf ReadPhaseExtension} that is inspired by the effect of the extra read ($\S$ \ref{sec:Effect of Extra Read and Read Phase Extension Method}), and the {\sf AggressiveGC} that is inspired by the negative effect of a long transaction shown in Figure \ref{fig:comp_cicada-ninline_ycsbA_tuple1m_gci1us-1s_tps}, and the {\sf AssertiveVersionReuse} for MVCC.
%
As mentioned in {\sf ReadPhaseExtension} ($\S$ \ref{sec:Effect of Extra Read and Read Phase Extension Method}), one can use this method just specifying the delay.
This method can exploit local conflict information in the validation phase, and thus it can perform more efficiently than conventional methods that use only global information.

\section*{Thanks Again!}
Again, thank you for giving us the opportunity to strengthen our manuscript with your valuable comments and queries.
We have worked hard to incorporate your feedback and hope that these revisions persuade you to accept our submission.

Sincerely,

Takayuki Tanabe, Takashi Hoshino, Hideyuki Kawashima, Osamu Tatebe


==> tmp/src/opt_table.tex <==
\begin{table*}
 \begin{center}
  %    \begin{scriptsize}
  \begin{small}
   \caption{Versatile Optimization Methods in CCBench.
   {\sf ---}: Irrelevant or Incompatible.
   {\sf Org}: Supported by original protocol.
   {\sf CCB}: Supported by CCBench.
   ({$\alpha$}) Delay inspired by the extra reads in OCC ($\S$ \ref{sec:Effect of Extra Read and Read Phase Extension Method}). Proposed in this work.
   ({$\beta$}) CCBench conducts read lock for hot records and invisible read for non-hot records.
   ({$\gamma$})  {\sf NoWait} locking optimization detects a write lock conflict and immediately aborts and retries the transaction. {\sf NoWaitTT} releases all locks and re-locks them.
   ({$\delta$}) Lightweight memory management. Proposed in this work ($\S$ \ref{sec:Implementing Optimization Techniques}).
   ({$\epsilon$}) {\sf PreempiveAbort} and {\sf TimestampHistory} cannot be applied to others.
   ({$\zeta$})   {\sf SortWriteSetByContention}, {\sf PrecheckVersionConsistency}, {\sf EarlyAborts}, {\sf BestEfforInlining} cannot be applied to others.
   %
   We applied optimization methods as follows.
   {\sf NoWait}: Silo in Fig. \ref{fig:ycsbA_tuple100m_skew09_slprp0-1000_tps}.
   {\sf RapidGC}: ERMIA and SI in all cases.
   {\sf AssertiveVersionReuse}: Cicada, ERMIA, and SI in all cases. 
   {\sf AdaptiveBackoff}: TicToc in Fig. \ref{fig:tuple10m_val1k_ycsb_high_tps} and all protocols in Figs. \ref{fig:ycsbA_tuple10m_ope16_rmw_skew099_tps}, \ref{fig:ycsbA_tuple10m_ope16_rmw_skew0-099_th28_tps}, \ref{fig:ycsbB_tuple10m_ope16_rmw_skew0-099_th28_tps}, and \ref{fig:ycsbB_tuple10m_ope1_rmw_skew099_tps}.
   }
   \label{table::protocol_opt}
   \begin{tabular}[tb]{r|cc|ccc|cc}
    \begin{tabular}{c} {\rm Performance}\\{\rm Factor}\end{tabular}&
    \multicolumn{2}{|c|}{{\rm CPU Cache}}&\multicolumn{3}{|c|}{{\rm Delay by Conflict}}&\multicolumn{2}{|c}{{\rm Version Lifetime}}\\ \hline\hline
    \begin{tabular}{c} {\sf Optimization} \\{\sf Method}          \end{tabular}&
    \begin{tabular}{c} {\sf Decentralized}\\{\sf Ordering}        \end{tabular} &
    \begin{tabular}{c} {\sf Invisible}    \\{\sf Read}            \end{tabular} &
    \begin{tabular}{c} {\sf NoWait}     \\or {\sf Wait}        \end{tabular} &
    \begin{tabular}{c} {\sf Adaptive}     \\{\sf Backoff}         \end{tabular} &
    \begin{tabular}{c} {\sf ReadPhase}    \\{\sf Extension}({$\alpha$})\end{tabular} &
    \begin{tabular}{c} {\sf AssertiveVersion}\\{\sf Reuse}({$\delta$})\end{tabular} &
    \begin{tabular}{c} {\sf Rapid}\\{\sf GC} \end{tabular} \\  \hline\hline
2PL~\cite{weikum2001transactional} &Org, CCB &---                 &Org,CCB       &CCB      &--- & --- &---\\
Silo~\cite{tu2013speedy}           &Org, CCB &Org, CCB            &CCB           &CCB      &CCB & --- &---\\
MOCC~\cite{wang2016mostly}         &Org, CCB &Org, CCB ({$\beta$})&---           &CCB      &CCB & --- &---\\
TicToc({$\epsilon$})~\cite{yu2016tictoc}&Org, CCB &---            &CCB ({$\gamma$}) &CCB   &CCB & --- &---\\
SI~\cite{jung2013performance}      &---      &---                 &---           &CCB      &--- & CCB &CCB\\
ERMIA~\cite{kim2016ermia}          &---      &---                 &---           &CCB      &--- & CCB &CCB\\
Cicada({$\zeta$})~\cite{lim2017cicada}       &Org, CCB &---       &---           &Org, CCB &CCB & CCB &Org, CCB\\
   \end{tabular}
  \end{small}
 \end{center}
\end{table*}


==> tmp/src/prep.tex <==
\section{Preliminaries}
\label{sec:Preparation}
\input{src/protocol}
\input{src/environment}



==> tmp/src/protocol.tex <==
\subsection{Concurrency Control Protocols}
\label{sec:Concurrency Control Protocols}

\input{src/key_facets.tex}

{\bf Silo~\cite{tu2013speedy}}~
%\color{blue} %REVISED_COLOR_BEGIN
is an OCC protocol.
It has affected subsequent concurrency control protocols.
For example, FOEDUS~\cite{kimura2015foedus} and MOCC~\cite{wang2016mostly} extend the commit protocol of Silo.
Silo chooses the design of {\sf InvisibleRead}~\cite{marathe2004design} that does not update the metadata of the records during any read operation.
The invisible read process avoids cache-line conflicts, so it provides scalability, as shown in \cite{wang2016mostly}.
%\color{black} %REVISED_COLOR_END

{\bf TicToc~\cite{yu2016tictoc}}~
\label{protocol::tictoc}
%\color{blue} %REVISED_COLOR_BEGIN
is an OCC based on timestamp ordering with data-driven timestamp management.
TicToc has a larger scheduling space than Silo so that it can commit schedules where Silo cannot.
TicToc provides three optimization methods.
{\sf PreemptiveAbort} conducts abort processing immediately if an abort is determined before write locking in the validation phase.
{\sf NoWaitTT} does not wait for lock releasing in the validation phase.
It instead releases the locks and retries the validation phase after a fixed duration of a wait without an abort.
{\sf TimestampHistory} expands the scheduling space by recording the write timestamp of an older version so that some of the read operations on the version can be verified after the record is overwritten.
%\color{black} %REVISED_COLOR_END

{\bf MOCC~\cite{wang2016mostly}}~
%\color{blue} %REVISED_COLOR_BEGIN
exhibits high performance for a wide range of workloads by adaptively switching its policy by adding pessimistic locking and temperature management to Silo.
MOCC locks high temperature (on highly conflicted) records while keeping the order of records locking to avoid deadlocks in the read phase.
The MOCC queuing lock (MQL) integrates a MCS lock that can be timed out~\cite{scott2001scalable} and a reader/writer fairness MCS lock~\cite{mellor1991scalable}.
%\color{black} %REVISED_COLOR_END

{\bf Cicada~\cite{lim2017cicada}}~
%\color{blue} %REVISED_COLOR_BEGIN
combines the OCC protocol, 
\color{blue}
a multi-version protocol
(multi-version timestamp ordering)
\color{black}
, and distributed timestamp generation.
%Due to the nature of the OCC protocol, cache-line conflicts are mitigated among concurrent transactions.
The distributed timestamp generation eliminates the need to access the centralized counter that conventional MVCC protocols require,
and thereby dramatically mitigates cache-line conflicts.
Cicada has a variety of optimization methods.
%
{\sf EarlyAbort} initiates an abort if it is predicted during the read phase.
{\sf BestEffortInlining} embeds an inline version in the record header at the top of the version list to reduce indirect reference cost.
{\sf PrecheckValidation} checks whether read versions are still valid at the early timing of the validation phase.
{\sf RapidGC} is a quick and parallel GC optimization method.
{\sf AdaptiveBackoff} dynamically decides how long to wait before retrying.
{\sf SortWriteSetByContention} detects conflicts before conducting wasted works due to aborts.
%\color{black} %REVISED_COLOR_END


{\bf SI~\cite{berenson1995critique}}
%\color{blue} %REVISED_COLOR_BEGIN
is a MVCC protocol that can generate write-skew and read-only-transaction anomalies, so it does not produce serializable schedules.
%\color{black} %REVISED_COLOR_END
Under SI, a transaction reads a snapshot of the latest committed version.
The write operations are also reflected in the snapshot.
%
%\color{blue} %REVISED_COLOR_BEGIN
SI requires a unique timestamp assignment for each transaction to provide snapshots.
%\color{black} %REVISED_COLOR_END
To determine the unique timestamp, a centralized shared counter is required.

{\bf SI with latch-free SSN~\cite{kim2016ermia}}~
integrates SI and SSN~\cite{wang2015serial} and exploit the latch-free mechanism~\cite{wang2017efficiently}.
%\color{blue} %REVISED_COLOR_BEGIN
SSN detects and aborts dangerous transactions that possibly lead to non-serializable schedules.
We refer to the integration of SI and SSN as {\bf ERMIA} in this paper.
%\color{black} %REVISED_COLOR_END

{\bf 2PL~\cite{eswaran1976notions,  weikum2001transactional}}~
%\color{blue} %REVISED_COLOR_BEGIN
releases all read/write locks at the end of each transaction.
{\sf NoWait} method, which immediately aborts the running transaction when a conflict is detected,
was originally proposed as a deadlock resolution mechanism~\cite{10.1145/356842.356846},
while we use it as an optimization method too.
%\color{black} %REVISED_COLOR_END


==> tmp/src/read_only_cache_effect.tex <==
% YCSB-C, cache, new
We investigated the strong effect of the L3 cache miss ratio.
As illustrated in Fig.~\ref{fig:ycsbC_tuple1k-1g_ca},
when cardinality is no more than $10^5$, the L3 cache miss ratios for Silo, TicToc, and Cicada are almost zero.
This is because the L3 cache size is 39 MB and the size of a record including the header is 64 byte (64 $\times 10^5 < 39 \times 10^6$).
However, as cardinality increases, their throughputs decrease linearly, as illustrated in Fig.~\ref{fig:ycsbC_tuple1k-1g}.
This is attributed to L1/L2 cache misses.
When cardinality is more than $10^5$, we observe L3 cache misses have a strong effect on performance even for read-only workloads.

% + mocc
The negative effect of read contentions is shown in Figs.~1 and 6 in~\cite{wang2016mostly}.
The cache-line conflicts that occur due to read lock contentions degrade performance and the difference in performance between OCC and 2PL rapidly increases as the number of threads increases.
%
However, there is no mention in the paper that the greater the number of the L3 cache misses for a read-only workload, the smaller the performance difference between OCC and 2PL.
As illustrated in Fig.~\ref{fig:ycsbC_tuple1k-1g}, when cardinality is no less than $10^7$, Silo, TicToc, and 2PL have almost the same throughput.
Moreover, their L3 cache miss ratio is almost the same, as shown in Fig.~\ref{fig:ycsbC_tuple1k-1g_ca}.
%
For read-only workloads, the differences in performance among protocols converge due to the L3 cache misses when the database size is large.
This has not been reported so far.

%\color{blue} %REVISED_COLOR_BEGIN
% Insight
\underline{\bf Insight 1:}~
% In cache
Even the entire database is within L3 cache,
as cardinality increases,
(1) OCC for read-intensive workloads improves due to decrease of L1/L2 cache-line conflicts, and
(2) OCC for read-only workloads deteriorates due to an increase of L1/L2 cache-line replacements in L1/L2 caches.
% Out cache
As known, if the entire database slightly overflows the L3 cache, the performance of protocols diverge.
While on the other hand, the entire database is much larger than the L3 cache, the performance of Silo, TicToc, MOCC, and 2PL converges to the same level due to frequent L3 cache-line replacements.
%
%\color{black} %REVISED_COLOR_END


==> tmp/src/read_phase_extension.tex <==
Besides {\sf Wait}, {\sf NoWait}, and {\sf AdaptiveBackoff},
we present a novel delay-related optimization method,
{\sf ReadPhaseExtension}, which was inspired by the positive effect of extra reads.

Comparing Figs.~\ref{fig:ycsbA_tuple100m_skew09_val4-1k_tps} and \ref{fig:ycsbA_tuple100m_skew09_val4-1k_er} reveals that the curves are similar.
This indicates that the throughput and the number of extra reads are correlated.
%
If this is correct, adding an artificial delay into the read phase should produce similar results.
%
We conducted such an experiment for a payload size of 4 bytes.
The results (Fig.~\ref{fig:ycsbA_tuple100m_skew09_slprp0-1000_tps}) show that a certain amount of additional delay (less than 9000 clocks) improves performance. This effect is similar to that of the extra read process.
We refer to this artificial delay as {\sf ReadPhaseExtension} and define it as a new optimization method.
{\sf ReadPhaseExtension} is configured by setting the delay on the basis of local conflict information.
%
This optimization method can exploit information on the access conflicts for each record during the read and validation phases whereas {\sf AdaptiveBackoff} uses only global information across all worker threads.

%\color{blue} %REVISED_COLOR_BEGIN
\underline{\bf Insight 4:}~
The extra read process plays a key role in the performance of OCC protocols.
It is known that the contention regulation caused by delay can contribute to performance improvement depending on the situation.
%
A remarkable finding here is that the {\sf ReadPhaseExtension} inspired by the extra read process can also improve performance.
% This kind of extension is similar to the artificial delay (1 micro sec or {\sf \_mm\_pause}) in {\sf NoWaitTT}.
% Necessary?
{\sf ReadPhaseExtension} differ from {\sf NoWaitTT} since it exploits information on conflicting records inside transactions to adjust the delay whereas the delay in {\sf NoWaitTT} is fixed.
%
Such additional delay in the read phase and the use of thread local conflict information is a unique in optimization method.
%
%\color{black} %REVISED_COLOR_END


==> tmp/src/related.tex <==
\section{Related Work}
\label{sec:Related Work}
\input{src/related_core.tex}

==> tmp/src/related_core.tex <==
Yu et al.~\cite{yu2014staring} evaluated CC protocols using DBx1000~\cite{dbx1000} which is open source.
They evaluated the scalability of CC protocols using a real machine and an emulator.
Three recent protocols~
\cite{
  kim2016ermia,
  lim2017cicada,
  wang2016mostly}
~that we offer in CCBench, are not included in DBx1000~\cite{dbx1000}.
% Peloton
Wu et al.~\cite{wu2017empirical} empirically evaluated MVCC protocols using Peloton~\cite{peloton}, which is open source.
They evaluated not only scalability, but also the contention effect, read ratio, attributes, memory allocation, and index.
They did not evaluate SVCC and modern MVCC protocols evaluated in this paper~
\cite{
  lim2017cicada,
  tu2013speedy,
  wang2016mostly,
  yu2016tictoc}.
% Trireme
Appuswamy et al.~\cite{trireme} evaluated CC protocols in four architecture classes using Trireme, which is not open source.
%
They determined that the shared everything architecture is still the best option for contention-tolerant in-memory transaction engines.
% Cavalia
Wu et al.~\cite{cavalia_paper} proposed an HTM-assisted CC protocol combined with Cavalia~\cite{cavalia}, which lacks some protocols evaluated in this paper~\cite{tu2013speedy,yu2016tictoc,wang2016mostly,wang2017efficiently,lim2017cicada}.
%Silo, TicToc, MOCC, ERMIA, and Cicada.
%CC protocols for distributed systems have been evaluated elsewhere \cite{10.14778/3055540.3055548,wang2020comprehensive}; this paper focuses on protocols on a single many-core architecture.

%
% Difference
%
%This study presented CCBench analysis platform~\cite{thawkccbench}.%, which is open source and enables to the application of a variety of versatile optimization methods about seven protocols.
%
Whereas previous studies mostly evaluated scalability and did not explore the behavior of protocols when thread parallelism was set to a high degree, this study fixed the thread parallelism at 224 and analyzed protocols for various settings.% of seven workload configuration parameters.
%
We classified a variety of methods into three classes of performance factors: cache, delay, and version lifetime.
This analysis let to the identification of three new optimization methods.

% others



==> tmp/src/repro.tex <==
%% \section{Reproduction of Experiments Performed in Prior Work}
\section{Reproduction in Prior Work}
\label{sec:Reproduction of Prior Work}
\input{src/repro_figure}

% CCBench measurement
Before presenting our analysis of reproducing experiments performed in prior work,
we explain how we validated the correctness of the CCBench implementation,
so that it successfully reproduces the results of experiments performed in previous work.
% DBx1000 measurement
We did this by evaluating DBx1000~\cite{dbx1000}, a standard analysis platform, as used in~\cite{10.1145/3399666.3399910} to validate the behavior of CCBench.
%
In all graphs showing DBx1000 result, we set {\tt CPU\_FREQ} to 2.095 after measuring the real clock rate used for {\tt rdtsc} instruction and each plot point shows an average of 10 runs. The duration of each run was 4.5 to 10 seconds.
For the access method, we used a hash index for DBx1000 and Masstree for CCBench.
%
DBx1000 does not support read-modify-write operations in YCSB workload so their plots are not presented in the reproduction of MOCC and Cicada.

%
% TicToc
%
\subsection{TicToc}
Our first experiment was aimed at reproducing {\rm TicToc} results~\cite{yu2016tictoc}.
We experimented with the settings in Figs.~6, 7, and 8 in that paper.
We set the epoch interval longer than 40 ms so that cache-line conflicts for the global epoch rarely occurred in {\rm Silo}.
\input{src/tictoc_repro.tex}

One finding is particularly noteworthy.
In Fig.~\ref{fig:tuple10m_val1k_ycsb_high_tps},
the behaviors of {\rm Silo} and {\rm TicToc} differ from those of Fig.~8 in \cite{yu2016tictoc}.
The performance of {\rm TicToc} improves as the number of threads increases, but when the number exceeds a certain value, the performance starts to deteriorate due to an increase in read/write conflicts.
Therefore, we presume that some sort of backoff was applied to {\rm TicToc} in \cite{yu2016tictoc}, and attach {\sf AdaptiveBackoff} to {\rm TicToc}.
This is shown as {\tt T+BO} in Fig.~\ref{fig:tuple10m_val1k_ycsb_high_tps}.
The performance curve for {\tt T+BO} is similar to that of Fig.~9 in \cite{yu2016tictoc}.
The lower performance of the original TicToc protocol shown as {\tt Torg} is attributed to excessive delays and read validation failures.
{\sf NoWaitTT} inserts fixed delays into the validation phase, which tends to result in read validation failure.
%
Therefore, {\tt Torg} shows low performance in this graph, and {\rm TicToc} is better due to the short read phase.
% DBx1000
The results of DBx1000 is also illustrated in the Figures, and their behaviors are similar to ours.

% Summary
Fig.~\ref{fig:tuple10m_val1k_ycsbC_tps} shows that Silo and TicToc exhibit linear scalability for a read-only workload, and Fig.~6 in \cite{yu2016tictoc} shows almost linear scalability.
Fig.~\ref{fig:tuple10m_val1k_ycsb_medium_tps} above and Fig.~7(a) in \cite{yu2016tictoc} show almost the same results.
%
In summary, CCBench tends to appropriately reproduce the results of {\rm TicToc}, and the results of CCBench are consistent with those of DBx1000.

%
% MOCC
%
\subsection{MOCC}
The second reproduction was aimed at reproducing MOCC results~\cite{wang2016mostly}.
Our MOCC implementation differs from the original one in terms of temperature and MQL, as described in $\S$\ref{sec:Implementing Optimization Techniques}.
To reproduce the in the original paper,
we experimented with the settings shown in Figs.~6 and 7 in the original paper~\cite{wang2016mostly}.
%The details of the workload are described in graph captions.

The results in Fig.~\ref{fig:ycsbC_tuple50_tps} appropriately reproduce those in Fig.~6 in the original paper.
The performance scales with the number of threads in the read-only workloads.
%
The underperformance of MOCC with more than 168 threads compared with Silo is attributed to the overhead of MOCC.
When MOCC reads a record, it accesses the corresponding temperature information and checks whether the temperature is high or not.

% hoshino
The results in Figs.~\ref{fig:silo-mocc_tuple50_rratio10-100_tps} and \ref{fig:silo-mocc_tuple50_rratio10-100_ar} appropriately reproduce those in Fig.~7 in the original paper. When the write ratio increases from 0\% to 10\%, the abort rate rapidly increases, and the performance deteriorates.
%
This is because the write operation produces a large amount of read validation failures.
In Fig.~\ref{fig:silo-mocc_tuple50_rratio10-100_tps}, the performance of Silo deteriorates at a write rate of 0-40\%,
while it improves at a write rate of 40-60\%.
There is thus a trade-off between reduced record-access contentions due to reduced write operations and frequent read validation failures due to increased read operations.
In contrast, MOCC shows stable performance, the reason for which is considered that abort is less likely to occur by temperature control.

% Summary
{\rm MOCC} and {\rm Silo} exhibit scalability in Fig.~\ref{fig:ycsbC_tuple50_tps} above, while {\rm MOCC} and {\rm FOEDUS} in Fig.~6 in \cite{wang2016mostly} also exhibit scalability.
Fig.~\ref{fig:silo-mocc_tuple50_rratio10-100_tps} shows the throughput of MOCC and Silo when varying the write ratio.
This result is almost the same as that in Fig.~7 in \cite{wang2016mostly}.
Abort ratio of {\rm Silo} and {\rm MOCC} in Fig.~\ref{fig:silo-mocc_tuple50_rratio10-100_ar} is consistent with that in Fig.~7 in \cite{wang2016mostly}.
%
In summary, CCBench appropriately reproduces the results of MOCC.
%

\subsection{Cicada}
\label{sec:Cicada}
Our third experiment was aimed at reproducing Cicada results~\cite{lim2017cicada}.
The workload parameters were set almost the same as those in \cite{lim2017cicada}.
The details of the workload are described in the graph caption.
The differences between this paper and the original paper are as follows:
(1) we redesigned and reimplemented all protocols.
(2) {\sf AdaptiveBackoff} was implemented in all protocols because it is easily attachable and effective for performance improvement.

Figs.~\ref{fig:ycsbA_tuple10m_ope16_rmw_skew099_tps},
\ref{fig:ycsbA_tuple10m_ope16_rmw_skew0-099_th28_tps},
\ref{fig:ycsbB_tuple10m_ope16_rmw_skew0-099_th28_tps},
and
\ref{fig:ycsbB_tuple10m_ope1_rmw_skew099_tps}
%
illustrate the experimental results reproducing Figs.~6a, 6b, 6c, and 7 in the original paper, respectively.
%
\input{src/cicada_repro_comment.tex}


==> tmp/src/repro_figure.tex <==
% 
% TicToc
%
\begin{figure*}[tb]
  \begin{tabular}{ccc}
    \begin{minipage}{0.33\hsize}
      \subcaptionbox{YCSB (Read-Only). 2 queries per transaction, skew 0.\label{fig:tuple10m_val1k_ycsbC_tps}}
      {\includegraphics[scale=1.02]{fig/reproduction/comp_tuple10m_val1k_ycsbC_tps.pdf}}
    \end{minipage}
    &
    \begin{minipage}{0.33\hsize}
      \subcaptionbox{YCSB (Medium Contention). 16 queries per transaction, 90\% reads-10\% writes, skew 0.8.\label{fig:tuple10m_val1k_ycsb_medium_tps}}
      {\includegraphics[scale=1.02]{fig/reproduction/comp_tuple10m_val1k_ycsb_medium_tps.pdf}}
    \end{minipage}
    &
    \begin{minipage}{0.33\hsize}
      \subcaptionbox{YCSB (High Contention). 16 queries per transaction, 50\% reads-50\% writes, skew 0.9\label{fig:tuple10m_val1k_ycsb_high_tps}}
      {\includegraphics[scale=1.02]{fig/reproduction/comp_tuple10m_val1k_ycsb_high_tps.pdf}}
    \end{minipage}
  \end{tabular}
 \caption{Reproduction of TicToc experiment. 10M records, payload 1K bytes. Different access methods (hash for DBx1000, Masstree for CCBench). CCBench without index outperformed (39.6 Mtps) DBx1000 (30 Mtps) at 80 threads}
\end{figure*}

% 
% MOCC
%
\begin{figure*}[tb]
 \begin{tabular}{ccc}
  \begin{minipage}{0.3\hsize}
   \subcaptionbox{Read Only Workload.\label{fig:ycsbC_tuple50_tps}}
   {\includegraphics[scale=1.1]{fig/reproduction/comp_ycsbC_tuple50_tps.pdf}}
  \end{minipage}
  &
  \begin{minipage}{0.3\hsize}
   \subcaptionbox{Read-Write YCSB. 224 threads.\label{fig:silo-mocc_tuple50_rratio10-100_tps}}
   {\includegraphics[scale=1.1]{fig/reproduction/comp-silo-mocc_tuple50_rratio10-100_tps.pdf}}
  \end{minipage}
  &
  \begin{minipage}{0.3\hsize}
   \subcaptionbox{Read-Write YCSB. 224 threads.\label{fig:silo-mocc_tuple50_rratio10-100_ar}}
   {\includegraphics[scale=1.1]{fig/reproduction/comp-silo-mocc_tuple50_rratio10-100_ar.pdf}}
  \end{minipage}
 \end{tabular}
 \caption{Reproduction of MOCC experiment. YCSB, 50 records, 10 ops/trans, Skew 0, Payload 4 bytes, reads are pure read, writes are read modify write.}
\end{figure*}

% 
% Cicada
%
\begin{figure*}[tb]
  \begin{tabular}{cccc}
    \begin{minipage}{0.23\hsize}
     \subcaptionbox{Write-Intensive. 16 requests/trans, skew 0.99, 50\% RMW - 50\% pure reads\label{fig:ycsbA_tuple10m_ope16_rmw_skew099_tps}}
      {\includegraphics[scale=0.8]{fig/reproduction/comp_ycsbA_tuple10m_ope16_rmw_skew099_tps.pdf}}
    \end{minipage}
    &
    \begin{minipage}{0.23\hsize}
      \subcaptionbox{Write-Intensive. 28 threads. 16 requests/trans, 50\% RMW - 50\% pure reads\label{fig:ycsbA_tuple10m_ope16_rmw_skew0-099_th28_tps}}
      {\includegraphics[scale=0.8]{fig/reproduction/comp_ycsbA_tuple10m_ope16_rmw_skew0-099_th28_tps.pdf}}
    \end{minipage}
    &
    \begin{minipage}{0.23\hsize}
      \subcaptionbox{Read-Intensive. 28 threads. 16 requests/trans, 5\% RMW - 95\% pure reads\label{fig:ycsbB_tuple10m_ope16_rmw_skew0-099_th28_tps}}
      {\includegraphics[scale=0.8]{fig/reproduction/comp_ycsbB_tuple10m_ope16_rmw_skew0-099_th28_tps.pdf}}
    \end{minipage}
   &
    \begin{minipage}{0.23\hsize}
      \subcaptionbox{Read-Intensive. 1 requests/trans, skew 0.99, 5\% RMW - 95\% pure reads\label{fig:ycsbB_tuple10m_ope1_rmw_skew099_tps}}
      {\includegraphics[scale=0.8]{fig/reproduction/comp_ycsbB_tuple10m_ope1_rmw_skew099_tps.pdf}}
    \end{minipage}
  \end{tabular}
 \caption{Reproduction of Cicada experiment. 10M records, payload 100 bytes}
 \label{fig:Reproduction of Cicada experiment. 10M records, payload 100 bytes}
\end{figure*}


==> tmp/src/resp-M1.tex <==
% R3-D2
Thanks for your comment.
To justify the implementations in CCBench, we used a standard benchmark system DBx1000.
%
DBx1000 supports DL\_DETECT, NO\_WAIT, HEKATON, SILO, TICTOC, and we evaluated SILO and TICTOC.
The results are shown in Fig. \ref{fig:tuple10m_val1k_ycsbC_tps} and \ref{fig:tuple10m_val1k_ycsb_medium_tps}.
The results show that CCBench and that of DBx1000 showed similar trends, and
Silo-DBx1000 and TicToc-DBx1000 outperformed those of CCBench.
We consider the reason is the difference in access methods (hash index for DBx1000 and Masstree for CCBench because DBx1000 does not support concurrent index).
It also should be noted that CCBench without index was around 30\% better than DBx1000 (with hash index) at 80 threads in the setting of Fig. \ref{fig:tuple10m_val1k_ycsbC_tps}.
%
Thus we consider the implementations of Silo and TicToc in CCBench are at least as optimized as the original implementations for these workloads.
%

However, we do not know the performance of DBx1000 for RMW workloads because DBx1000 does not support the operations.
Thus, we could not conduct experiments related to Fig. \ref{fig:Reproduction of Cicada experiment. 10M records, payload 100 bytes} since all the results in this Figure required RMW operation.


==> tmp/src/resp-M2.tex <==
Thanks for your comment.
TPC-C is a popular and standard benchmark and often used to evaluate the scalability of OLTP systems.
The scalabilities have been well explored, while this paper analyzes different parameter spaces beyond the scalability as shown in Table \ref{tab:Experimental Parameters}.
We conducted all the experiments setting the thread size to 224.
%
Then, unfortunately TPC-C benchmark does not useful for our purpose.
We gained six insights in our analysis with our workload parameter sets.
However, we think it is difficult to gain another insight using TPC-C because the scalability has been well studied and it is simpler than our parameter sets.

%
We described the reason why we do not use TPC-C benchmark in $\S$ \ref{Configurable Workloads} in the manuscript.


==> tmp/src/resp-M3.tex <==
Thanks for your comment.
We fully and carefully revised this manuscript, and we also used a proofreading service to improve the quality and readability of this paper.
The revised places are colored in
\color{blue}
blue.
\color{black}


==> tmp/src/resp-M4.tex <==
Thanks for your comment.
We revised the related work in $\S$ \ref{sec:Related Work}.
We first summarize conventional studies and then describe the differences between this paper and them.


==> tmp/src/resp-M5.tex <==
Thanks for your comment.
To explain how to extend CCBench, we first prepare a guide for the extension~\cite{cc_format}.
We then asked a member of our laboratory to implement a simple OCC protocol in CCBench following the guide.
He easily implemented it~\cite{occ_nemoto} and published the experience for CCBench users~\cite{nemotoccbench}.
%
We described the above contents at the final paragraph of $\S$ \ref{sec:A Platform for Fair Comparison} in the manuscript.


==> tmp/src/resp-R1-D3.tex <==
 Thanks for your suggestion.
 %
 It is interesting to find out certain optimizations that perform efficiently for real applications.
 We think it is also interesting to clarify the facets of optimization methods in detail.
 Since there are no silver bullets, each method should have pros and cons.
 The motivation of this paper is to find out such characteristics with unprecedented workload settings.
 %
 Thus, we prefer settings that a method demonstrates both good and bad results to understand the characteristics well.
 %
 However, as you point out, real applications are also impressive, so we will study such workloads in future work.
 Thank you for your great suggestion!


==> tmp/src/resp-R3-D1.tex <==
Thank you for your comment.
We fully rewrote this paper so that readers can understand its contributions.
%
We summarized our findings as six insights.
We describe
insight 1 in $\S$~\ref{sec:Cache Miss Mitigation},
insight 2 in $\S$~\ref{sec:Effect of Invisible Read},
insight 3 in $\S$~\ref{sec:Confirmation of Effect of NoWait},
insight 4 in $\S$~\ref{sec:Effect of Extra Read and Read Phase Extension Method},
insight 5 in $\S$~\ref{sec:problem-many-visible-versions} and
insight 6 in $\S$~\ref{sec:discussion-towards-version-lifetime-control}.
%
We mention them in
$\S$ \ref{sec:Contribution} and $\S$ \ref{sec:Conclusion}.


==> tmp/src/resp-R3-D6.tex <==
 Thanks for your comment.
 It is interesting to find out certain optimizations that perform efficiently or inefficiently in a variety of settings like centralized data objects.
 It is also interesting to clarify the facets of optimization methods.
 Since there are no silver bullets, each method should have pros and cons.
 The purpose of this paper is to find out such characteristics with unprecedented workload settings.
 %
 Thus, we prefer settings that a method demonstrates both good and bad results to understand the characteristics well.
%
 In this paper, {\sf NoWait} performs well for short transactions while it does not for long transactions as in Fig. \ref{fig:ycsbB_tuple100m_skew08_ope10-100_tps},
 Silo, TicToc, MOCC outperforms Cicada as shown in Fig. \ref{fig:comp_tuple100m_skew0-099} for certain situations, and Silo outperforms TicToc as shown in Fig. \ref{fig:ycsb_rratio10-90_tps} for certain situations.
 These results are not reported in original papers, and it shows that the exploration of concurrency control protocols is still midway.


==> tmp/src/tictoc_repro.tex <==
The experimental results are shown in Figs.~\ref{fig:tuple10m_val1k_ycsbC_tps}, \ref{fig:tuple10m_val1k_ycsb_medium_tps}, and \ref{fig:tuple10m_val1k_ycsb_high_tps}.
{\rm TicToc} uses {\sf NoWait} optimization instead of {\sf NoWaitTT}\footnote{Hereafter, we denote {\rm TicToc} that adopts the {\sf NoWait} instead of {\sf NoWaitTT} in the rest of this paper.}.
%When a write lock collision is detected, the transaction aborts and retries.
{\rm Torg} is the original TicToc including using all the optimizations including {\sf NoWaitTT}.
{\rm T+BO} is {\rm TicToc} with {\sf AdaptiveBackoff}.

Fig.~\ref{fig:tuple10m_val1k_ycsbC_tps} shows that Silo and TicToc show comparable performance for read-only workloads, and it is consistent with the results shown in Fig.~6 in the original paper.
In Fig.~\ref{fig:tuple10m_val1k_ycsb_medium_tps}, Silo and TicToc both scale in performance.
This is also consistent with the results shown in Fig.~7 in the original paper.
% Silo shows a performance of about 4 M tps, and the performance of TicToc shows a slightly lower performance.
% DBx1000
The results for DBx1000 are also shown in the figures, and their behavior is similar to that of CCBench.
DBx1000 outperforms CCBench, and we consider it is due to the access methods.
Hash index is used for DBx1000 while masstree is used for CCBench, and hash indexes are typically faster than tree indexes.
%
We confirmed that CCBench without index demonstrates 30\% higher performance (39.6 Mtps) than that of DBx1000 (30 Mtps).
It is already known, but we again claim the effect of the access method should be considered for a fair comparison.


==> tmp/src/tmp/related_core.tex <==
{\sf

Yu et al.~\cite{yu2014staring} evaluated concurrency control protocols with one thousand cores.
The protocols are three 2PLs and four T/Os.
As for the benchmarks, YCSB and TPC-C are used.
Throughputs and the breakdown of execution time are shown.
Five recent protocols evaluated in this paper~\cite{tu2013speedy}~\cite{kim2016ermia}~\cite{wang2016mostly}~\cite{yu2016tictoc}~\cite{lim2017cicada} were not included.
Wu et al.~\cite{wu2017empirical} empirically evaluated MVCC protocols.
They discussed the theory and techniques superior in some workload situations.
They focused on MVCC and did not evaluate SVCC protocols proposed recently~\cite{wang2016mostly}~\cite{tu2013speedy}~\cite{yu2016tictoc}~\cite{lim2017cicada}
Harding et al.~\cite{10.14778/3055540.3055548} evaluated distributed concurrency control protocols.
No distributed protocols are evaluated in this paper.

Platforms to evaluate transaction processing are important and have been studied.
It includes Trireme~\cite{trireme}, Shore-MT~\cite{10.1145/1516360.1516365}, DBx1000~\cite{dbx1000} and Peloton~\cite{peloton}.
The evaluations of these studies provide users mainly a way to investigate the scalability of protocols, which is significant today for increasing CPU cores.
On the other hand, none of them does not care varying workload parameters at a highly parallel environment.
This paper fixes the number of worker thread to 224, and provides analysis with varying other parameters: skew, payload size, transaction size, and cardinality.
%
Besides, this paper enables to apply optimization techniques to all the protocols even though it has not been applied in the original paper.
%
}


==> tmp/src/tmp/repro-proofread.tex <==
\subsection{Reproduction of Prior Work}
	
When evaluating concurrency control protocols, the performance of protocols should be compared under fair conditions.
The meaning of fairness may vary depending on contexts, and we think the following two conditions should be satisfied for a fair comparison.

{\bf Fairness Condition 1.}
Basic modules should be shared: The base modules of an evaluation platform should be shared.
Access methods (e.g., Masstree) and local datasets (read and write sets) need to be shared among protocols.
The effects of memory allocator should be eliminated as much as possible.
The workload should be generated in the same way.
This is important because the performance of a protocol depends on not only the design principle but also engineering details.
The performance of modern protocols is deeply related to the exploitation of underlying hardware, and thus they are sensitive to engineering details.

This above fairness condition may not clearly be satisfied in some cases.
In some papers, we see comparison protocols are not implemented by the authors.
Section 4.2 in Cicada paper [16] states, ”Cicada and existing schemes in DBx1000 share the benchmark code, but have separate data storage and transaction processing engines.”. 
n MOCC paper [27], pure OCC, MOCC, PCC (2PL variants) implementation uses FOEDUS, Dreadlock/WaitDie/BlindDie (2PL variants) uses Orthrus and ERMIA implementation uses ERMIA system.
Three benchmark systems are mixed, In ERMIA paper [14], Silo implementation uses the Silo system while the SI/SSI use the ERMIA system, and the two benchmark systems are mixed.
In these cases, a huge amount of effort by experts is required to avoid unfair comparison.
Such activity is hard for non-experts. Then, we say our fairness condition 1 is not satisfied with their cases.

Wu et al. [29] use the same platform for comparing multiple multi-version protocols, which satisfies the fairness condition 1.
Design philosophy on the platform of CCBench is similar to them.
Their work focuses on evaluating multi-version protocols, and some modern protocols (Cicada, ERMIA, Silo, TicToc, MOCC) are out of scope there.
Yu et al. [30] developed an evaluation platform DBx1000 using a CPU simulator to clarify the scalability impediments of the protocols.
DBx1000 can simulate environments with up to 1024 cores.
Of the seven protocols they targeted, our targets share 2PL, Silo, and TicToc.
On the viewpoint of fairness condition 1, our philosophy is relevant to that of them.

{\bf Fairness Condition 2.}
Applicable optimization techniques should be applied: A protocol consists of a basic method and optimization technique(s).
Sometimes, an optimization technique can be integrated into other basic methods even if a protocol P does not include the optimization technique O at the time of proposal, O can be applied P.
For example, RapidGC is proposed by Cicada [16], and it can be applied to both SI and ERMIA.
NoWait in the validation phase of OCC is proposed by TicToc [31], and it can be applied to Silo.

We think each protocol should be compared with others in the best condition from the viewpoint of fair evaluation.
As described above, the performance of a protocol highly depends on engineering details, and thus applying optimization techniques can improve performance.
One may think such additional optimizations are only laborious and rarely improve performance.
One may have an objection.
By applying an optimization technique to non-original basic methods, the protocol is different from the original one.
However, the application of optimization techniques often improves performance, and we think each protocol should take its best
form in this paper.

Our fairness condition 2 is not satisfied sometimes.
TicToc [31] does not apply NoWait to Silo.
Cicada [16] does not apply RapidGC to ERMIA(SI + SSN) and Hekaton.
Cicada also does not apply adaptive backoff to all protocols used by evaluations in the original paper.

3.2
A Platform for Fair Comparison

We developed CCBench, an evaluation platform for in-memory concurrency control protocols that satisfies the above fairness conditions.
CCBench is publicly available on GitHub [1].
The architecture of CCBench is illustrated in Fig. 1.
To satisfy fairness condition 1, all worker threads in CCBench run in a single node, and it shares the same address space.
Clients and a server run in the same process.
CCBench standardizes the workload generation method.
Client operations (read/write) are generated online.
The generation task is combined with worker threads.
For each transaction execution, workload generation based on the workload setting given before the experiment is performed.
The generated workload information is stored in the STL container, and its memory space reused throughout the experiment.
Allocated memories for a local data structure (read/write set) will be reused for the next transaction, so this improves performance by avoiding memory manager overhead.
We placed record data and concurrency control metadata on the same cache-line.

To fairly provide access methods for protocols in CCBench, all protocols use Masstree [17].
We implemented wrappers for the original implementation [3].
CCBench uses mimalloc [4] for a memory allocator.
We conducted memory allocation evenly in all sockets by using the Linux numactl command for stable results in experiments.
CCBench supports the Yahoo! Cloud Serving Benchmark (YCSB) [9] with flexible configurations on six parameters shown in Table 1.
CCBench currently focuses on read and write operations only, and insert and delete operations are out of scope, which is left as future work.
To determine the skew, CCBench uses a fast approximation method [10].

To satisfy fairness condition 2, CCBench provides seven optimization techniques, as shown in Table 2.
(1) Distributed counter: mitigating simultaneous accesses to a shared single counter.
(2) Invisible read: a read operation that does not pollute the cache memory.
(3) Version inlining: allocating space to keep versions in the record header.
(4) NoWait: immediate abort when detecting a conflict.
(5) Extra Read: retry of the read operation in optimistic protocols.
(6) Adaptive backoff: artificial delay before restarting an aborted transaction.
(7) RapidGC: frequently updating timestamp watermark for garbage collection in multi-version protocols.
CCBench enables additional optimization techniques to 2PL, Silo, TicToc, SI, ERMIA, and Cicada.

It should be noted that CCBench does not support read-only optimization techniques introduced in Silo, FOEDUS, MOCC, and ERMIA.
This is because this optimization improves performance in a specific case (i.e., 99\% read-only transactions, 1\% write transactions, skew at 0.99), and such a workload does not appear in this paper

3.3 Implementing Optimization Techniques
2PL: For efficiency, we implemented the reader/writer lock system used in the protocol from scratch.
Silo: We padded the global epoch (64 bits) into the cache line size (64 bytes) to reduce cache pollution that can be caused by the global epoch state change.
The calculation of commit tid is computationally expensive since it requires loops for both the read set and the write set.
We reduced these two loops by calculation at write lock acquisition and read verification, which leads efficiency.

ERMIA: We adopted the latch-free SSN to avoid expensive SSN serial validation.
This implementation avoided the validation from being a critical section.
We implemented the leveraging existing infrastructure that integrates pstamp and sstamp to reduce memory usage.
We optimized the transaction mapping table.
In a straightforward way, the mapping table is designed as a two-dimensional global array with a thread number, TID, cstamp, and last cstamp, which requires a lock manager for updates and read over the rows.
This clearly causes performance degradation due to serialization and cache pollution.
Therefore, we design a data structure that expresses the rows in a one-dimensional array so that it can be latched with a single atomic compare-and-swap (CAS) operation, and performance was improved by avoiding serialization and cache pollution for row element access.
In our ERMIA implementation, we adopted rapid garbage collection (RapidGC) in Cicada.
CASed transaction mapping table objects and version objects are garbage collected based on calculating a threshold that is not accessed by other workers.
The transaction mapping table object exploits our aggressive version reuse described later in this section, and the load on the memory manager is almost eliminated.

TicToc: We implemented all the three optimization methods (no-wait locking in the validation phase, preemptive aborts, timestamp history).
We also improved the algorithm 5 in the original paper by removing redundant read timestamp updates.
It should be noted that if the recorded read timestamp and updating value is the same, there is no need to perform it.

MOCC: In the original paper, MOCC periodically resets temperature information.
This approach changes many cache lines to the invalid state simultaneously, and performance deteriorates.
We instead perform temperature management only for the record that caused read validation failure.
When resetting the temperature, the epoch at that time is added to the temperature information.
At the time of temperature control, the epoch at that time is compared with the epoch attached to the temperature information.
If the epoch is different, we reset the temperature information.
Therefore, the performance was improved by reducing the cache pollution cost and the resetting cost while finely controlling the temperature.
We did not implement MQL lock since our environment has only 4 NUMA nodes, and its novel effect would be limited.
We instead used the reader/writer lock that is also used by 2PL implementation.

Cicada: We implemented all the six optimization techniques (sort write set by contention, pre-check version consistency, adaptive backoff, early aborts, rapid garbage collection, and best-effort inlining).
In addition, we fixed a logical bug, which is the incomplete version consistency check in the validation phase.
The original paper only confirms that the read version is still the visible version.
However, it needs to check if it is the latest visible version too.
If a newer version exists in the observation range, it means that it should have been read and the transaction view will be broken.

As for the one-sided synchronization, we turned off it to provide higher efficiency.
Aggressive Version Reuse for MVCC: In multi-version protocols (SI, ERMIA, and Cicada), some operations such as creating new versions and deleting old versions provide a load on the memory manager, which also true for memory managers with thread-local memory pools.
So, we worked on a new optimization method, aggressive version reuse that avoids overloading the memory manager in multi-version protocols.
By using the aggressive version reuse, each worker thread maintains a container for future version reuse.
When garbage collection occurs, collected versions are stored in this container.
When a new version is requested, it is taken from this container if this container is not empty.
Otherwise, it requests a memory space to the memory manager as usual.
As an optimization in our experiment, our system expects the necessary memory space for the first garbage collection in advance, and it allocates
them in advance. By this optimization, our multi-version protocols put almost no burden on the memory manager.

3.4 Reproduction of Prior Work
Before introducing the result of the evaluation, we need to validate the correctness of CCBench implementation.
We demonstrate that CCBench successfully reproduces the experimental result in some of the prior work.

3.4.1 MOCC
The first reproduction is MOCC [27].
The MOCC we implemented has two differences, as described in Section 3.3.
In order to confirm the graph shown in the original paper can be reproduced by our implementation, we conduct an experiment with the settings shown in Figs 6 and 7 of the original paper.
The settings are also described in the graph caption.
The experimental results are shown in Fig. 2a that the performance scales with the number of threads in the read-only workload.
It reproduces the result of Fig. 6 in the original paper.
The reason is that there is no interaction between threads.
The reason why the performance improvement rate deteriorates after 112 threads is that there
are only 112 physical cores, and the reason that the MOCC performance is slightly lower than Silo is that there is a new calculation process.
On reading, MOCC calculates the temperature information address.
Also, it performs a process for determining whether the temperature is high, which requires memory access.
This process that not exist in Silo, and it may differentiate their results.
The results shown in Figs. 2b and 2c show that when the write rate increases from 0\% to 10\%, the abort rate rapidly increases, and the performance deteriorates.
This experiment is the reproduction of Fig. 7 in the original paper.
The reason is that write operation produces a large amount of the read validation failures.
In Figure 2b, the performance of Silo deteriorates at a write rate of 0-40\%, but the performance improves at a write rate of 40-60\%.
This is a trade-off between reduced read/write contentions due to reduced write operations and frequent read validation failures due to increased read operations.
Compared to that, MOCC shows stable performance, which is considered to progress steadily by temperature control.

3.4.2 TicToc
The second reproduction is TicToc [31].
To confirm our implementation can reproduce the graph shown in the original paper, we experiment with the settings shown in Figs 6, 7, and 8 of the original paper.
The details of the workload are also described in the graph caption.
We set epoch interval long so that it does not to occur cache line contentions in Silo.

Figure 3a shows that Silo and TicToc show comparable performance in read-only workloads, exceeding 20 M tps, which is consistent with Fig. 6 in the original paper.
In Figure 3b, Silo and TicToc both scale in performance.
This is also consistent with Fig. 7 in the original paper.
On the other hand, we found an impressive result.
In Fig. 3c, TicToc shows different performances from Fig. 8 in the original paper.
The performance of TicToc improves as the number of threads increases, but when the number of threads exceeds a specific number, the performance starts
to deteriorate due to an increase in read/write contention.
Therefore, in the original paper, we considered the possibility of a sort of optimization on TicToc and tried to introduce Cicada backoff optimization.
This is shown as TicToc + BO in Fig. 3c.
In our environment, TicToc + BO showed a similar performance curve of TicToc to that of Fig. 9 in the original paper.
The third reproduction is Cicada [16].
The workload was set almost the same as the original paper.
The details of the workload also are described in the graph caption.
The differences from the original paper and here are as follows: 
(1) Redesign and reimplementation of all protocols by authors.
(2) The backoff optimization that Cicada has is installed in all protocols because this optimization technique can be implemented without using Cicada, and we found it is effective for improving performance.

Figures 4a, 4c, 4b, and 4d illustrate the experimental results.
All the results showed the same tendency as the original paper (Figs 6 and 7).
As a result of applying the backoff optimization techniques fairly to all protocols, MOCC or TicToc won over almost all the given parameters,
which is inconsistent with the original paper.
Evaluation on the original paper compared different systems.
Therefore, it is considered that different designs and implementations between the systems affected the performance in the evaluation of the original paper.


==> tmp/src/tpcc.tex <==
%\color{blue} %REVISED_COLOR_BEGIN
%To evaluate protocols at a highly parallel environment, TPC-C benchmark is not suitable.
%
Since the purpose of this paper is to identify factors that greatly affect performance in a highly parallel environment (i.e., 224 threads) with high resource contention and/or many read/write conflicts, we did not use the TPC-C benchmark for investigating the factors.
%
Without using TPC-C, we managed to clarify the relationships between three major performance factors and several optimization methods and to identify three two optimization methods described above.
%First, the TPC-C workload has low-contention and low-conflict~\cite{wang2016mostly}. Although this workload is suitable for our purpose, it has been used in conventional studies~\cite{trireme,wu2017empirical,dbx1000}.
%
%Second, the only configurable parameters in TPC-C are the warehouse and the number of threads, which are insufficient for exploring performance factors in a variety of situations. We need a set of parameters that can generate various situations.
%
\color{blue} %REVISED_COLOR_BEGIN
Beyond the purpose of this paper, it is important for a benchmark system to support TPC-C because it models a retail operation and is the current industry standard to evaluate transaction processing systems~\cite{tpcc}. 
%
CCBench currently supports TPC-C benchmark partially.
Among protocols, CCBench supports only Silo.
CCBench supports only two (Payment and NewOrder) out of five transctions in TPC-C.
%
The details are described in Appendix.
\color{black} %REVISED_COLOR_END


==> tmp/src/unknown.tex <==
\section{New Performance Factor}
\input{src/delay}
\input{src/version-lifetime-control}


==> tmp/src/version-lifetime-control.tex <==
\section{Analysis of Version Lifetime}
\label{sec:version-lifetime-control}
\input{src/version-lifetime-control_figure}

The life of a version begins when it is created by a corresponding write operation.
The version state is called {\bf visible} during the period when other transactions can read it.
Otherwise, the version state is called {\bf non-visible}.
Recent CC protocols typically make the version visible at the pre-commit phase~\cite{aether,tu2013speedy}.
After a certain period, the life of the version ends, and it is made non-visible.
SVCC protocols typically make a version by overwriting its previous version,
with the former becoming visible and the latter becoming non-visible at the same time.
MVCC protocols typically make a version on a different memory fragment from other visible versions of the same record, so their life does not end unless GC works.

\subsection{Confirming Overhead of Versions}
\label{sec:problem-many-visible-versions}
The performance of MVCC is thought to suffer from the existence of many visible versions~\cite{10.14778/2095686.2095689,10.1145/2723372.2749436}.
%
Many visible versions leads to a significant burden due to memory exhaustion or an increase in cache-line replacements for traversal or installation.
MVCC protocols can provide higher performance than SVCC ones due to their larger scheduling spaces.
It should be noted that architectural issues sometimes negate the benefits, as mentioned in $\S$ \ref{sec:changing_database_size}.
%
We analyzed this situation in depth.
Please note that the cost for allocating new pages is negligible in the result below since our {\sf AssertiveVersionReuse}($\S$\ref{sec:A Platform for Fair Comparison}) conducts the space allocation before experiments.

MVCC protocols often demonstrate their novel performance compared with SVCC protocols for high contention workloads.
% 
To begin, we measured the throughput for various degrees of skew (0 to 0.99) as shown in Fig.~\ref{fig:comp_tuple100m_skew0-099}.
Here we focus on the difference between Cicada (MVCC) and Silo (SVCC).
In Figs.~\ref{fig:comp_ycsbA_tuple100m_skew0-099_tps} and \ref{fig:comp_ycsbA_tuple100m_skew0-099_ar} for YCSB-A, Cicada outperforms Silo when the skew is higher than 0.8.
% 
The larger the payload, the greater the superiority of Cicada.
%
This is attributed to Cicada having larger scheduling spaces than Silo;
%
nevertheless, these results confirm that the performance of MVCC suffers from having many versions~\cite{10.14778/2095686.2095689,10.1145/2723372.2749436}.
%
In Figs.~\ref{fig:comp_ycsbB_tuple100m_skew0-099_tps} and \ref{fig:comp_ycsbB_tuple100m_skew0-099_ar} of YCSB-B, Cicada always underperforms Silo, TicToc, and MOCC.

% Micro analysis
To clarify the reason, we analyze the characteristics of versions.
The larger scheduling spaces are supported by many versions, and they can be an overhead.
This overhead in modern protocols remains to be analyzed.
%
We show the latency breakdown with a skew of 0, where MVCC is disadvantageous, in Fig.~\ref{fig:latency_breakdown_tuple100m_skew0}.
In Figs.~\ref{fig:comp_cicada-silo_ycsbA_tuple100m_gci10us_224th_main-latency} and ~\ref{fig:comp_cicada-silo_ycsbB_tuple100m_gci10us_224th_main-latency},
we can see that the major overhead of Cicada lies in the read and write operations rather than validation or GC.
%
To clarify the reasons for the overhead, we designed a SVCC version of Cicada, Cicada-SV, that overwrites the inline versions of Cicada.
This eliminates the need to allocate new areas, so Cicada-SV performs like a SVCC protocol.
%
We prepared the special workload in which transactions are completely partitioned to avoid contentions because Cicada-SV does not cope well with contentions.
The result is illustrated in Fig.~\ref{fig:latency_breakdown_tuple100m_skew0_cicada-sv}.
The latencies of Cicada-SV and Silo are almost the same.
We attribute that the overhead of Cicada shown in Figs.~\ref{fig:comp_cicada-silo_ycsbA_tuple100m_gci10us_224th_main-latency} and \ref{fig:comp_cicada-silo_ycsbB_tuple100m_gci10us_224th_main-latency} to the cost of version chain traversal and the increase in cache misses.

Since having many visible versions degrades performance, reducing the number should improve performance.
{\sf RapidGC} optimization effectively mitigates this problem.
To confirm its efficiency, we varied the interval setting and measured the throughput of Cicada.
Fig.~\ref{fig:comp_cicada-ninline_ycsbA_tuple1m_gci1us-1s_tps} of legend 0 illustrates high throughput is obtained when the interval is no more than 100 us as reported elsewhere ~\cite{lim2017cicada,wu2017empirical}.
%
This is because the number of visible versions is small, and most of them are kept in cache.
So, can {\sf RapidGC} with its short intervals perform efficiently for any workloads? The answer is no. We explain why in $\S$ \ref{sec:limitation-of-current-approaches}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

\underline{\bf Insight 5:~}
The overhead of multi-version management cannot be negligible.
Silo and TicToc outperformed Cicada for high skew (0.99), read-intensive (YCSB-B), non-RMW and, high cardinality (100 M records) cases.
%
A study~\cite{lim2017cicada} reported that all of them exhibit the same performance for a similar workload in Fig.~7 (skew 0.99, read 95\%, RMW, 10 M records, payload 100 byte).
The inconsistency is due to the use of multiple different platforms in \cite{lim2017cicada}.
%
Using a single platform, we observed the difference and found that version management cost of Cicada is not negligible even for a low contention case
as shown in Fig.~\ref{fig:comp_cicada-silo_ycsbA_tuple100m_gci10us_224th_main-latency} and \ref{fig:comp_cicada-silo_ycsbB_tuple100m_gci10us_224th_main-latency}.
%
It is difficult to find deep knowledge using multiple different reference implementations or platforms,
and the deep analysis of CC protocols must be done on the same platform.
%

\subsection{Limit of Current Approach}
\label{sec:limitation-of-current-approaches}
We investigated the behavior of {\sf RapidGC} using the same workloads as in our third experiment with a long transaction.
%
Even state-of-the-art GC does not sufficiently reduce the number of visible versions if there is only a single long transaction.
This is because modern protocols assume that transaction execution is one-shot, and that the transactions are relatively small (e.g. 16 for YCSB).
%
Long transactions except read-only ones have been ignored in modern transaction studies.
%

To generate a long transaction, we added an artificial delay at the end of the read phase of them.
Both the long and short transactions use the same number of operations with the same read-write ratio.
Only one worker thread executes a long transaction,
and the remaining worker threads execute the short transactions.
The skew is set to 0 so that contentions in record accesses rarely occur and do not affect performance,
even if there exists such a long transaction.

We measured the performance of Cicada under the workload described above, varying the {\sf RapidGC} interval settings and the delay of a long transaction.
Fig.~\ref{fig:comp_cicada-ninline_ycsbA_tuple1m_gci1us-1s_tps} shows the results.
%
All the results in the figure with delays had saturated their performances. The saturation points were exactly when the GC intervals are the same as the delays of the a long transactions.
%
For example, the light blue line includes a long transaction with a $1$ ms delay, and its performance saturates when the GC interval is $1$ ms.
% 
Similar behaviors were observed with larger delays.
%
This is because current GC methods do not collect visible versions that may be read by active long transactions.
%
The current GC scheme does not allow collecting the versions until the transaction finishes.
We consider that this limitation is the primary hurdle in improving MVCC performance by reducing the number of visible versions.
%
We could not obtain a result for a 1 s delay because such a delay requires a huge amount of memory, which causes the Linux OOM (out-of-memory) killer to kill the process.

\subsection{Aggressive Garbage Collection}
\label{sec:discussion-towards-version-lifetime-control}
From the limitation of current GC scheme described in $\S$ \ref{sec:limitation-of-current-approaches},
we suggest a novel GC scheme, {\sf AggressiveGC} that aggressively collects versions beyond the current one to deal with long transactions.
%
An example of such a protocol is to integrate MVTO protocol with a GC method that aggressively collects visible versions.
Using the protocol, some versions are made non-visible even though active or future transactions need to read them.
Such a protocol may incur read operation failures unlike conventional MVTO, and needs to handle such a case by aborting the transaction and retrying it with a new timestamp.
%
Restricting the number of versions has been discussed in kVSR~\cite{10.5555/645478.654954} or 2V2PL~\cite{10.1145/320141.320146,10.1145/582318.582330}.
They keep only the latest contiguous versions and less flexible than our suggestion.
We suggest the visible versions do not need to be contiguous, and the number of versions can be flexible in contexts.
%
An interesting topic in this scheme is the risk of starvation.
One way for the mitigation can be the management of priorities among transactions such as wait-die~\cite{10.1145/320251.320260}, and this topic has not yet been discussed in modern MVCC studies.

We suggest two optimizations for write operations in terms of the aggressive protocols.
%
The first is version overwriting that creates a new version by overwriting the memory segment of an old version, which becomes non-visible at the same time, like that used in SVCC protocols.
Version overwriting is efficient because two operations are combined into one operation.
%
The second is non-visible writes that make versions non-visible from the beginning of their life.
The idea of non-visible writes was originally proposed as the Thomas write rule~\cite{10.1145/320071.320076} and recently generalized as the non-visible write rule (NWR)~\cite{nakazono2019invisiblewriterule} to deal with blind writes.
%We have a chance to develop novel protocols and optimization techniques on version lifetime control to improve MVCC protocols.
Novel protocols and optimization techniques based on version lifetime control are a promising way to improve MVCC protocols.

%\color{blue} %REVISED_COLOR_BEGIN
\underline{\bf Insight 6:}~
Even state-of-the-art GC cannot hold down the number of versions in MVCC protocols if a single long transaction is mixed into the workload.
An aggressive approach can solve this problem by aggressively changing the version state to non-visible for both reads and write, even though the state is still required by transactions.
%\color{black} %REVISED_COLOR_END


==> tmp/src/version-lifetime-control_figure.tex <==
%
% 
%
\begin{figure*}[tb]
\begin{tabular}{cccc}
\begin{minipage}{0.23\hsize}
\subcaptionbox{YCSB-A Throughput \label{fig:comp_ycsbA_tuple100m_skew0-099_tps}}
{\includegraphics[scale=0.9]{fig/version-lifetime-control/comp_ycsbA_tuple100m_skew06-099_tps.pdf}}
\end{minipage}
&
\begin{minipage}{0.23\hsize}
\subcaptionbox{YCSB-A Closing up High Skew \label{fig:comp_ycsbA_tuple100m_skew0-099_ar}}
{\includegraphics[scale=0.9]{fig/version-lifetime-control/comp_ycsbA_tuple100m_skew09-099_tps.pdf}}
\end{minipage}
&
\begin{minipage}{0.23\hsize}
\subcaptionbox{YCSB-B Throughput \label{fig:comp_ycsbB_tuple100m_skew0-099_tps}}
{\includegraphics[scale=0.9]{fig/version-lifetime-control/comp_ycsbB_tuple100m_skew06-099_tps.pdf}}
\end{minipage}
&
\begin{minipage}{0.23\hsize}
\subcaptionbox{YCSB-B Closing up High Skew \label{fig:comp_ycsbB_tuple100m_skew0-099_ar}}
{\includegraphics[scale=0.9]{fig/version-lifetime-control/comp_ycsbB_tuple100m_skew09-099_tps.pdf}}
\end{minipage}
\end{tabular}
\caption{Impact of workload skew: 100M records, 224 threads, payload 4 bytes, 10 ops/trans.}
\label{fig:comp_tuple100m_skew0-099}
	\end{figure*}

%
%
%
\begin{figure}[tb]
\begin{tabular}{cc}
\begin{minipage}{0.45\hsize}
\subcaptionbox{YCSB-A \label{fig:comp_cicada-silo_ycsbA_tuple100m_gci10us_224th_main-latency}}
{\includegraphics[scale=0.9]{fig/version-lifetime-control/comp_cicada-silo_ycsbA_tuple100m_gci10us_224th_main-latency.pdf}}
\end{minipage}
&
\begin{minipage}{0.45\hsize}
\subcaptionbox{YCSB-B \label{fig:comp_cicada-silo_ycsbB_tuple100m_gci10us_224th_main-latency}}
{\includegraphics[scale=0.9]{fig/version-lifetime-control/comp_cicada-silo_ycsbB_tuple100m_gci10us_224th_main-latency.pdf}}
\end{minipage}
\end{tabular}
\caption{Latency breakdown: skew 0, 100M records, 224 threads, payload 4 bytes, 10 ops/trans.}
\label{fig:latency_breakdown_tuple100m_skew0}
\end{figure}

%
%
%
\begin{figure}[tb]
\begin{tabular}{cc}
\begin{minipage}{0.45\hsize}
\subcaptionbox{YCSB-A \label{fig:comp_cicada-silo-part_ycsbA_tuple100m_gci10us_224th_main-latency}}
{\includegraphics[scale=0.9]{fig/version-lifetime-control/comp_cicada-silo-part_ycsbA_tuple100m_gci10us_224th_main-latency.pdf}}
\end{minipage}
&
\begin{minipage}{0.45\hsize}
\subcaptionbox{YCSB-B \label{fig:comp_cicada-silo-part_ycsbB_tuple100m_gci10us_224th_main-latency}}
{\includegraphics[scale=0.9]{fig/version-lifetime-control/comp_cicada-silo-part_ycsbB_tuple100m_gci10us_224th_main-latency.pdf}}
\end{minipage}
\end{tabular}
 \caption{Latency breakdown of Cicada-SV and Silo under a partitioned workload. The other setting is the same as Fig. 12}
\label{fig:latency_breakdown_tuple100m_skew0_cicada-sv}
\end{figure}


%
% long tx
%
\begin{figure}[t]
  \centering
  \includegraphics[scale=1.0]{fig/version-lifetime-control/comp_cicada-ninline_ycsbA_tuple1m_gci1us-1s_tps.pdf}
  \caption{Analysis of RapidGC: YCSB-A, skew 0, 224 threads, 1M records, payload 4 bytes, 10 ops/trans.
Each legend indicates the inserted delay of long transactions.}
  \label{fig:comp_cicada-ninline_ycsbA_tuple1m_gci1us-1s_tps}
\end{figure}



==> vldb_format/header.tex <==
\usepackage{graphicx}
\usepackage{balance}  % for  \balance command ON LAST PAGE  (only there!)
\usepackage{caption}
\usepackage{subcaption}
\usepackage{ascmac}

% It should be used on writing.
\usepackage{color}

% It is required to use \url in bibliography for arXiv.
\usepackage{url}

% Include information below and uncomment for camera ready
\vldbTitle{An Analysis of Concurrency Control Protocols for In-Memory Database with CCBench.}
\vldbAuthors{Takayuki Tanabe, Takashi Hoshino, Hideyuki Kawashima, Osamu Tatebe.}
\vldbDOI{https://doi.org/10.14778/xxxxxxx.xxxxxxx}
\vldbVolume{13}
\vldbNumber{46}
\vldbYear{2020}

\begin{document}
% ****************** TITLE ****************************************

\title{An Analysis of Concurrency Control Protocols\\ for In-Memory Database with CCBench}

% possible, but not really needed or used for PVLDB:
%\subtitle{[Extended Abstract]
%\titlenote{A full version of this paper is available as\textit{Author's Guide to Preparing ACM SIG Proceedings Using \LaTeX$2_\epsilon$\ and BibTeX} at \texttt{www.acm.org/eaddress.htm}}}

% ****************** AUTHORS **************************************

% You need the command \numberofauthors to handle the 'placement
% and alignment' of the authors beneath the title.
%
% For aesthetic reasons, we recommend 'three authors at a time'
% i.e. three 'name/affiliation blocks' be placed beneath the title.
%
% NOTE: You are NOT restricted in how many 'rows' of
% "name/affiliations" may appear. We just ask that you restrict
% the number of 'columns' to three.
%
% Because of the available 'opening page real-estate'
% we ask you to refrain from putting more than six authors
% (two rows with three columns) beneath the article title.
% More than six makes the first-page appear very cluttered indeed.
%
% Use the \alignauthor commands to handle the names
% and affiliations for an 'aesthetic maximum' of six authors.
% Add names, affiliations, addresses for
% the seventh etc. author(s) as the argument for the
% \additionalauthors command.
% These 'additional authors' will be output/set for you
% without further effort on your part as the last section in
% the body of your article BEFORE References or any Appendices.

\numberofauthors{4} %  in this sample file, there are a *total*
% of EIGHT authors. SIX appear on the 'first-page' (for formatting
% reasons) and the remaining two appear in the \additionalauthors section.

\author{
% You can go ahead and credit any number of authors here,
% e.g. one 'row of three' or two rows (consisting of one row of three
% and a second row of one, two or three).
%
% The command \alignauthor (no curly braces needed) should
% precede each author name, affiliation/snail-mail address and
% e-mail address. Additionally, tag each line of
% affiliation/address with \affaddr, and tag the
% e-mail address with \email.
%
% 1st. author
\alignauthor
Takayuki Tanabe\titlenote{Work done while at University of Tsukuba}\\
       \affaddr{NAUTILUS Technologies, Inc}\\
       \email{tanabe@nautilus-technologies.com}
% 2nd. author
\alignauthor
Takashi Hoshino\\
       \affaddr{Cybozu Labs}\\
       \email{hoshino@labs.cybozu.co.jp}
% 3rd. author
\alignauthor
Hideyuki Kawashima\\
       \affaddr{Keio University}\\
       \email{river@sfc.keio.ac.jp}
\and  % use '\and' if you need 'another row' of author names
% 4th. author
\alignauthor
Osamu Tatebe\\
       \affaddr{University of Tsukuba}\\
       \email{tatebe@cs.tsukuba.ac.jp}
}
% There's nothing stopping you putting the seventh, eighth, etc.
% author on the opening page (as the 'third row') but we ask,
% for aesthetic reasons that you place these 'additional authors'
% in the \additional authors block, viz.
%\additionalauthors{Additional authors: John Smith (The Th{\o}rv\"{a}ld Group, {\texttt{jsmith@affiliation.org}}), Julius P.~Kumquat
%(The \raggedright{Kumquat} Consortium, {\small \texttt{jpkumquat@consortium.net}}), and Ahmet Sacan (Drexel University, {\small \texttt{ahmetdevel@gmail.com}})}
%\date{1 March 2020}
% Just remember to make sure that the TOTAL number of authors
% is the number that will appear on the first page PLUS the
% number that will appear in the \additionalauthors section.



==> vldb_format/src/abst.tex <==
\begin{abstract}
 This paper proposes yet another concurrency control analysis platform CCBench.
 CCBench offers seven protocols and seven optimization methods, and enable to configure seven workload parameters.
%
 We analyzed the protocols and optimization methods varying the parameters fixing the number of worker threads to 224 while conventional studies focus on scalability.
% takeaway
 Through the analysis using CCBench, we first revealed the relationship between the performance factors and the optimization methods.
%
 The key factors were CPU cache, delay, and version lifetime.
%
 The cache is related to the distributed counters, invisible read, and version inlining.
%
 The delay is related to NoWait, backoff.
%
 The version lifetime is related to rapid garbage collection.
%
 We then found two new candidates of optimization methods.
%
 From the extra read, we suggest the read phase extension method that is classified into the delay control.
 It exploits local conflict information while ordinary delay control methods rely on global information.
%
 From the limit of rapid garbage collection that deteriorates performance in the presence of a single long transaction, we suggest the aggressive-GC that is classified into the version lifetime factor.
 It collects non-obsolete versions to deal with the long transaction problem requiring to change the read protocol.
%Such tight communication requires the integration of protocol and GC.
% public
The code of CCBench and all the data in this paper are publicly available.

 \if 0
 In recent years, excellent concurrency control protocols have been proposed for in-memory database systems.
 Each protocol presents various optimization techniques for high performance by adjusting performance factors, implicitly and explicitly.
 We believe a platform for fair and flexible evaluation is essential to organize the relationship between the performance factors and the optimization techniques.
  For this purpose, we present a platform CCBench that provides a way to evaluate the protocols by flexibly adjusting a variety of optimization techniques and workload settings: skew, payload size, transaction size, carnality, read ratio, and write model.
  CCBench is publicly available on GitHub.
  In CCBench, we implemented seven protocols: 2PL, Silo, MOCC, TicToc, ERMIA, Cicada, and snapshot isolation.
  Using CCBench, we can apply a variety of techniques to protocols to improve performance even if the original papers do not conduct them, and we clarify three performance factors for concurrency control protocols and analyze the effects of optimization techniques for them.
  The first factor is the CPU cache.
  Distributing centralized counter mitigates cache line , and invisible reads reduce cache pollution.
  The second factor is the delay with conflicts.
 In addition to known techniques such as NoWait and adaptive back off optimizations, we found the extra reads that occur in optimistic protocols mitigate access concentration to records.
 The third factor is version lifetime in multi-version protocols.
  RapidGC is effective for harnessing version lifetime while the effect is constrained by the presence of long transactions.  
\fi
\end{abstract}


==> vldb_format/src/ack.tex <==
\section*{Acknowledgments}
We would like to thank Masahiro Tanaka, and the anonymous reviewers for their valuable feedback.
This work is partially supported by JSPS Kakenhi Grant Number 19H04117 and Project commissioned by the New Energy and Industrial Technology Development Organization (NEDO).


==> vldb_format/src/analyzed_space.tex <==
CCBench supports six parameters shown in Table~\ref{tab:Experimental Parameters} and write model (read-modify-write or not).
%
Skew is the access pattern under Zipf distribution.
Cardinality is the number of records in database.
Payload size is the size of a record (key and value).
Transaction size is the number of operations in a transaction.
Read ratio is the ratio of read in a transaction.
Write model is whether read modify write or not.
Thread size is the number of worker threads though it is fixed to 224 in this paper.
%
To determine the skew, CCBench uses a fast approximation method~\cite{gray1994quickly}.
This paper does not deal with insert and delete operations and left them as future work.
%
We analyze CC protocols with 224 threads with CCBench.
Most of benchmarks are YCSB, and some of them are its variants.
The analyzed parameter sets are summarized in Table \ref{tab:Experimental Parameters}.
We vary skew, cardinality, payload size, transaction size, read ratio fixing the thread parallelism to 224.
%
The caption in Table \ref{tab:Experimental Parameters} describes when parameters are varies as \$1 $\ldots$ \$6.

\begin{table}[tb]
 \begin{center}
  \begin{scriptsize}
 \caption{Configurable Parameters in CCBench and Analyzed Space.
   \$1: Cardinality: range from $10^3$ records to $10^9$ records.
   \$2: Cardinality: points $10^3$ records or $10^6$ records.
   \$3: Read ratio: range from 0\% to 100\%.
   \$4: Transaction size: range from 10 to 100.
   \$5: Payload size: range from 4 byte to 1000 byte.
   \$6: Skew: range from 0.6 to 0.99.
   }
 \label{tab:Experimental Parameters}

 \begin{tabular}[tb]{l|cccccc}
  Parameter
  & Fig. \ref{fig:central_tuple1k-1g}
  & Fig. \ref{fig:Analysis of Invisible Read: YCSB, 224 Threads, Payload 4 bytes, Skew 0, 10 ops/trans.}
  & Fig. \ref{fig:Impact of Transaction Size: YCSB-B, 100M Records, 224 Threads, Payload 4 bytes, Skew 0.8.}
  & Fig. \ref{fig:Effect of Delay provided by Extra Read: YCSB-A, 100M records, 224 threads, skew 0.9, 10 ops/trans.}
  & Fig. \ref{fig:comp_tuple100m_skew0-099}\\
 \hline
  Skew            &0   &0   &0.8   &0.9  &\$6 \\
  Cardinality     &\$1 &\$2 &$10^8$&$10^8$&$10^8$\\
  Payload  (Byte) &4   &4   &4     &\$5  &4\\
  Xact Size       &10  &10  &\$4   &10   &10\\
  Read Ratio(\%)  &0,5 &\$3 &50,95 &50   &50,95\\
  \# Threads      &224 &224 &224   &224  &224\\
 \end{tabular}
  \end{scriptsize}
 \end{center}
\end{table}


==> vldb_format/src/appen.tex <==
\begin{appendix}
tbd
\end{appendix}


==> vldb_format/src/cache-proof.tex <==
\section{Effect of Cache}
\label{sec:Cache Effect}

\input{src/analyzed_space.tex}
% Why not tpcc
\input{src/tpcc}

\subsection{Cache Line Conflict}
\label{sec:changing_database_size}
\input{src/cache_figure.tex}

%We set the number of worker threads to 224 in all the experiments below.
%
We first analyze the effect of the centralized data object.
%Modern CPU provides a few hundreds of cores \cite{10.1145/3399666.3399910}, which provides massive parallelism on OLTP.
Some protocols require centralized data structures (e.g., shared counter) \cite{jung2013performance,kim2016ermia} while some others decentralize them \cite{tu2013speedy,yu2016tictoc,wang2016mostly,lim2017cicada}.
%
Here we revisit the effect of the centralized data structure.
The details of the workload are described in the graph caption. 
%
The results are shown in Figs.~\ref{fig:ycsbB_tuple1k-1g}, \ref{fig:ycsbC_tuple1k-1g}, \ref{fig:ycsbB_tuple1k-1g_ar}, and \ref{fig:ycsbC_tuple1k-1g_ca}.
% omit?
The result of YCSB-A have the same trend as those of YCSB-B, so it is omitted.
%YCSB-C is a read-only workload, so the abort rate is 0, and the corresponding result about abort rate is omitted.
%
Fig.~\ref{fig:central_tuple1k-1g} illustrates that the throughput of ERMIA and SI do not scale although their scheduling spaces are wider than that of SVCC serializable protocols.
This is because both protocols depend on a central data object
 %(i.e., a shared counter for the timestamp of both protocols and transaction mapping table of ERMIA), and access to the central data structure
causes the cache line conflict, which in turn causes performance degradation.
%This is consistent with the claims in ~\cite{tu2013speedy, wang2016mostly}.
%\cite{tu2013speedy} describes in Section 5.2 that MemSilo + GlobalTID does not scale because it issues a commit tid with a single shared counter.
%\cite{wang2016mostly} states in Section 5.3 that on large machines such as GryphonHawk, ERMIA 's centralized data structure for inter-thread communications used by SSN becomes a major bottleneck.
%\cite{wang2016mostly} also states that interthread communication impedes scalability in Section 2.2.

%
To investigate the reason of the inefficiency, we measured the throughput of an atomic shared counter incrementation by multiple threads.
The results are shown Figs.~\ref{fig:fetch_add_test_tps} and \ref{fig:fetch_add_test_cm}. 
The cache miss rate is measured using the Linux Perf tool, and it means L3 cache miss rate.
Fig.~\ref{fig:fetch_add_test_tps} shows that one thread exhibits the best performance.
This is because %atomic operations are atomically serialized and
frequent reads/writes to the same memory address by multiple threads cause high conflicts of a cache line.
%The trend in performance degradation of ~\ref{fig:fetch_add_test_tps} shows that cache line contention degrades performance more severely than serialization.
%Therefore, Cache pollution is the primary cause of performance degradation when the centralized data structure is accessed by multiple threads.
Fig.~\ref{fig:fetch_add_test_cm} illustrates that the L3 cache miss that rate increases as the number of threads increases.
%Cache-misses event in perf counts L3 cache misses.
%In the experiment of incrementing one shared counter atomically, the situation that causes L3 cache miss is cache pollution.
Cache line conflicts incur L3 cache misses and longer communication delay if the CPU core requiring the cache line and the another core having it exclusively are running in the different CPU sockets. In the experiment, 28 threads setting used one socket, 56 threads setting used two sockets, 112 or more threads setting used four sockets. Thus larger L3 cache miss rate indicates occurrence of communication among sockets and it significantly deteriorates the performance of fetch\_add. Consequently, centralized counters should be avoided in many-core environments, especially multi-socket ones.
%Thus, a centralized counter incurs not only cache line contentions that blocks other instructions, but also cache misses that require long delay to fetch data from memory, which is not yet widely known.
%
Consequently, centralized objects should be avoided by the above reason.
%When cache pollution occurs, data consistency is managed through the fastest layer of memory hierarchy shared by coordination targets.
%If threads do not share the same physical core but share the same socket, consistency is managed through L3.
%If threads run on different sockets, consistency management is conducted through memory.
%Under 28 threads, all threads coexist in the same physical core, and L3 cache miss for consistency of shared counter does not occur.
%Until threads increase to 112 (28 cores x 4 sockets), the cache pollution frequency increases, and the number of L3 cache misses increases.
%ERMIA has a transaction mapping table as a shared data structure, and SI has a centralized counter to define the start and end points of a transaction.
%Therefore, we consider that the performance of these protocols severely degrades by the cache line conflicts.

\subsection{Cache Line Replacement}
\label{sec:Cache Miss Mitigation}
% YCSB-B result, cache > contention..
After confirming the inefficiency of centralized objects, we discuss the effects of cache line replacement.
We first discuss about YCSB-B result.
In Figs.~\ref{fig:ycsbB_tuple1k-1g} and \ref{fig:ycsbB_tuple1k-1g_ar}, as cardinality increases,
(1) throughput first improves and then deteriorates, and
(2) abort rate monotonically improves.
%
When cardinality is quite low, the footprint of accessible records are also small
so that all of records fit inside L3 cache. However, it is more likely happen contentions at L1 or L2. As cardinality increases, such contentions are alleviated since accessible records increase, and performance improves.
%
It is considered that with more cardinality, the total amount of records start to overflow L3 cache.
It attracts L3 cache misses and consecutive accesses of remote socket cache or DRAM, which degrades performance.
%
%The effect of L3 cache miss is stronger than that of L1/L2 cache misses.

% YCSB-C result, cache > contention..
\input{src/read_only_cache_effect.tex}

\if 0
Here we have a hypothesis.
If the performance of a protocol is strongly affected by cache memory utilization, the location of the data to be accessed is either inside (cache-inside) or outside the cache (cache-outside).
The data location is considered to depend greatly on the cardinality.
If the cardinality is small, the data tends to be within the cache, while in the opposite case, the data is less likely to be within the cache.

This situations are evident from ~\ref{fig:ycsbC_tuple1k-1g} and~\ref{fig:ycsbC_tuple1k-1g_ca}.
If the protocol does not update shared meta data, 
the increase in cardinality degrades the throughput and increases the cache miss rate due to using large memory.
Surprisingly, 2PL, SI, and ERMIA which update shared meta data in the read only workload do not show this trend.
2PL uses reader/writer locks and operating read lock updates the shared status of the data.
SI uses centralized counter to define start and end points.
ERMIA uses transaction mapping table.
In these protocols, as it transits from small records to large records, the throughput first improves and then deteriorates, the cache miss rate first improves and then deteriorates.
The reason is considered as follows.
First, even in YCSB-C (read only), when cardinality is quite low, access items are limited, which more likely provides cache contentions.
Second, as cardinality increases, such contentions are alleviated since access items increase.
However, when cardinality increases to some extent, some records are not fit into cache, and the cache evictions incur performance degradation.

Therefore, the above hypothesis holds.
With the cache-inside workload type, more records provide better performance than cache-outside workloads.
\fi

% Invisible read
\input{src/invisible}


==> vldb_format/src/cache_figure.tex <==
\begin{figure*}[tb]
 \begin{tabular}{cccc}
  \begin{minipage}{0.23\hsize}
   \subcaptionbox{YCSB-B \label{fig:ycsbB_tuple1k-1g}}
   {\includegraphics[scale=0.7]{fig/central/comp_tuple1k-1g_ycsbB_tps.pdf}}
  \end{minipage}
  &
  \begin{minipage}{0.23\hsize}
   \subcaptionbox{YCSB-C \label{fig:ycsbC_tuple1k-1g}}
   {\includegraphics[scale=0.7]{fig/central/comp_tuple1k-1g_ycsbC_tps.pdf}}
  \end{minipage}
  &
  \begin{minipage}{0.23\hsize}
   \subcaptionbox{YCSB-B \label{fig:ycsbB_tuple1k-1g_ar}}
   {\includegraphics[scale=0.7]{fig/central/comp_tuple1k-1g_ycsbB_ar.pdf}}
  \end{minipage}
  &
  \begin{minipage}{0.23\hsize}
   \subcaptionbox{YCSB-C \label{fig:ycsbC_tuple1k-1g_ca}}
   {\includegraphics[scale=0.7]{fig/central/comp_tuple1k-1g_ycsbC_ca.pdf}}
 \end{minipage}
 \end{tabular}
 \caption{Varying Cardinality. Payload 4 bytes, 224 Threads, Skew 0, 10 ops/trans.}
 \label{fig:central_tuple1k-1g}
\end{figure*}

% centralized counter
\begin{figure}[t]
  \begin{tabular}{cc}
    \begin{minipage}{0.45\hsize}
      \subcaptionbox{Throughput. \label{fig:fetch_add_test_tps}}
      {\includegraphics[scale=0.8]{fig/central/fetch_add_tps.pdf}}
    \end{minipage}
    &
    \begin{minipage}{0.45\hsize}
      \subcaptionbox{Cache-miss ratio. \label{fig:fetch_add_test_cm}}
      {\includegraphics[scale=0.8]{fig/central/fetch_add_cm.pdf}}
    \end{minipage}
  \end{tabular}
  \caption{Scalability of fetch\_add}
\end{figure}



==> vldb_format/src/ccbench-proof.tex <==
\section{CCBench}
\label{sec:Platform}

\begin{figure}[tb]
 \begin{center}
  \includegraphics[scale=0.41]{fig/CCBench-arch-kaw-yoko.pdf}
  \caption{CCBench Architecture}
  \label{figure::CCBench Architecture}
 \end{center}
\end{figure}

\subsection{Fairness Condition}
When analyzing concurrency control protocols, the performance of protocols should be evaluated under a fair condition.
%
The meaning of fairness may vary depending on situations.
In this paper, we claim that {\bf basic modules should be shared to keep fair analysis}.
The performance of modern protocols is deeply related to the exploitation of underlying hardware, and thus they are sensitive to engineering details.
Therefore, the basic modules of an evaluation platform should be shared for fair evaluation.
%
Access methods (e.g., Masstree) and local data structures (read and write sets) need to be shared among protocols.
The effects of memory allocator should be eliminated as much as possible.
The workload should be given in the same way.

%
% conventional platforms
% 
Some of analysis studies satisfy our fairness condition.
%
Yu et al.~\cite{yu2014staring} developed DBx1000~\cite{dbx1000}.
It is used to analyze multiple protocols, to evaluate TicToc, and to evaluate protocols with the real 1568 core machine~\cite{10.1145/3399666.3399910}.
Some modern protocols (Cicada, MOCC, ERMIA) are out of scope.
%
Wu et al.~\cite{cavalia_paper} developed Cavalia~\cite{cavalia} to compare HTCC protocol to conventional protocols. Some modern protocols (Cicada, ERMIA, Silo, TicToc, MOCC) are out of scope.
%
Wu et al.~\cite{wu2017empirical} developed Peloton~\cite{peloton} to compare MVCC protocols though they focused on evaluating only MVCC protocols and some modern protocols (Cicada, ERMIA, Silo, TicToc, MOCC) are out of scope.
%
Appuswamy et al.~\cite{trireme} developed Trireme to compare protocols in four architecture classes including shared everything.
Some modern protocols (TicToc, Cicada, MOCC, ERMIA) are out of scope.
%
A protocol offers a variety of optimization methods.
Even if a protocol {\sf P} does not include the optimization method {\sf O} at the time of proposal, a platform should be able to offer {\sf O} to {\sf P} if users require because performance of a protocol highly depends on optimization methods.
%
For example, RapidGC proposed by Cicada can be also applied to both SI and ERMIA.
NoWait~\cite{10.1145/356842.356846} can applied to Silo and it can improve performance 
as illustrated in Fig. \ref{fig:ycsbA_tuple100m_skew09_slprp0-1000_tps}.
%
None of the above platforms do not have this concept.

Some of studies do not satisfy our fairness condition.
% Cicada
Section 4.2 in Cicada paper~\cite{lim2017cicada} states,
``Cicada and existing schemes in DBx1000 share the benchmark code,
but have separate data storage and transaction processing engines.''.
% MOCC
In MOCC paper~\cite{wang2016mostly}, pure OCC, MOCC, PCC (2PL variants) implementation uses FOEDUS, Dreadlock / WaitDie / BlindDie (2PL variants) uses Orthrus and ERMIA implementation uses ERMIA system, which means three benchmark systems are mixed.
% ERMIA
In ERMIA paper~\cite{kim2016ermia}, to implement Silo, it uses the Silo system while the SI/SSI use the ERMIA system, which means two benchmark systems are mixed.
In these cases, a huge amount of efforts by experts is required to conduct the fair comparison, and it seems not easy especially for papers that propose a novel protocol or optimizations.

\subsection{CCBench: A Platform for Fair Analysis}
\label{sec:A Platform for Fair Comparison}

\input{src/opt_table}

We developed CCBench, an analysis platform for in-memory CC protocols
that satisfies the above fairness conditions.
CCBench is publicly available on GitHub~\cite{thawkccbench}.

To satisfy fairness condition, CCBench shares basic modules among protocols.
The architecture of CCBench is illustrated in Fig.\ref{figure::CCBench Architecture}.
CCBench runs a fixed number of worker threads in a single node.
Each thread executes both the client and the server logic.
The client generates a transaction with read/write operations using the workload parameters at runtime.
The server provides APIs as C++ functions, such as read, write, commit, and abort.
The client calls the APIs to run transactions.
The server runs the transactions requested from the client inside a worker thread.
The code of client is separated from that of server in CCBench, while their codes are built into a single executable binary.
CCBench uses mimalloc~\cite{mimalloc} as a memory allocator.
We conducted memory allocation that is interleaved among all CPU sockets by using the Linux numactl command.
CCBench carefully avoids memory allocation as much as possible so that the penalty~\cite{clements2013radixvm} of the Linux virtual memory system can be ignored, and the execution of protocols can avoid performance degradation due to undesirable side-effects of memory allocators.
CCBench initializes the database for each experiment,
pre-allocates the memory for objects, and reuses them during the experiment.
Allocated memories for local data structure (read/write set)
and the generated operations for a transaction are reused for next transaction.
We properly aligned the metadata and record data to reduce false sharing.
We implemented a wrapper of Masstree implementation~\cite{masstree_beta}, and all protocols use it for access methods.

CCBench offers seven versatile optimization methods as shown in Table~\ref{tab:Experimental Parameters}.
(1) {\sf Decentralized ordering}: avoiding simultaneous accesses to a shared single counter.
(2) {\sf Invisible read}: a read operation that does not pollute the cache memory.
(3) {\sf NoWait}: an immediate abort when detecting a conflict and retry.
(4) {\sf Read Phase Extension}: an artificial delay in the read phase inspired by the extra read that retries the read operation after abort. This is proposed by us.
(5) {\sf Adaptive backoff}: an artificial delay before restarting an aborted transaction.
(6) {\sf Assertive Version Reuse}: allocating thread local space to keep versions to avoid memory manager access.
(7) {\sf RapidGC}: frequently updating timestamp watermark for garbage collection in MVCC protocols.
%
CCBench enables additional optimization methods to 2PL, Silo, TicToc, SI, ERMIA, and Cicada.
%
It should be noted that CCBench does not support read-only optimization methods introduced in Silo, FOEDUS, MOCC, and ERMIA.
This is because this optimization improves performance in a specific case
(i.e., 99\% read-only transactions, 1\% write transactions, skew at 0.99),
and such a workload does not appear in this paper.

%
% Extend CCBench
%
\input{src/extend_ccbench.tex}

\subsection{Details of Optimization Methods}
\label{sec:Implementing Optimization Techniques}
{\bf 2PL:~}
For efficiency, we implemented the reader/writer lock system with the CAS operation used in the protocol from scratch.

{\bf Silo:~} We padded the global epoch (64 bits) into the cache line size (64 bytes)
to reduce false sharing that can be caused by the global epoch state change.
The calculation of commit TID is expensive since it requires loops for both the read set and the write set.
We reduced these two loops by calculation at write lock acquisition and read verification, which leads efficiency.

{\bf ERMIA:~}
We adopted the latch-free SSN to avoid expensive SSN serial validation.
This implementation avoids the validation from being a critical section.
We integrate pstamp and sstamp to reduce memory usage.
We optimized the transaction mapping table.
Straightforwardly, the mapping table is designed as a two-dimensional global array with a thread number, TID, cstamp, and last cstamp, which requires a lock manager for updates and read over the rows.
%
This causes performance degradation due to serialization.
Therefore, we design a data structure that expresses the rows in a one-dimensional array
so that it can be latched with a single atomic compare-and-swap (CAS) operation,
and performance was improved by avoiding serialization and cache pollution for row element access.
We adopted rapid garbage collection {\sf RapidGC}~\cite{lim2017cicada}.
%CASed transaction mapping table objects and version objects are garbage collected based on calculating a threshold that is not accessed by other workers.
The transaction mapping table object exploits our {\sf assertive version reuse} described at the end of this section,
and the load on the memory manager is almost for free.

{\bf TicToc:~}
We implemented all the three optimization methods (TicToc-NoWait, preemptive aborts, timestamp history).
We also improved the algorithm 5 in the original paper by removing redundant read timestamp updates.
It should be noted that if the recorded read timestamp and updating value is the same, actual update is not necessary.

{\bf MOCC:~}
MOCC periodically resets temperature information~\cite{wang2016mostly}.
This approach changes many cache lines to the invalid state simultaneously, and performance deteriorates.
% hoshino
Instead, our implementation stores the epoch ID of the latest reset timing and temperature together and avoids multiple resets in the same epoch.
%
Therefore, the performance was improved by reducing the cache pollution cost and the resetting cost
while finely controlling the temperature.
We do not implement MQL lock since our environment has only 4 NUMA nodes, and its effect would be limited.
We instead use the reader/writer lock that is also used in our 2PL implementation.


{\bf Cicada:~}
We implement all the six optimization methods. 
({\sf sort write set by contention}, {\sf pre-check version consistency}, {\sf adaptive backoff},
{\sf early aborts}, {\sf rapid garbage collection}, and {\sf best-effort inlining}). 
Besides, we fixed a logical bug, which is the incomplete version consistency check in the validation phase.
The original paper only confirms that the read version is still the visible version.
However, it needs to check if it is the latest visible version too.
If a newer version exists in the observable range, it means that it should have been read and the transaction view will be broken.
As for the one-sided synchronization, we turned off it to provide high efficiency.

{\bf CCBench:~}
{\sf Assertive Version Reuse}:~ In MVCC protocols (SI, ERMIA, and Cicada),
some operations such as creating new versions and deleting old versions puts a load on the memory manager.
%which is also true for memory managers with thread-local memory pools.
So, we worked on a new optimization method, assertive version reuse that avoids overloading the memory manager in MVCC protocols.
By using this method, each worker thread maintains a container for future version reuse.
When garbage collection begins, collected versions are stored in this container.
A new version is taken from this container except it is not empty.
Otherwise, it requests a space to the memory manager as usual.
%
Our system estimates the necessary space at a garbage collection before starting experiments,
and the spaces are allocated in advance.
By this optimization, our MVCC protocols put almost no burden on the memory manager.
%
Besides, we present {\sf Read Phase Extension} that delays execution inspired by the extra reads in Section \ref{sec:Effect of Extra Read and Read Phase Extension Method}, 
 and {\sf Aggressive Garbage Collection} that collects even visible versions in Section \ref{sec:discussion-towards-version-lifetime-control}.

==> vldb_format/src/cicada_repro_comment.tex <==
In Figs.
\ref{fig:ycsbA_tuple10m_ope16_rmw_skew0-099_th28_tps},
\ref{fig:ycsbB_tuple10m_ope16_rmw_skew0-099_th28_tps},
and \ref{fig:ycsbB_tuple10m_ope1_rmw_skew099_tps}, the tendencies in our result with Silo, TicToc, MOCC, ERMIA, 2PL are
the same to the corresponding figures in the original paper.
%though our absolute throughputs are relatively lower.
% 
However, the results of Cicada are different from ours.
Fig. \ref{fig:ycsbB_tuple10m_ope1_rmw_skew099_tps} shows Cicada is worse than Silo and TicToc in read intensive workload, and this is inconsistent with Fig. 7 in \cite{lim2017cicada}.
We consider original result is inconsistent with theory.
In read-intensive workload, Cicada needs to create versions on write operations and the cost for version traversal increases while SVCCs do not have such additional cost.
This can be confirmed by our experiment about read intensive workload (YCSB-A/B, no skew, high cardinality) shown in Fig. \ref{fig:latency_breakdown_tuple100m_skew0}.
Besides, it should be pointed out that our results with MOCC and TicToc are almost consistent with original papers as described above.
%
%In addition, all the data in Fig. \ref{fig:ycsbA_tuple10m_ope16_rmw_skew099_tps} are around three times less efficient than that of the original paper.
%We guess it is for the parameter of the adaptive backoff that is effective for YCSB-A with high skew. The values of {\sf max} and {\sf min} parameters of the adaptive backoff are not described in \cite{lim2017cicada}. The adaptive backoff for Cicada is highly efficient than the simple backoff scheme in DBx1000 for other protocols, and only Cicada uses the adaptive one while others use the simple one in \cite{lim2017cicada} to demonstrate the effect of the adaptive backoff. 

We consider the reasons for this inconsistent result is caused by the use of multiple different reference implementations.
The Cicada system itself is implemented by authors.
However, they use reference implementation for Silo, TicToc, MOCC, and ERMIA.
Since the performance of modern protocols are deeply related to the engineering details, use of different basic modules or different implementation of optimization method incline to produce inconsistent result.
%
If all the analyses are done at a single platform, this problem disappears.


==> vldb_format/src/concl.tex <==
\section{Conclusion}
\label{sec:Conclusion}
This paper proposed yet another concurrency control analysis platform CCBench besides DBx1000~\cite{dbx1000}, Peloton~\cite{peloton} and Trireme~\cite{trireme}.
CCBench offers seven protocols and seven optimization methods, and enable to configure seven workload parameters.
We analyzed the protocols and optimization methods varying workload parameters fixing the thread number to 224.
Conventional studies~\cite{dbx1000,peloton,trireme} focus on thread scalability, and none of them explore the space we analyzed.

% takeaway 
\input{src/key_takeaway.tex}

In future work, we add new functions that process insertion/deletion operations and recovery module to CCBench.
%
The code of CCBench and all the data in this paper are publicly available~\cite{thawkccbench}.
We wish CCBench contributes to the progress of transaction research at the many-core architecture era.


==> vldb_format/src/delay.tex <==
\section{Effect of Delay}
\label{sec:Delay Control}
\subsection{Confirmation of Effect of NoWait}
\subsubsection{Wait or NoWait?}
\label{sec:Wait or NoWait?}
\input{src/delay_figure}

To mitigate performance degradation caused by conflicts, putting an additional artificial delay before retry has been studied as optimization methods such as
{\sf TicToc-NoWait}~\cite{yu2016tictoc} or {\sf adaptive backoff}~\cite{lim2017cicada}.
%
In contrast to the {\sf Wait} method that waits for a lock release, the {\sf NoWait} immediately releases locks when a conflict is detected and immediately retries.
%TicToc proposes a variant of {\sf NoWait} denoted as {\sf TicToc-NoWait} described in Section \ref{sec:Concurrency Control Protocols}.
%
The question is that to deal with the contention, which should we choose, {\sf NoWait} or {\sf Wait}?

To answer this question, varying the skew, we compare three methods:
2PL-Wait, 2PL-NoWait, and MOCC that is the mix of OCC and 2PL-Wait.
%
In Fig.~\ref{fig:ycsbB_tuple100m_skew06-085_tps}, all three protocols start to degrade performance at skew 0.7 due to high conflicts.
%
%Aborts occur at 2PL-Wait by deadlock resolution.
%A protocol can choose either wait for a lock to be released or not, i.e., Wait or NoWait, to deal with conflicts.
%Though NoWait is a popular technique, it is not yet investigated that which is more efficient.
We compare 2PL-Wait, 2PL-NoWait, and MOCC(-Wait) that performs similarly to 2PL-Wait on a highly conflicted situation.
All operations of each transaction are sorted before its starting in advance to avoid deadlock for 2PL-Wait.

MOCC demonstrates excellent performance as shown in Fig.~\ref{fig:ycsbB_tuple100m_skew06-085_tps}. This is because MOCC manages fewer lock objects under the workloads with less skew.
%Both 2PL and MOCC uses the reader-writer lock implemented by atomic operations in our platform.
%Lock management requires some overhead and less skew requires less usage of locks, which provides efficiency for MOCC. Fig.~ \ref{fig:ycsbB_tuple100m_skew06-085_ar} illustrates that 2PL-NoWait starts to abort at skew 0.7, read/write contensions have begun to occur, and performance degradation has started.
It should be noted that 2PL-Wait and 2PL-NoWait are compatible.
2PL-Wait and 2PL-NoWait show similar performances at skew 0.6-0.85, so it is considered that the cost of abort-retry and the cost of waiting for lock were almost the same in this workload.
Therefore, we need more contention to answer the question.

\subsubsection{When NoWait is Inefficient}
\label{sec:When NoWait is Inefficient}
To provide more contentions, we increase the transaction size, the number of operations in a transaction.
The cost of aborts should be small for short transactions, while large for long ones.
Therefore, in long transactions, the abort-retry cost increases, which may exceed the lock waiting cost.
We used YCSB-B benchmark, setting the cardinality to 100 million, skew to 0.8, and varied the number of operations.
Operations are sorted due to the same reason in Section \ref{sec:Wait or NoWait?}.
%Access destinations are sorted before a transaction starts to avoid deadlock resulution overhead.
% problem,
Fig. \ref{fig:skew_on_large_records} illustrates that the lock waiting cost of {\sf Wait} and the abort-retry cost of {\sf NoWait} are similar.
However, Fig. \ref{fig:ycsbB_tuple100m_skew08_ope10-100_tps} illustrates that {\sf Wait} outperforms {\sf NoWait } as transaction size increases.
%In other words, which of NoWait and Wait is better depends on the workload, and NoWait is less efficient in this experiment.
%
%Also, MOCC still shows the best performance.
%In Fig.~\ref{fig:ycsbB_tuple100m_skew08_ope10-100_tps}, the performance of 2PL deteriorates sharply when the skew is 0.8.
%In Fig.~\ref{fig:skew_on_large_records}, we observe sufficient read/write contentions when the skew is 0.8.
%At this time, we observe that the same performance is exhibited because the abort-retry cost is almost the same as the lock waiting cost.
%
%We claim that both of Wait and NoWait are considered as delay control methods that deals with the conflicts.
%
% Summary
%
NoWait demonstrates efficiency only for small size transactions.
Therefore, the control of waiting time is important for efficiency.

\if 0
Aside from Wait and NoWait, backoff is an optimization that flexibly adjusts the time interval between abort and retry.
Its specific example is the adaptive backoff in Cicada.
%The Cicada paper claims that it is an effective technique.
The control of delay from conflict detection to retry invocation is considered to have a significant effect on performance.
This performance factor is summarized in this paper as delay control.
\fi


\subsection{Effect of Extra Read and Read Phase Extension Method}
\label{sec:Effect of Extra Read and Read Phase Extension Method}
Besides {\sf Wait}, {\sf NoWait}, and {\sf adaptive backoff}, we present another deley related optimization method, {\sf read phase extension} that is inspired by the positive effect of extra read.
Extra reads is a process to read the same record twice or more due to interrupts of concurrent update transactions.
%Such retries are necessary to emulate the atomic read of the record contents.
%A transaction under optimistic protocols reads a unique record identifier for each update before loading the payload.
%After that, the transaction reads payload, and then it reads the record identifier again.
%If the record identifier is not the same, the transaction executes another read operation.
%This is the extra read.
% TicToc
\if 0
The effect of extra read is similar to the artificial delay with validation phase failure presented by TicToc-NoWait. The delay in TicToc is described as 1 us in paper, but the sleep code in its implementation on GitHub~\cite{dbx1000} have been replaced to {\tt \_mm\_pause} call that means almost zero delay when we investigated it.
\fi
%
Fig.~\ref{fig:ycsbA_tuple100m_skew09_val4-1k_tps} illustrates that throughput first increases as payload size increases, and then it starts to decrease after passing a certain point.
%
It is expected the increase of payload size causes performance degradation in OCC, and this is consistent with the right half of the graph.
However, the performance improvement in the left half of the graph is counterintuitive.
%
We hypothesized that this result was provided by the delay caused by extra read.
%
As explained, according the increase of payload size, the time for reading payload prolongs.
%
Then, the possibility of being interrupted by update transaction improves, and the number of extra reads increases.
%
This behavior extends the read phase and reduces the number of transactions that run the validation phase in parallel.
%
%It reduces concurrent transactions and reduces contention.
As committing update transactions decreases, the number of the read validation failures also decreases, and it leads to performance improvement.
%
By delaying the retry of the atomic read, the number of concurrent workers that process the validation phase in the entire system is reduced, which also reduces contentions.

% Read phase extension
\input{src/read_phase_extension.tex}



==> vldb_format/src/delay_figure.tex <==
\begin{figure}[t]
  \begin{tabular}{cc}
    \begin{minipage}{0.45\hsize}
     \begin{flushleft}
      \subcaptionbox{Throughput \label{fig:ycsbB_tuple100m_skew06-085_tps}}
      {\includegraphics[scale=0.9]{fig/delay/comp_ycsbB_tuple100m_skew06-085_tps.pdf}}
     \end{flushleft}
    \end{minipage}
    &
    \begin{minipage}{0.45\hsize}
      \subcaptionbox{Abort Ratio \label{fig:ycsbB_tuple100m_skew06-085_ar}}
      {\includegraphics[scale=0.9]{fig/delay/comp_ycsbB_tuple100m_skew06-085_ar.pdf}}
    \end{minipage}
  \end{tabular}
  \caption{Wait or NoWait: YCSB-B, 100 M Records, 224 Threads, Payload 4 bytes, 10 ops/trans.}
  \label{fig:skew_on_large_records}
\end{figure}


%
% Wait outperforms NoWait
%
\begin{figure}[t]
  \begin{tabular}{cc}
    \begin{minipage}{0.45\hsize}
     \subcaptionbox{Throughput.\label{fig:ycsbB_tuple100m_skew08_ope10-100_tps}}
     {\includegraphics[scale=0.9]{fig/delay/comp_ycsbB_tuple100m_skew08_ope10-100_tps.pdf}}
    \end{minipage}
    &
    \begin{minipage}{0.45\hsize}
     \subcaptionbox{Abort ratio.\label{fig:ycsbB_tuple100m_skew08_ope10-100_ar}}
     {\includegraphics[scale=0.9]{fig/delay/comp_ycsbB_tuple100m_skew08_ope10-100_ar.pdf}}
    \end{minipage}
  \end{tabular}
 \caption{Impact of Transaction Size: YCSB-B, 100M Records, 224 Threads, Payload 4 bytes, Skew 0.8.}
 \label{fig:Impact of Transaction Size: YCSB-B, 100M Records, 224 Threads, Payload 4 bytes, Skew 0.8.}
\end{figure}


%
% Read Phase Extension
%
\begin{figure*}[t]
  \begin{tabular}{ccc}
    \begin{minipage}{0.3\hsize}
     \subcaptionbox{Throughput \label{fig:ycsbA_tuple100m_skew09_val4-1k_tps}}
      {\includegraphics[scale=1.15]{fig/delay/comp_ycsbA_tuple100m_skew09_val4-1k_tps.pdf}}
    \end{minipage}
   &
    \begin{minipage}{0.3\hsize}
     \subcaptionbox{Extra Reads \label{fig:ycsbA_tuple100m_skew09_val4-1k_er}}
     {\includegraphics[scale=1.15]{fig/delay/comp_ycsbA_tuple100m_skew09_val4-1k_er.pdf}}
    \end{minipage}
   &
    \begin{minipage}{0.3\hsize}
     \subcaptionbox{Read Phase Extension Method\label{fig:ycsbA_tuple100m_skew09_slprp0-1000_tps}}
     {\includegraphics[scale=1.15]{fig/delay/comp_ycsbA_tuple100m_skew09_slprp0-1000_tps.pdf}}
    \end{minipage}
  \end{tabular}
 \caption{Effect of Delay provided by Extra Read: YCSB-A, 100M records, 224 threads, skew 0.9, 10 ops/trans.}
 \label{fig:Effect of Delay provided by Extra Read: YCSB-A, 100M records, 224 threads, skew 0.9, 10 ops/trans.}
\end{figure*}



==> vldb_format/src/diff.tex <==
In our setting, we applied the RapidGC to ERMIA and SI in all the cases, NoWaitto Silo in Fig. \ref{fig:ycsbA_tuple100m_skew09_slprp0-1000_tps}, and adaptive backoff to TicToc in Fig. \ref{fig:tuple10m_val1k_ycsb_high_tps}


==> vldb_format/src/environment.tex <==
\subsection{Environment}
% Machine
In the experiment, we used a single server that has four Intel (R) Xeon (R) Platinum 8176 CPU @ 2.10GHz.
The CPU has 28 physical cores with hyper threading, and the server has 224 logical cores.
%
Each physical core has 32 KB private L1d cache and 1 MB private L2 cache.
%
The 28 cores of a single processor share a 39 MB L3 cache.
%
The total cache size is about 160 MB.
Forty-eight DDR4-2666 are connected, the size of each is 32 GB, and the total size is 1.5 TB.

% Result
In all graphs in this paper about CCBench, each plot point shows an average of 5 times of runs and the duration of each run is 3 seconds.
We confirm that these number produce stable results in CCBench.
%We set number of runs so that stable results are obtained.
If an error bar is displayed, it indicates the range of maximum and minimum values.
We counted the number of the committed and the aborted transactions to calculate average throughput.
We use \texttt{rdtscp} instruction to measure the latency of the transitions and their portions.
Each worker thread was pinned to a specific CPU core in every experiment.
%
%As can be seen below, we set the number of worker threads to 224 except from reproductions.


==> vldb_format/src/extend_ccbench.tex <==
Users of CCBench can easily add new protocols into the platform.
After replicating the existing protocol with a directory, the user rewrites functions corresponding to the transaction begin/read/write/commit/abort in the transaction executor class. The user can reuse basic modules such as workload generator, memory management, and so on.
%
Users easily attach or detach optimization methods provided by CCBench to their protocols just by rewriting the preprocessor definition in the Makefile.
A developer guide for CCBench user is available at \cite{cc_format}.
%
One of our team members implemented the simple OCC following this guide~\cite{occ_nemoto}, and published the experience for other users~\cite{nemotoccbench}.
%
Users can also switch the configuration of the optimization methods, key-value size, and protocol details in the same way.
%
At the experiment, user can set the workload settings by specifying the run-time argument using the six workload parameters described in Table \ref{tab:Experimental Parameters}.
%
This design helps a user of CCBench to conduct experiment than that of DBx1000 \cite{dbx1000} since DBx1000 manages these values preprocessor definitions in a configuration file ({\sf config.h}), a user needs to recompile the code to conduct an experiment, which requires more efforts to users.


==> vldb_format/src/intro.tex <==
\section{Introduction}
\subsection{Motivation}
Transacting processing systems or concurrency control protocols for thousands of CPU cores in a single server
emulated~\cite{yu2014staring}, implemented~\cite{kimura2015foedus},
and have just analyzed~\cite{10.1145/3399666.3399910}.
%
Along with them, a variety of concurrency control protocols for a single server~
\cite{tu2013speedy} % Silo
\cite{wang2016mostly} % MOCC
\cite{yu2016tictoc} % TocToc
\cite{kim2016ermia} % ERMIA
\cite{lim2017cicada} %
have been proposed in recent years to exploit many core architecture.
%
%For example, Silo~\cite{tu2013speedy}~exhibits high performance as optimistic concurrency control which were traditionally thought to be inefficient.
These modern protocols have a variety of optimization methods, and they vary their behaviors depending on workload characteristics (e.g., skew, read ratio, cardinality, etc.).
%
%Since no silver bullets exist, a database user needs to find out appropriate protocols for their purposes; however, how can they do that? Currently, there are two problems to satisfy such user requirements.
%These modern protocols and optimizations have been carefully evaluated.
New protocol studies compare their novel proposals to conventional ones~
\cite{tu2013speedy}   % Silo
\cite{wang2016mostly} % MOCC
\cite{yu2016tictoc}   % TocToc
\cite{kim2016ermia}   % ERMIA
\cite{lim2017cicada}  % Cicada
and analytic studies compare conventional protocols at a common platform~
\cite{yu2014staring}            % DBx1000 or Abyss
\cite{wu2017empirical}          % MVCC
\cite{trireme}                  % Trireme
\cite{10.1145/3399666.3399910}. % Supredome
All the studies mainly evaluate the scalability of protocols. If a protocol increases its throughput as the number of threads increase under a certain workload, the protocol is highly evaluated.
%
However, a machine is usually dedicated for a transaction system.
Then, the number of worker threads is set to the number of CPU cores.
%
We are interested in analyzing protocols in such an environment.
This sort of analyses have not yet conducted in conventional studies, to our knowledge.
%
%Analyzing protocols for a given workload requires a comprehensive and fair evaluation of the protocols.
%
To conduct such analyses, current studies have problems about {\it fairness}.


%To conduct fair evaluation, an analysis platform should provide shared core modules such as access methods (concurrent index) and thread local data structures (read and write sets) for any of the protocols.
To conduct fair evaluation, new protocol studies sometimes use multiple platforms.
% monku to cicada
%This is sometimes unsatisfied.
% Cicada
Cicada~\cite{lim2017cicada} have separate data storage and transaction processing engines.
% MOCC
MOCC~\cite{wang2016mostly} uses three benchmark systems: FOEDUS system, Orthrus system, and ERMIA system.
%Pure OCC/MOCC/PCC implementation uses FOEDUS, Dreadlock/WaitDie/BlindDie implementation uses Orthrus, and ERMIA implementation uses ERMIA. 
% ERMIA
ERMIA~\cite{kim2016ermia} uses two benchmark systems: Silo system and ERMIA system.
%It uses Silo system for Silo implementation while SI/SSI implementation uses ERMIA system.
%
In these cases, a huge amount of efforts by experts is essential to conduct the fair comparison because 
the performance of protocols on many-core architecture is highly associated with the exploitation of underlying hardware, and it requires deep engineering knowledge.
Without experts, reproduction experiment is difficult.
%
% Platform
%
To conduct fair comparison without experts, a common analysis platform is necessary.
The platform provide shared core modules such as access methods (concurrent index) and thread local data structures (read and write sets) for any of the protocols.
It also provide a variety of optimization methods to provide a way to deeply understand protocols.
If an optimization method {\it O} proposed for a protocol {\it P} can be applied to another protocol {\it P'}, it should be possible.
Finally, the platform should be publicly available for reproduction experiments.
%, and it seems not easy especially for papers that propose a novel protocol or optimizations.
% 2. OSS
%Second, an analysis platform should be available because the performance of protocols on many-core architecture is highly associated with the exploitation of underlying hardware, and it requires deep engineering knowledge for efficient software/hardware interactions.
%
Trireme~\cite{trireme} provides CC protocols in four architecture classes: shared everything, partitioned serial execution, delegation, and data-oriented. However, Trireme is not open source.
% 3. Modern protocols
There are open source platforms: DBx1000~\cite{dbx1000}, Peloton~\cite{peloton}, and Cavalia~\cite{cavalia}.
They do not provide modern protocols.
DBx1000 lacks MOCC, ERMIA, and Cicada.
Cavalia and Peloton lack all of Silo, TicToc, MOCC, ERMIA, and Cicada.
% Why not implement on them?

\subsection{Contribution}
{\bf CCBench: A Concurrency Control Evaluation Platform for Fair Comparison:}
We present yet another analysis platform CCBench that provides flexible configurations on both optimizations and workloads for concurrency control.
%
Protocols implemented in CCBench currently are 2PL, Silo, MOCC, TicToc, Snapshot Isolation, latch-free SSN, and Cicada.
%
CCBench offers a variety of versatile optimization methods proposed in both conventional protocols and this work (Table \ref{table::protocol_opt}).
CCBench enables to apply some optimization methods to non-original protocols.
For example, NoWait~\cite{bernstein1987concurrency} to Silo, rapid garbage collection~\cite{lim2017cicada} to multi-version protocols, and adaptive backoff~\cite{lim2017cicada} to all protocols.
%
To provide fairness in analyzing protocols, CCBench provides shared modules including workload generator, access methods (Masstree~\cite{mao2012cache, masstree_beta}), local datasets (read/write sets), and memory manager (mimalloc~\cite{mimalloc} and optimization method {\sf assertive version reuse}).
To evaluate protocols in a variety of situations, CCBench provides seven configuration parameters of workload: skew, payload size, transaction size, cardinality, read ratio, and read-modify-write or not, and number of worker threads.
%
%This flexibility allows CCBench to easily conduct YCSB-A, B, C, and F benchmarks.
CCBench and all of data in this paper are available~\cite{thawkccbench}.

{\bf Analyze Cache, Delay, and Version at 224 threads}
We worked on clarifying the effect of protocols on performance factors by configuring optimization methods and workload settings.
%In this paper, all of our experiments except from reproduction experiments are conducted by using 224 threads. This is because the number of CPU cores is increasing steadily and more parallelism will be common in the near future.
As suggested in~\cite{yu2014staring} or \cite{kimura2015foedus}, the era of a thousand cores is just around the corner.
Conventional analysis studies focus to evaluate thread scalability ~\cite{yu2014staring}~\cite{wu2017empirical}~\cite{10.14778/3055540.3055548}, however, 
we conduct analyses with {\it 224 threads on 224 cores}.

% Cache
We first investigate the effect of optimization methods related to {\bf cache}.
After confirming the centralized counter increases cache line conflicts and performance degradation, we found the following insights.
% Insight 1.
(1) Performance of OCC at read only workload rapidly degrades as cardinality increases even without L3 cache misses (Section \ref{sec:Cache Miss Mitigation}).
% Insight 2.
(2) Silo outperforms TicToc under write intensive workload due to {\sf invisible read} (Section \ref{sec:Effect of Invisible Read}).

% Delay
We second investigate optimization methods related to {\bf delay}.
We found the following insights.
% Insight 3.
(3) OCC requires the extra read process that reads the same record twice or more due to interrupts of concurrent transactions.
Surprisingly, it can improve performance in a certain situation, and we indicate a new optimization method {\sf read phase extension} based on it (Section \ref{sec:Effect of Extra Read and Read Phase Extension Method}).
% Insight 4.
(4) Coping with conflicts, there are two approaches: {\sf Wait} or {\sf NoWait}.
The effectiveness depends on the situation.
Silo with {\sf NoWait} can outperform Silo (Section \ref{sec:Effect of Extra Read and Read Phase Extension Method}),
while 
2PL with {\sf Wait} can outperform 2PL with {\sf NoWait} (Section \ref{sec:When NoWait is Inefficient}).

%
% Besides, we claim that the {\it extra read} is categorized into the delay performance factor.
% Extra read is a re-read process in optimistic protocols.
% Intuitively, it degrades performance.
% However, it indirectly leads to high performance in some situations.
% It is not easy to find out the effect of extra read because it implicitly affects efficiency.
%
%We clarify the situation that extra read provides high performance, and then we discuss a new optimization method, the {\it read phase extension} that provides an artificial delay exploiting local and real-time conflict information.

% Version lifetime
We third investigate optimization methods related to {\bf version lifetime} in multi-version concurrency control (MVCC) protocols.
We found the following insights.
% Insight 5
(5) Mixing implementations is inappropriate. Silo and TicToc can outperform Cicada under a high skew situation (0.99) and
%Other parameters (e.g. write ratio, cardinality, et al) besides skew should be considered simultaneously to compare OCC and MVCC (Section \ref{sec:problem-many-visible-versions}).
% Insight 6
Cicada underperforms Silo under YCSB-A/B with skewless environment, which is inconsistent with results in \cite{lim2017cicada}.
%
%It is confirmed by the result that the latency breakdown of single versioned Cicada is almost the same as that of Silo, which means the cost of version management is not negligible under write intensive workload like YCSB-A (Section \ref{sec:problem-many-visible-versions}).
% Insight 6
(6) Even state of the art garbage collection can not improve performance of MVCC if a single long transaction is mixed into the workload.
%MVCC protocols are expected to demonstrate high performance because of their large scheduling spaces. % compared to single-version concurrency control (SVCC) protocols.
% Its primary overhead is the management of multiple versions.
%If the number of versions grows in main memory, performance would degrade due to both the memory space exhaustion and the high CPU cache miss rate caused by many version traversals or garbage collection.
%Modern MVCC protocols exhibit high throughput, and they rapidly generate many versions, which may incur performance degradation.
%To mitigate the problem, garbage collection plays a key role.
%The rapid garbage collection proposed by Cicada is a state-of-the-art method.
%It frequently checks the visibility of versions and collect obsolete versions immediately.
%We experimentally confirmed that RapidGC is highly effective for a workload that include only short transactions.
%However, we found that it is does not perform even if one long transaction is mixed into the workload.
%In addition, we confirmed that even a machine equipped with 1.5 TB of DRAM would cause a fatal shortage of memory if it does not perform GC at intervals of less than 1 second.
%To our knowledge, none of modern MVCC protocols including Cicada or ERMIA deal with this problem.
%To tackle the problem, we suggest to explore more aggressive version lifetime control methods that collect versions even if they are visible.
%On the other hand, versions can be reduced if write operations can be omittable.
%This idea was first proposed by the Thomas write rule and has been generalized by the non-visible write rule.
%
To overcome the problem, we indicate a new optimization method, {\sf Aggressive Garbage Collection} that collect non-obsolete versions. It requires an unprecedented protocol that weaves GC into MVCC beyond current assumption that GC is attachable (Section \ref{sec:discussion-towards-version-lifetime-control}).

\subsection{Organization}
The rest of this paper is organized as follows.
Section \ref{sec:Preparation} describes preparation. It describes existing concurrency control methods and the evaluation environment.
Section \ref{sec:Platform} first presents CCBench, which is a platform for fairly comparing concurrency control protocols. 
Section \ref{sec:Reproduction of Prior Work} describes the reproduction experiments of prior work using CCBench.
Section \ref{sec:Cache Effect} describes the effect of cache exploitation.
Section \ref{sec:Delay Control} describes delay control.
Section \ref{sec:version-lifetime-control} describes version lifetime management.
Section \ref{sec:Related Work} describes related work, and
Section \ref{sec:Conclusion} concludes this paper.


==> vldb_format/src/invisible.tex <==
\input{src/invisible_figure}
\subsection{Effect of Invisible Read}
\label{sec:Effect of Invisible Read}
%
Updating shared data causes L3 cache misses, leading to performance degradation.
% Silo
%On the other hand, in the evaluation of Silo, the decrease of the L3 cache miss rate is relatively gentle.
The read operation of Silo does not update the metadata, and read operation in Silo does not cause L3 cache misses.
%
This method is referred to as the {\sf invisible read}~\cite{marathe2004design}.
%
{\sf Invisible read} is effective to improve performance in read intensive workloads, however its details have not been yet explored.
% TicToc
Read operations of TicToc typically update the read timestamp and thus it is not the {\sf invisible read}.

%
% Result
To investigate the details, we measure performance of Silo and TicToc varying read ratio and cardinality.
The result is illustrated in Figs.~\ref{fig:ycsb_rratio10-90_tps}-\ref{fig:ycsb_rratio10-90_ca}.
% highly contended
Fig.~\ref{fig:ycsb_rratio10-90_tps} illustrates that TicToc-1K outperforms Silo-1K in low cardinality and write-intensive workloads.
Abort ratio of TicToc-1K is much worse than that of Silo-1K in this case as illustrated in Fig. \ref{fig:ycsb_rratio10-90_ar}.
As shown in Fig. \ref{fig:ycsb_rratio10-90_tps}, at a read-most (90\%) case,
Silo outperforms TicToc rapidly increasing abort ratio (Fig. \ref{fig:ycsb_rratio10-90_ar}).
This is for the {\sf invisible read}.
% low contended
In high cardinality workloads, Silo-1M always outperforms TicToc-1M. Abort ratios of Silo-1M and TicToc-1M are both zero as illustrated in Fig. \ref{fig:ycsb_rratio10-90_ar}. Seemingly this is mysterious since abort rates for both Silo and TicToc are almost zero, and L3 cache miss ratio for both of them are the same.
%
This is because of the cost to deal with contention resolution at TicToc.
They are timestamp history management, early abort judgement, and read time stamp update.
These functions require additional instructions, and thus degraded performance.
To weave {\sf invisible read}, a protocol needs to give up to using them.
%

{\bf Insight 2.}~
Silo can outperform TicToc under write intensive workload due to {\sf invisible read}.

%It is considered that this result is led by the design of TicToc which exhibits high performance in a high contention and high conflicts workloads.
%In a low cardinality workload such as one thousand records, Silo shows the high throughput due to the invisible read when the read ratio is very high.
%For similar reasons, in Fig.~\ref{fig:ycsb_rratio10-90_ca}, Silo appears to have a lower cache miss rate than that of TicToc.
%In the protocol design of Silo, it selected not to track the anti-dependency, and it led to invisible read.
%However, TicToc tracks anti-dependency, and it does not fully provide invisible read.

% 競合が強い環境下で，競合に強い TicToc 設計が活きることがあり，invisible read 設計が活きることがあることを説明する．
% throughput に関する議論

\if 0
% cache-miss rate に関する議論
As cardinality increases, the cache miss ratio of TicToc decreases in Fig.~\ref{fig:ycsb_rratio10-90_ca}.
This is probably because the read-timestamp update of TicToc is likely to cause cache pollution in low memory usage workload.
However, it is not likely to cause it in high memory usage workload due to low cache efficiency.
TicToc updates read timestamps as needed.
As the number of writes increases, the frequency of updating timestamp increases, so the frequency decreases as the read increases, and the cache miss rate may have decreased.
In Fig.~\ref{fig:ycsb_rratio10-90_ca}, the performance trends of Silo and TicToc are the same due to the reduction of the read/write contentions with the increase in the read ratio.
Similarly, with large cardinality such as one million records and low skew, the cache miss rate is low because the access destinations are more distributed and contention is very low.

% optional?? 1M records の方が cache-miss rate が低いのはなぜかの説明（まさかり回避）
The plot of one million records shows a lower cache miss ratio than the plot of one thousand records.
Besides, aborts frequently occur at the situation with one thousand records.
Therefore, the cache is often polluted, and the cache miss rate becomes high.
In Fig.~\ref{fig:ycsb_rratio10-90_tps}, the contentions are reduced by a sufficient number of records, so the abort rate of one million records is almost 0.
Besides, as described above, the memory usage increases due to the sufficient number of records, and then naturally the cache usage rate decreases, and the effect of invisible read are reduced consequently.
As shown in Figs.~\ref{fig:ycsb_rratio10-90_tps}, TicToc is inferior to Silo under low contention workloads because TicToc is designed to achieve high performance under high contention workloads by tracking anti-dependency while Silo does not track, and it becomes overhead under low contention workloads.
On the other hand, in the case of high contention, as shown in Fig.~\ref{fig:ycsb_rratio10-90_tps}, it is considered that the superiority or inferiority of Silo and TicToc is determined by the trade-off between the design for high contention workloads and the effect of invisible read.
\fi

==> vldb_format/src/invisible_figure.tex <==
\begin{figure*}[tb]
  \begin{tabular}{ccc}
    \begin{minipage}{0.33\hsize}
      \subcaptionbox{Throughput \label{fig:ycsb_rratio10-90_tps}}
      {\includegraphics[scale=1]{fig/invisible/comp-silo-tictoc_rratio10-90_tps.pdf}}
    \end{minipage}
    &
    \begin{minipage}{0.33\hsize}
      \subcaptionbox{Abort Ratio \label{fig:ycsb_rratio10-90_ar}}
      {\includegraphics[scale=1]{fig/invisible/comp-silo-tictoc_rratio10-90_ar.pdf}}
    \end{minipage}
    &
    \begin{minipage}{0.33\hsize}
      \subcaptionbox{Cache-Miss Ratio \label{fig:ycsb_rratio10-90_ca}}
      {\includegraphics[scale=1]{fig/invisible/comp-silo-tictoc_rratio10-90_ca.pdf}}
    \end{minipage}
  \end{tabular}
  \caption{Analysis of Invisible Read. 224 Threads, Payload 4 bytes, Skew 0, 10 ops/trans. Cardinality $10^3$ or $10^6$ records}
  \label{fig:Analysis of Invisible Read: YCSB, 224 Threads, Payload 4 bytes, Skew 0, 10 ops/trans.}
\end{figure*}



==> vldb_format/src/key_facets.tex <==
This section describes the concurrency control protocols that we analyze.
%The protocols are listed in Table \ref{tab:Experimental Parameters}.
We classify them into five classes as follows.
(1) pessimistic concurrency control (PCC): 2PL~\cite{weikum2001transactional}.
(2) optimistic concurrency control (OCC): Silo~\cite{tu2013speedy} and TicToc~\cite{yu2016tictoc}.
(3) multi-version concurrency control (MVCC): SI~\cite{jung2013performance} and ERMIA~\cite{kim2016ermia}.
(4) integration of OCC and PCC: MOCC~\cite{wang2016mostly}.
(5) integration of OCC and MVCC: Cicada~\cite{lim2017cicada}.
We explain the details in the rest of this Section.

\if 0
Each protocol has optimization methods, and they are listed in Table \ref{table::protocol_opt}.
\begin{table}[tb]
\begin{center}
 \caption{Analyzed Protocols}
 \label{tab:Experimental Parameters}
\begin{scriptsize}
 \begin{tabular}[tb]{r|l}
  Type & Examples\\
  \hline
  PCC         & 2PL~\cite{weikum2001transactional}\\
  OCC         & Silo~\cite{tu2013speedy}, TicToc~\cite{yu2016tictoc}\\
  MVCC        & SI~\cite{jung2013performance}, ERMIA~\cite{kim2016ermia}\\
  OCC \& PCC  & MOCC~\cite{wang2016mostly}\\
  OCC \& MVCC & Cicada~\cite{lim2017cicada}\\
 \end{tabular}
\end{scriptsize}
\end{center}
\end{table}
\fi

==> vldb_format/src/key_takeaway.tex <==
Through the analysis using CCBench, we first revealed the relationship between the performance factors and the optimization methods.
The key factors were CPU cache, delay, and version lifetime.
The cache is related to the distributed counters and invisible read. The delay is related to NoWait, backoff, and extra read. The version lifetime is related to RapidGC.
%
We then found two new candidates of optimization methods.
%
From the extra read, we discussed the read phase extension. It is classified into the delay control and has more potential than conventional methods since it exploits local contention information while ordinary methods use global information.
%
From the limit of RapidGC that deteriorated in the presence of a long transactions, we discussed the aggressiveGC. It is classified into the version lifetime factor.
It collects non obsolete versions to deal with the long transaction problem.
However, it forces to change the read method in the CC protocol.
Such tight communication requires the integration of protocol and GC.
%


==> vldb_format/src/letter.tex <==
\newpage

\section{Response to Meta Reviewer}
\subsection{Meta-1}
\begin{screen}
 For each algorithm include a performance comparison to results reported in the paper that introduced the algorithm.
\end{screen} 
 
Thanks for your comment. CCBench enables to apply a variety of optimization methods in theory. In this paper, however, we attached only a part of them to some protocols. We explain it in Section \ref{sec:A Platform for Fair Comparison}.
%\input{src/diff.tex}

\subsection{Meta-2}
\begin{screen}
Include TPC-C results for all algorithms.
\end{screen}

Thanks for your comment. We think TPC-C is not suitable for our research purpose. It is because we explored performance factors and the relationship between them and optimization methods. For our purpose, TPC-C is too simple to satisfy our requirements. That is the reason why we used YCSB and provided six parameters. 
%
We explain it in Section \ref{sec:A Platform for Fair Comparison}.
%\input{src/tpcc.tex}

\subsection{Meta-3}
\begin{screen}
Greatly improve the writing clarity. This is very important, since part of the paper’s value is as a tutorial. There are many grammar errors, which is a distraction, but the bigger problem are the vague sentences where the reader has to guess what is meant.
\end{screen} 
Thanks for your comment. We fully and carefully revised this manuscript, and used a proofreading service. 

\subsection{Meta-4}
\label{sec:Meta-4}
\begin{screen}
Expand the Related Work section, which is too sketchy. In particular, do not simply list related papers but compare your work to theirs.
\end{screen}

Thanks for your comment. We revised the related work in Section \ref{sec:Related Work}.
%\input{src/related_core.tex}

\subsection{Meta-5}
 \label{sec:Meta-5}
\begin{screen}
Explain how to extend the framework with other CC algorithms, storage mechanisms, and optimizations.
\end{screen} 

Thanks for your comment.
We add the procedure in Section \ref{sec:A Platform for Fair Comparison}.
%\input{src/extend_ccbench.tex} 


\section{Response to Reviewer-1}
\subsection{Review1-D1}

\begin{screen}
This paper is better suited as an experiments paper since the novel research contributions of the paper is low. Even though it is not tagged as an experiments
paper, I evaluate it as one, and my evaluation is based on that characterization.
\end{screen} 

Thanks for your comment. We intended to submit this paper to the ''experimental and analysis '' track. If there is any mistake about submission, we are sorry that for the mistake.

\subsection{Reviewer1-D2}
\begin{screen}
Since the paper starts with a summary of the different protocol, it would be good to summarize the key facets of each protocol in one table that allows the reader to grasp them at once and better understand the key results presented in the experiments. Much like Table 2, but for the original approaches. Similarly, since there are a lot of experiments presented, it would be good to provide a section/table that summarizes the key takeaways.
\end{screen} 

Thanks for your suggestion. About key facets, we added a table and an explanation in Section \ref{sec:Concurrency Control Protocols}.
%\input{src/key_facets.tex}

Then we added an explanation about key takeaways in Section \ref{sec:Conclusion}.
%\input{src/key_takeaway.tex}

\subsection{Reviewer1-D3}

\begin{screen}
All the experiments are with YCSB. Even though YCSB is pretty configurable, it
is still very simple transactions not very representative of realistic applications. It would be good to add a bit more diversity with the benchmarks, e.g., consider the suite of benchmarks supported by OLTPBench
%(https://github.com/oltpbenchmark/oltpbench/tree/master/src/com/oltpbenchmark/benchmarks) 
 and picking one or two from there that adds diversity in the workloads, potentially making the analysis more interesting.
\end{screen}

Thank you for your suggestion.
%
The purpose of this paper is to classify optimization methods into three performance factors, and to explore new optimization methods. As you point out, YCSB is pretty configurable and we achieved our purpose. The OLTPBench has a variety of workloads and is really interesting, but could not find more configurable one than YCSB. Thus we did not use it. We also tried to find real applications from Subaru telescope team who try to discover time-varying celestial body (a kind of outlier) in real-time, but the workload is not transactional, and gave up.
%\input{src/analyzed_space.tex}

\subsection{Reviewer1-D5}

\begin{screen}
How extensible is this framework for addition of other algorithms or implementations of storage engines or other configurations.
\end{screen} 
 
Thanks for your comment.
We add the procedure in Section \ref{sec:A Platform for Fair Comparison}.
%\input{src/extend_ccbench.tex}

\subsection{Reviewer1-D6}

\begin{screen}
The language of the paper needs significant improvements. For instance,\\
-- ``We second organize two performance factors that have not been fully organized yet.'' What does this sentence mean?\\
-- ``The rapid garbage collection at Cicada demonstrates''\\
-- ``We show these optimizations harness the version lifetime factor with limitations.''\\
and many more..\\
\end{screen}
 
Thanks for your comment. We fully and carefully revised this manuscript, and used a professional proofreading service. 

\subsection{Reviewer1-D7}
\begin{screen}
The related work section needs more work. Related work is more than just a list of papers as the current section presents. It would be good to better compare and contrast with similar related work studying performance characteristics.
\end{screen}

Thanks for your comment. We revised the related work in Section \ref{sec:Related Work}. Please see Section \ref{sec:Meta-4} (Meta-4).

\section{Response to Reviewer-3}
\subsection{Reviewer3-D1}

\begin{screen}
It can be a nice contribution to evaluate state-of-the-art concurrency control protocols with a fair performance comparison among them and demonstrate what
insights are learned from the study and how we should design concurrency control protocols in the future. This paper tries the first step (fair performance evaluation)
but does not give many insights to the readers. Therefore, not much can be learned from this paper besides what has been learned in the original papers describing these concurrency control protocols.
\end{screen} 

Thank you for your comment. We rewrite this paper so that readers can understand the contributions.
%
In this paper, we first confirmed knowledge presented by original papers with CCBench.
Then we present the following insights.
\begin{itemize}
 \item In read intensive workload, Silo outperforms TicToc due to its solid design. As can be seen in Fig.~\ref{fig:ycsb_rratio10-90_tps}, Silo outperforms TicToc though abort ratio of them are zero, and their L3 cache miss ratios are the same. This is due to the additional function at TicToc. Since conventional studies evaluate only the scalability, none of them report this difference.
 \item Wait policy outperforms NoWait policy if transaction size is large. A modern optimization methods TicToc-Wait is effective. It immediately release locks when it detects write/write conflict. However, the NoWait policy underperforms when transaction size is large. This is not known for modern protocols. This is described in Section \ref{sec:When NoWait is Inefficient}.
 \item Extra read in OCC can improve performance, and from the behavior we designed  a new optimization method {\sf read phase extension} and implemented it onto CCBench. This is described in Section \ref{sec:Effect of Extra Read and Read Phase Extension Method}.
 \item As known, efficient garbage collection plays a key role for MVCC performance. We first show that even the state of the art method RapidGC does not perform if the workload includes a single long transaction as shown in Fig. \ref{fig:comp_cicada-ninline_ycsbA_tuple1m_gci1us-1s_tps}, and we propose the idea of {\sf aggressive GC} to deal with this problem. This is described in Section \ref{sec:limitation-of-current-approaches} and \ref{sec:discussion-towards-version-lifetime-control}.
\end{itemize}

\subsection{Reviewer3-D2}

\begin{screen}
Given that all of these state-of-the-art protocols have their own optimized implementations. The paper needs to justify that the implementations in CCBench are at least as optimized as the original implementations. An evaluation of both original protocols and CCBench on standard benchmarks is necessary.
\end{screen}

In our reproduction experiments  described in Section \ref{sec:Reproduction of Prior Work}, you can find that our result and original results are consistent in the following cases.
\begin{enumerate}
 \item Fig. \ref{fig:ycsbC_tuple50_tps} in this paper shows MOCC and Silo achieves around 100 Mtps with 224 threads, and Fig. 6 in MOCC paper \cite{wang2016mostly} show MOCC and Foedus achieves 100 Mtps with 288 threads.
 \item Fig. \ref{fig:silo-mocc_tuple50_rratio10-100_tps} show the throughput of MOCC and Silo when varying write ratio. This result is almost the same to Fig. 7 in MOCC paper \cite{wang2016mostly}. Fig. \ref{fig:silo-mocc_tuple50_rratio10-100_ar} in this paper abort ratio of Silo and MOCC, and this is consistent with Fig 7 in MOCC paper.
 \item Fig. \ref{fig:tuple10m_val1k_ycsbC_tps} in this paper shows Silo and TicToc' achieve 25 Mtps with 80 threads in read-only workload, and Fig. 6 in TicToc paper show almost the same result.
 \item Fig. \ref{fig:tuple10m_val1k_ycsb_medium_tps} in this paper shows Silo and TicToc shows around 4 Mtps with 80 threads in YCSB(medium contention), and Fig. 7(a) in TicToc paper shows the almost the same result.
 \item We evaluate a standard benchmark system DBx1000, and the results are shown in
       Fig. \ref{fig:ycsbC_tuple50_tps},
       \ref{fig:silo-mocc_tuple50_rratio10-100_tps},
       \ref{fig:silo-mocc_tuple50_rratio10-100_ar},
       \ref{fig:tuple10m_val1k_ycsbC_tps},
       \ref{fig:tuple10m_val1k_ycsb_medium_tps}.
       The results of CCBench and that of DBx1000 showed similar trends, and CCBench outperformed DBx1000. Thus we consider the implementations of CCBench are at least as optimized as the original implementations. 
       One of reproduction experiments about TicToc can be found at {\it https://github.com/thawk105/ccdata/blob/eda48f6eb6b31a8f7310dbdcac7a79c6d4cd4abb/dbs11/key8-val1k/masstree\_use/result\_tictoc-original-no-wait\_ycsb\_tuple10m\_skew09.dat}.
       Readers can check all the experimental data in this paper on GitHub {\it https://github.com/thawk105/ccdata }
       
\end{enumerate}

% TicToc problem
One problem in reproduction experiment with TicToc is Fig. \ref{fig:tuple10m_val1k_ycsb_high_tps} in this paper. This is not consistent with Fig. 8(a) in original paper. When we attach backoff function to TicToc, its behavior is almost the same. So, we think description about backoff is omitted in the original paper.

% Cicada problem
% omit?
Result of Cicada is partially reproducible. We describe it in Section \ref{sec:Cicada}.

\subsection{Reviewer3-D3}

\begin{screen}
 There are some factual errors in the paper.

 - Section 2.1: The description of TicToc says: ``NoWait in validation does not wait for lock releasing at validation phase. It instead immediately aborts and retries the
transaction.'' The NoWait optimization in TicToc does not abort and retry the entire transaction, it only retries the lock acquiring process. This leads to significant
 performance difference.

 - End of Section 2.1: ``For the deadlock resolution, our 2PL adopts the NoWait optimization technique introduced by TicToc that immediately aborts when conflict
is detected.''. NoWait is not introduced by TicToc, NoWait has existed decades before TicToc, TicToc is just reusing the idea for the lock acquiring process...
Furthermore, NoWait is not an ``optimization'' with respect to other deadlock resolution schemes. It is just one scheme with its own properties. Many previous papers
have shown that NoWait can underperform other 2PL protocols under certain scenarios (e.g., [29]).
\end{screen}

Thanks for your comment, and we are sorry that we did not describe TicToc NoWait optimization. We revised our implementation and describe the optimization as TicToc-NoWait in the paper so that it can be clearly distinguished from the conventional NoWait. 
We reimplemented the optimization method and redraw the graph.
%\input{src/tictoc_repro.tex}

Thanks again for your comment that ``NoWait is not an optimization''. It provides performance degradation, while it provides performance improvement as Silo is accelerated in Fig. \ref{fig:ycsbA_tuple100m_skew09_slprp0-1000_tps}. This is common in any optimization methods. A optimization method performs well in a certain context, while it degrades performance in another context. Thus we claim it can be considered as an optimization method.

\subsection{Reviewer3-D4}

\begin{screen}
Most of the findings discussed in the evaluation of this paper have already been known. Some were discussed in the original papers of these protocols. The
discussion in this paper restates these findings but there is little deeper discussion.
\end{screen}

 In this paper, we first clarified factors that directly affect performance. They are CPU cache, delay, and, version lifetime. We also clarified the relationship between the factors and optimization methods. We then discussed new optimization methods: {\sf read phase extension} and {\sf aggressive GC}. To our knowledge, these are not yet discussed so far. We summarized it in Section \ref{sec:Conclusion}.
%\input{src/key_takeaway.tex}

\subsection{Reviewer3-D5}

\begin{screen}
The evaluation tries to cover a large multi-dimensional space of parameters. But clearly not all the configurations are shown. Please explain which part of the space is evaluated and which part is not.
\end{screen}

Thank you for your suggestion.
We describe a parameter space table in Table \ref{tab:Experimental Parameters} so that readers can understand the analyzed space.

\subsection{Reviewer3-D6}

\begin{screen}
Related to D5, In Figure 7 when showing the effect of invisible read, Silo (with invisible read) outperforms TicToc (without invisible read). In Figure 10, when showing the effect of extra read, TicToc (without extra read) outperforms Silo (with extra read). The two experiments use different parameters and different conclusions can be drawn. Clearly it is possible to pick a specific parameter setting to show one protocol better than another; it is important to demonstrate the effect of certain optimizations in a more general setting.
\end{screen}
 
 Thanks for your comment. We agree with your comment that ``it is important to demonstrate the effect of certain optimizations in a more general setting.''
%
 However, an optimization method performs well in a certain context, while it degrades performance in another context.
%
 In this paper, NoWait performs well for short transactions while it does not for long transactions as in Fig. \ref{fig:ycsbB_tuple100m_skew08_ope10-100_tps}. 

 Aside from this paper, an interesting example is timestamp history optimization in TicToc. Its effect is not observed by original paper \cite{yu2016tictoc}, while it has been confirmed by a recent one \cite{10.14778/3377369.3377373}.

\subsection{Reviewer3-D7}

\begin{screen}
There is no evaluation on TPC-C.
\end{screen}
 
 Thanks for your comment. We think TPC-C is not suitable for our research purpose. It is because we explored performance factors and the relationship between them and optimization methods. For our purpose, TPC-C is too simple to satisfy our requirements. That is the reason why we used YCSB and provided six parameters. We added the following explanation in Section \ref{sec:A Platform for Fair Comparison}.
%\input{src/tpcc.tex}

\section{Response to Reviewer-4}
\subsection{Reviewer4-D1}

\begin{screen}
This paper has several language issues. Starting from the very first sentence (“... concurrency control protocols have [been] proposed for in-memory database
systems.”), it contains numerous syntactic and semantic errors. Some of the errors even make the meaning of sentences opposite. For instance: “... causes optimistic protocols to read excessively \_by interrupting\_ the updating transaction...” should be “as getting interrupted by”.
“... the possibility of being interrupted by the update transaction \_improves\_,...” should be “increases”.Combined with the above issue is the presentation of this paper. For instance, it took a while for this reviewer to capture the overview of this work from the first section.
Its narrative is not easy to follow.
This paper should go through substantial edits aided by native speakers.
\end{screen}

Thanks for your comment. We fully and carefully revised this manuscript, and used a professional proofreading service. 

\subsection{Reviewer4-D2}

\begin{screen}
If CCBench is only to compare a couple CC schemes evaluated in this paper, its value is quite limited. It is unclear whether/how one can extend CCBench for a
new, yet-to-come CC scheme that might be drastically different from existing ones.
Are the authors committed to keep extending CCBench for future CC schemes? If not, it has to be easy for \_others\_ to extend it for their new CC scheme. So far it is
unclear whether that is the case.
\end{screen}
 
Thanks for your comment.
We add the procedure in Section \ref{sec:A Platform for Fair Comparison}. Please see Section \ref{sec:Meta-5} (Meta-5).

\subsection{Reviewer4-D3}

\begin{screen}
The paper has various observations that make sense, such as effects of cache-miss and dirtying additional cache lines. However, they do not look significant enough to motivate yet another optimization to exploit the effects, at least for general cases. For example, the effect of “Extra Read” reported in Section 5.2 is hard to exploit. One cannot blindly place waits to reduce contention although it improved the throughput in this particular case. Unless there is some finding to distill a generally-applicable optimization, the value of these finding is limited.
\end{screen}

In this paper, we propose two new optimization methods.
They are the {\sf read phase extension} that is inspired by the effect of the extra read shown in Figure \ref{fig:ycsbA_tuple100m_skew09_val4-1k_er}, and the {\sf aggressive garbage collection} that is inspired by the negative effect of a long transaction shown in Figure \ref{fig:comp_cicada-ninline_ycsbA_tuple1m_gci1us-1s_tps}.


==> vldb_format/src/opt_table.tex <==
\begin{table*}
 \begin{center}
  \begin{scriptsize}
   \caption{Versatile Optimization Methods in CCBench.
   {\sf ---}: Irrelevant or Incompatible.
   {\sf Org}: Supported by original protocol.
   {\sf CCB}: Supported by CCBench.
   ({\#a}) Proposed in this work. Delay inspired by the extra reads in OCC (Section \ref{sec:Effect of Extra Read and Read Phase Extension Method}).
   ({\#b}) CCBench conducts read lock for hot records and invisible read for non-hot records.
   ({\#c}) {\sf Preempive abort} and {\sf time-stamp history} cannot be applied to others.
   ({\#d}) {\sf No-wait} locking optimization detects a write lock conflict and immediately aborts and retries the transaction. {\sf TicToc-NoWait} releases all locks and re-locks them.
   ({\#e}) Proposed in this work. 
   We applied optimization methods as follows.
   RapidGC: ERMIA and SI in all cases.
   NoWait: Silo in Fig. \ref{fig:ycsbA_tuple100m_skew09_slprp0-1000_tps}.
   Adaptive backoff: TicToc in Fig. \ref{fig:tuple10m_val1k_ycsb_high_tps}.
   %\input{src/diff.tex}
   }
   \label{table::protocol_opt}
   \begin{tabular}[tb]{r|cc|ccc|cc}
    \begin{tabular}{c} {\bf Performance}\\{\bf Factor}\end{tabular}&
    \multicolumn{2}{|c|}{CPU Cache}&\multicolumn{3}{|c|}{Delay by Conflict}&\multicolumn{2}{|c}{Version Lifetime}\\ \hline\hline
    \begin{tabular}{c} {\bf Optimization}\\{\bf Method}          \end{tabular}&
    \begin{tabular}{c} {\sf Decentralized} \\{\sf Ordering}      \end{tabular} &
    \begin{tabular}{c} {\sf Invisible}   \\{\sf Read}            \end{tabular} &
    \begin{tabular}{c} {\sf NoWait on}   \\{\sf Conflict}        \end{tabular} &
    \begin{tabular}{c} {\sf Adaptive}    \\{\sf Backoff}         \end{tabular} &
    \begin{tabular}{c} {\sf Read Phase}  \\{\sf Extension}({\#a})\end{tabular} &
    \begin{tabular}{c} {\sf Assertive}   \\{\sf Version Reuse}   \end{tabular} &
    \begin{tabular}{c} {\sf Rapid}       \\{\sf GC}              \end{tabular} \\  \hline\hline
2PL~\cite{weikum2001transactional} &Org, CCB &---                &CCB           &CCB      &--- & --- &---\\
Silo~\cite{tu2013speedy}           &Org, CCB &Org, CCB           &CCB           &CCB      &CCB & --- &---\\
MOCC~\cite{wang2016mostly}         &Org, CCB &Org, CCB ({\bf b}) &---           &CCB      &CCB & --- &---\\
TicToc({\bf c})~\cite{yu2016tictoc}&Org, CCB &---                &CCB ({\bf d}) &CCB      &CCB & --- &---\\
SI~\cite{jung2013performance}      &---      &---                &---           &CCB      &--- & CCB &CCB\\
ERMIA~\cite{kim2016ermia}          &---      &---                &---           &CCB      &--- & CCB &CCB\\
Cicada~\cite{lim2017cicada}        &Org, CCB &---                &---           &Org, CCB &CCB & CCB &Org, CCB\\
   \end{tabular}
  \end{scriptsize}
 \end{center}
\end{table*}


==> vldb_format/src/prep.tex <==
\section{Preliminaries}
\label{sec:Preparation}
\input{src/protocol}
\input{src/environment}



==> vldb_format/src/protocol.tex <==
\subsection{Concurrency Control Protocols}
\label{sec:Concurrency Control Protocols}

\input{src/key_facets.tex}

{\bf Silo~\cite{tu2013speedy}}~
is an optimistic concurrency control (OCC) protocol consists of a read phase, a validation phase (locking and read-write conflict detection), and a write phase. 
Silo has had an impact on subsequent concurrency control protocols.
FOEDUS~\cite{kimura2015foedus} and MOCC~\cite{wang2016mostly} extend the commit protocol of Silo.
Silo chooses the design of {\sf invisible reads}~\cite{marathe2004design} that do not update the metadata of the records at any read operations.
Therefore the invisible read avoids cache-line conflicts so it provides scalability as shown in \cite{wang2016mostly}.

{\bf TicToc~\cite{yu2016tictoc}}~
\label{protocol::tictoc}
is an optimistic protocol based on timestamp ordering with data driven timestamp management.
TicToc has a larger scheduling space than that of Silo so that TicToc can commit some schedules where Silo can not.
TicToc provides three optimization methods.
{\sf Preemptive abort} conducts abort processing immediately if abort is determined before write locking in validation phase.
{\sf TicToc-NoWait} does not wait for lock releasing at the validation phase.
It instead releases holding locks and retries the validation phase after a fixed duration of wait without abort.
{\sf Timestamp history} expands the scheduling space by recording the write timestamp of an older version so that some of the read operations on the version can be verified after the record is overwritten.

{\bf MOCC~\cite{wang2016mostly}}~exhibits high performance in a wide range of workloads by adaptively switches its policy by adding pessimistic locking and temperature management to Silo. 
MOCC locks high temperature (highly conflicted) records while keeping the order of records locking to avoid deadlocks in the read phase.
MOCC proposes the MOCC Queuing Lock that integrates MCS lock that can be timed out~\cite{scott2001scalable} and reader/writer fairness MCS lock~\cite{mellor1991scalable}.

{\bf Cicada~\cite{lim2017cicada}}~combines optimistic protocol, multi-version protocol, and distributed timestamp generation.
Due to the nature of the optimistic protocol, cache-line conflicts are mitigated among concurrent transactions.
Distributed timestamp generation in Cicada avoids to access to the centralized counter that conventional MVCC protocols require so that Cicada dramatically mitigates cache-line conflicts.
Cicada has a variety of optimization methods.
%
{\sf Early abort} conducts aborts if an abort is predicted during the read phase.
{\sf Best-effort inlining} embeds an inline version in the record header at the top of the version list to reduce indirect reference cost.
{\sf Precheck validation} checks whether read versions are still valid.
{\sf Rapid garbage collection (RapidGC)} is a quick and parallel garbage collection.
{\sf Adaptive backoff} dynamically decides how long to wait for retrying.

{\bf Snapshot Isolation (SI)~\cite{berenson1995critique}} is a MVCC protocol, and can generate write-skew and read-only-transaction anomalies so it does not produce serializable schedules.
Under SI, a transaction reads a snapshot of the latest committed version.
The write operations are also reflected in the snapshot.
%Records with newer timestamps than the start-timestamp of the transaction are out of contention resolution.
SI requires unique timestamp assignment for each transaction to provide snapshots. 
To determine the unique timestamp, a centralized shared counter is required.

{\bf SI with Latch-Free SSN (ERMIA)~\cite{kim2016ermia}}~integrates snapshot isolation and the serial safety net (SSN)~\cite{wang2015serial} exploiting the latch-free mechanism~\cite{wang2017efficiently}.
SSN detects and aborts non-serializable or dangerous transactions which are a possibly non-serializable in consideration of transaction dependency order and commit order. 
%This mechanism requires to be executed serially, but latch-based serial validation has an unacceptable scalability penalty~\cite{jung2013performance}. 
%An efficient mechanism for parallel execution of SSN is the latch-free SSN~\cite{wang2017efficiently}. 
We refer the integration of the snapshot isolation and the latch-free SSN to as {\bf ERMIA} in this paper.

{\bf 2 phase locking (2PL)\cite{weikum2001transactional} \cite{eswaran1976notions}}~
Our 2PL immediately aborts when conflict is detected at the locking phase, and releases all read/write locks at the end of the transaction.
This locking method is called {\sf NoWait} and originally proposed as a deadlock resolution~\cite{10.1145/356842.356846}.
We exploit the mechanism of {\sf NoWait} to optimization.

==> vldb_format/src/read_only_cache_effect.tex <==
% YCSB-C, cache, new
We investigate the strong effect of L3 cache miss illustrated in Fig. ~\ref{fig:ycsbC_tuple1k-1g_ca}.
When cardinality is  $<= 10^5$, L3 cache miss for Silo, TicToc, and Cicada are almost zero as illustrated in Fig. \ref{fig:ycsbC_tuple1k-1g_ca}.
However, as cardinality increases, their throughputs decrease linearly as illustrated in Fig. ~\ref{fig:ycsbC_tuple1k-1g_ca}.
This is considered as L1/L2 cache misses.
Even for read only workload, L3 cache miss has strong effect on performance.

% + mocc
The negative effect of read contentions is reported by Figs. 1 and 6 in \cite{wang2016mostly}.
It points out the cache line conflicts incurred by read lock contentions degrade performance and the difference between OCC and 2PL rapidly increases as threads increase.
%
However, it does not report that the more L3 cache misses on read only workload reduces the distance between OCC and 2PL.
As illustrated in Fig. \ref{fig:ycsbC_tuple1k-1g}, when cardinality is more than $10^7$, Silo, TicToc, and 2PL demonstrate almost the similar throughput, and their L3 cache miss ratio is also the similar as illustrated in Fig. \ref{fig:ycsbC_tuple1k-1g_ca}.
%
In read only workloads, the difference of performance among protocols converges when the size of database is large due to the L3 cache misses.
This fact has not been pointed out so far.

% Insight
{\bf Insight 1.}~
Performance of OCC at read intensive workload is associated with cardinality even entire database is within L3 cache.
This is due to the cache-line conflicts at L1/L2 caches.
Furthermore, performance of OCC at read only workload is associated with cardinality.
If the entire database does not fit in L3 cache, cache-line replacements occur and performance deteriorates.
When the entire database is quite large and occur frequent cache-line replacements, performance of Silo, TicToc, and 2PL converges to the same.
%


==> vldb_format/src/read_phase_extension.tex <==

By comparing Figs.~\ref{fig:ycsbA_tuple100m_skew09_val4-1k_tps} and \ref{fig:ycsbA_tuple100m_skew09_val4-1k_er}, we can find that their graphs illustrate similar curves.
It implies that the throughput and the number of extra reads are correlated.
%
If the above hypothesis holds, adding an artificial delay into the read phase would demonstrate similar result.
%
We conduct such an experiment by setting payload size to 4 bytes.
The result illustrated in Fig.~\ref{fig:ycsbA_tuple100m_skew09_slprp0-1000_tps} shows that a certain amount of additional delay (less than 9000 clocks) improves performance. This effect is similar to that of the extra read.
We refer this artificial delay to as {\sf read phase extension}, and consider as a new optimization method.
The {\sf read phase extension} is configurable with the delay.
%
This optimization can exploit information of access conflicts of each record through the read phase and the validation phase while {\sf adaptive backoff} uses only global information across all the worker threads. 
%This optimization exploits conflicting information through the commit phase (e.g. locking phase and validation phase) to decide the delay. It requires only the thread local information about contentions while the adaptive backoff uses global information across all the worker threads. 

{\bf Insight 3.}~
Consequentially, extra read plays a key role for performance of OCC protocols.
It is known that the contention reduction caused by delay can contribute to performance improvement depending on the situation.
%
A remarkable finding here is that the read phase extension inspired by the extra read can also improve performance in our case.
%
%This kind of extension is similar to the artificial delay (1 micro sec or {\sf \_mm\_pause}) in TicToc-NoWait.
%
Read phase extension is different from {\sf TicToc-NoWait} since the former exploits information of conflicting records inside transaction to adjust the delay, while the delay in latter is fixed.
%
%Read phase extension is different from adaptive backoff since the former exploits 
%
Such additional delay in the read phase and the exploit of thread local information about conflicts has not been proposed as an optimization method so far.
%
%We believe that it should be considered as a new optimization method in addition to NoWait and backoff for the delay control.
%

{\bf Insight 4.}~
As described in Section \ref{sec:When NoWait is Inefficient} and illustrated in Fig. \ref{fig:ycsbB_tuple100m_skew08_ope10-100_tps}, {\sf Wait} outperforms {\sf NoWait } as transaction size increases.
On the other hand, as illustrated in Fig. \ref{fig:ycsbA_tuple100m_skew09_slprp0-1000_tps}, Silo-NoWait outperforms Silo.
Therefore, we cannot give a general statement about which is better, {\sf NoWait} or {\sf Wait}.
It depends on situations.

==> vldb_format/src/related.tex <==
\section{Related Work}
\label{sec:Related Work}
\input{src/related_core.tex}

==> vldb_format/src/related_core.tex <==
%They are DBx1000~\cite{dbx1000}, Trireme~\cite{trireme}, and Peloton~\cite{peloton}.
% DBx1000
%Platforms to analyze CC protocols have been studied.
Yu et al.~\cite{yu2014staring} evaluate CC protocols with DBx1000~\cite{dbx1000} that is open source and used by third person~\cite{10.1145/3399666.3399910}.
They evaluate the scalability of CC protocols with a real machine and an emulator.
Three recent protocols evaluated in this paper~\cite{kim2016ermia}~\cite{wang2016mostly}~\cite{lim2017cicada}
are not included in this paper though DBx1000 offers ~\cite{tu2013speedy, yu2016tictoc}.
% Peloton
Wu et al.~\cite{wu2017empirical} empirically evaluate MVCC protocols with Peloton~\cite{peloton} that is open source.
They evaluate not only the scalability, but also contention effect, read ratio, attributes, memory allocation, and index.
They focus on MVCC and do not evaluate SVCC and modern MVCC protocols evaluated in this paper~\cite{tu2013speedy}~\cite{yu2016tictoc}~\cite{wang2016mostly}~\cite{lim2017cicada}.
% Trireme
Appuswamy et al.\cite{trireme} evaluate CC protocols in four architecture classes: shared everything, partitioned serial execution, delegation, and data-oriented with Trireme that is not open source.
They evaluate four types of architectures and one of their insights describes shared everything architecture is still the best option for contention-tolerant in-memory OLTP engines.
% Cavalia
Wu et al.~\cite{cavalia_paper} proposes a HTM-assisted CC protocol with Cavalia~\cite{cavalia}.
Cavalia lacks all of Silo, TicToc, MOCC, ERMIA, and Cicada.

%
% Difference
%
Compared to these studies, we present the following novelty with CCBench~\cite{thawkccbench} that is open source and enables to apply a variety of optimization methods.
%
First, they evaluate scalability and none of them do not explore the behavior of protocols fixing thread parallelism at a high degree.
This paper fixes the thread parallelism to 224, and analyze protocols varying seven parameters: skew, payload size, transaction size, read ratio, cardinality, and read-modify-write or not.
%
Second, this paper first discusses the relationship between performance factors and optimization methods. We classify variety of methods into three class of performance factors: cache, delay, and version lifetime.
%
Third, through the analysis, we suggest three new optimization methods.
We propose {\sf Assertive Version Reuse} to avoid putting a load to memory manager, and implement it into CCBench.
We propose {\sf Read Phase Extension} through the analysis of extra read that has been considered to an overhead, and implement it into CCBench.
We propose {\sf Aggressive Garbage Collection} to overcome the limit of the state of the art garbage collection, and discuss its design.
%

% others
CC protocols for distributed systems are evaluated in \cite{wang2020comprehensive,10.14778/3055540.3055548} while this paper focuses on protocols on a single many core architecture.

==> vldb_format/src/repro-proofread.tex <==
\subsection{Reproduction of Prior Work}
	
When evaluating concurrency control protocols, the performance of protocols should be compared under fair conditions.
The meaning of fairness may vary depending on contexts, and we think the following two conditions should be satisfied for a fair comparison.

{\bf Fairness Condition 1.}
Basic modules should be shared: The base modules of an evaluation platform should be shared.
Access methods (e.g., Masstree) and local datasets (read and write sets) need to be shared among protocols.
The effects of memory allocator should be eliminated as much as possible.
The workload should be generated in the same way.
This is important because the performance of a protocol depends on not only the design principle but also engineering details.
The performance of modern protocols is deeply related to the exploitation of underlying hardware, and thus they are sensitive to engineering details.

This above fairness condition may not clearly be satisfied in some cases.
In some papers, we see comparison protocols are not implemented by the authors.
Section 4.2 in Cicada paper [16] states, ”Cicada and existing schemes in DBx1000 share the benchmark code, but have separate data storage and transaction processing engines.”. 
n MOCC paper [27], pure OCC, MOCC, PCC (2PL variants) implementation uses FOEDUS, Dreadlock / WaitDie / BlindDie (2PL variants) uses Orthrus and ERMIA implementation uses ERMIA system.
Three benchmark systems are mixed, In ERMIA paper [14], Silo implementation uses the Silo system while the SI / SSI use the ERMIA system, and the two benchmark systems are mixed.
In these cases, a huge amount of effort by experts is required to avoid unfair comparison.
Such activity is hard for non-experts. Then, we say our fairness condition 1 is not satisfied with their cases.

Wu et al. [29] use the same platform for comparing multiple multi-version protocols, which satisfies the fairness condition 1.
Design philosophy on the platform of CCBench is similar to them.
Their work focuses on evaluating multi-version protocols, and some modern protocols (Cicada, ERMIA, Silo, TicToc, MOCC) are out of scope there.
Yu et al. [30] developed an evaluation platform DBx1000 using a CPU simulator to clarify the scalability impediments of the protocols.
DBx1000 can simulate environments with up to 1024 cores.
Of the seven protocols they targeted, our targets share 2PL, Silo, and TicToc.
On the viewpoint of fairness condition 1, our philosophy is relevant to that of them.

{\bf Fairness Condition 2.}
Applicable optimization techniques should be applied: A protocol consists of a basic method and optimization technique(s).
Sometimes, an optimization technique can be integrated into other basic methods even if a protocol P does not include the optimization technique O at the time of proposal, O can be applied P.
For example, RapidGC is proposed by Cicada [16], and it can be applied to both SI and ERMIA.
NoWait in the validation phase of OCC is proposed by TicToc [31], and it can be applied to Silo.

We think each protocol should be compared with others in the best condition from the viewpoint of fair evaluation.
As described above, the performance of a protocol highly depends on engineering details, and thus applying optimization techniques can improve performance.
One may think such additional optimizations are only laborious and rarely improve performance.
One may have an objection.
By applying an optimization technique to non-original basic methods, the protocol is different from the original one.
However, the application of optimization techniques often improves performance, and we think each protocol should take its best
form in this paper.

Our fairness condition 2 is not satisfied sometimes.
TicToc [31] does not apply NoWait to Silo.
Cicada [16] does not apply RapidGC to ERMIA(SI + SSN) and Hekaton.
Cicada also does not apply adaptive backoff to all protocols used by evaluations in the original paper.

3.2
A Platform for Fair Comparison

We developed CCBench, an evaluation platform for in-memory concurrency control protocols that satisfies the above fairness conditions.
CCBench is publicly available on GitHub [1].
The architecture of CCBench is illustrated in Fig. 1.
To satisfy fairness condition 1, all worker threads in CCBench run in a single node, and it shares the same address space.
Clients and a server run in the same process.
CCBench standardizes the workload generation method.
Client operations (read/write) are generated online.
The generation task is combined with worker threads.
For each transaction execution, workload generation based on the workload setting given before the experiment is performed.
The generated workload information is stored in the STL container, and its memory space reused throughout the experiment.
Allocated memories for a local data structure (read/write set) will be reused for the next transaction, so this improves performance by avoiding memory manager overhead.
We placed record data and concurrency control metadata on the same cache line.

To fairly provide access methods for protocols in CCBench, all protocols use Masstree [17].
We implemented wrappers for the original implementation [3].
CCBench uses mimalloc [4] for a memory allocator.
We conducted memory allocation evenly in all sockets by using the Linux numactl command for stable results in experiments.
CCBench supports the Yahoo! Cloud Serving Benchmark (YCSB) [9] with flexible configurations on six parameters shown in Table 1.
CCBench currently focuses on read and write operations only, and insert and delete operations are out of scope, which is left as future work.
To determine the skew, CCBench uses a fast approximation method [10].

To satisfy fairness condition 2, CCBench provides seven optimization techniques, as shown in Table 2.
(1) Distributed counter: mitigating simultaneous accesses to a shared single counter.
(2) Invisible read: a read operation that does not pollute the cache memory.
(3) Version inlining: allocating space to keep versions in the record header.
(4) NoWait: immediate abort when detecting a conflict.
(5) Extra Read: retry of the read operation in optimistic protocols.
(6) Adaptive backoff: artificial delay before restarting an aborted transaction.
(7) RapidGC: frequently updating timestamp watermark for garbage collection in multi-version protocols.
CCBench enables additional optimization techniques to 2PL, Silo, TicToc, SI, ERMIA, and Cicada.

It should be noted that CCBench does not support read-only optimization techniques introduced in Silo, FOEDUS, MOCC, and ERMIA.
This is because this optimization improves performance in a specific case (i.e., 99\% read-only transactions, 1\% write transactions, skew at 0.99), and such a workload does not appear in this paper

3.3 Implementing Optimization Techniques
2PL: For efficiency, we implemented the reader/writer lock system used in the protocol from scratch.
Silo: We padded the global epoch (64 bits) into the cache line size (64 bytes) to reduce cache pollution that can be caused by the global epoch state change.
The calculation of commit tid is computationally expensive since it requires loops for both the read set and the write set.
We reduced these two loops by calculation at write lock acquisition and read verification, which leads efficiency.

ERMIA: We adopted the latch-free SSN to avoid expensive SSN serial validation.
This implementation avoided the validation from being a critical section.
We implemented the leveraging existing infrastructure that integrates pstamp and sstamp to reduce memory usage.
We optimized the transaction mapping table.
In a straightforward way, the mapping table is designed as a two-dimensional global array with a thread number, TID, cstamp, and last cstamp, which requires a lock manager for updates and read over the rows.
This clearly causes performance degradation due to serialization and cache pollution.
Therefore, we design a data structure that expresses the rows in a one-dimensional array so that it can be latched with a single atomic compare-and-swap (CAS) operation, and performance was improved by avoiding serialization and cache pollution for row element access.
In our ERMIA implementation, we adopted rapid garbage collection (RapidGC) in Cicada.
CASed transaction mapping table objects and version objects are garbage collected based on calculating a threshold that is not accessed by other workers.
The transaction mapping table object exploits our aggressive version reuse described later in this section, and the load on the memory manager is almost eliminated.

TicToc: We implemented all the three optimization methods (no-wait locking in the validation phase, preemptive aborts, timestamp history).
We also improved the algorithm 5 in the original paper by removing redundant read timestamp updates.
It should be noted that if the recorded read timestamp and updating value is the same, there is no need to perform it.

MOCC: In the original paper, MOCC periodically resets temperature information.
This approach changes many cache lines to the invalid state simultaneously, and performance deteriorates.
We instead perform temperature management only for the record that caused read validation failure.
When resetting the temperature, the epoch at that time is added to the temperature information.
At the time of temperature control, the epoch at that time is compared with the epoch attached to the temperature information.
If the epoch is different, we reset the temperature information.
Therefore, the performance was improved by reducing the cache pollution cost and the resetting cost while finely controlling the temperature.
We did not implement MQL lock since our environment has only 4 NUMA nodes, and its novel effect would be limited.
We instead used the reader/writer lock that is also used by 2PL implementation.

Cicada: We implemented all the six optimization techniques (sort write set by contention, pre-check version consistency, adaptive backoff, early aborts, rapid garbage collection, and best-effort inlining).
In addition, we fixed a logical bug, which is the incomplete version consistency check in the validation phase.
The original paper only confirms that the read version is still the visible version.
However, it needs to check if it is the latest visible version too.
If a newer version exists in the observation range, it means that it should have been read and the transaction view will be broken.

As for the one-sided synchronization, we turned off it to provide higher efficiency.
Aggressive Version Reuse for MVCC: In multi-version protocols (SI, ERMIA, and Cicada), some operations such as creating new versions and deleting old versions provide a load on the memory manager, which also true for memory managers with thread-local memory pools.
So, we worked on a new optimization method, aggressive version reuse that avoids overloading the memory manager in multi-version protocols.
By using the aggressive version reuse, each worker thread maintains a container for future version reuse.
When garbage collection occurs, collected versions are stored in this container.
When a new version is requested, it is taken from this container if this container is not empty.
Otherwise, it requests a memory space to the memory manager as usual.
As an optimization in our experiment, our system expects the necessary memory space for the first garbage collection in advance, and it allocates
them in advance. By this optimization, our multi-version protocols put almost no burden on the memory manager.

3.4 Reproduction of Prior Work
Before introducing the result of the evaluation, we need to validate the correctness of CCBench implementation.
We demonstrate that CCBench successfully reproduces the experimental result in some of the prior work.

3.4.1 MOCC
The first reproduction is MOCC [27].
The MOCC we implemented has two differences, as described in Section 3.3.
In order to confirm the graph shown in the original paper can be reproduced by our implementation, we conduct an experiment with the settings shown in Figs 6 and 7 of the original paper.
The settings are also described in the graph caption.
The experimental results are shown in Fig. 2a that the performance scales with the number of threads in the read-only workload.
It reproduces the result of Fig. 6 in the original paper.
The reason is that there is no interaction between threads.
The reason why the performance improvement rate deteriorates after 112 threads is that there
are only 112 physical cores, and the reason that the MOCC performance is slightly lower than Silo is that there is a new calculation process.
On reading, MOCC calculates the temperature information address.
Also, it performs a process for determining whether the temperature is high, which requires memory access.
This process that not exist in Silo, and it may differentiate their results.
The results shown in Figs. 2b and 2c show that when the write rate increases from 0\% to 10\%, the abort rate rapidly increases, and the performance deteriorates.
This experiment is the reproduction of Fig. 7 in the original paper.
The reason is that write operation produces a large amount of the read validation failures.
In Figure 2b, the performance of Silo deteriorates at a write rate of 0-40\%, but the performance improves at a write rate of 40-60\%.
This is a trade-off between reduced read/write contentions due to reduced write operations and frequent read validation failures due to increased read operations.
Compared to that, MOCC shows stable performance, which is considered to progress steadily by temperature control.

3.4.2 TicToc
The second reproduction is TicToc [31].
To confirm our implementation can reproduce the graph shown in the original paper, we experiment with the settings shown in Figs 6, 7, and 8 of the original paper.
The details of the workload are also described in the graph caption.
We set epoch interval long so that it does not to occur cache line contentions in Silo.

Figure 3a shows that Silo and TicToc show comparable performance in read-only workloads, exceeding 20 M tps, which is consistent with Fig. 6 in the original paper.
In Figure 3b, Silo and TicToc both scale in performance.
This is also consistent with Fig. 7 in the original paper.
On the other hand, we found an impressive result.
In Fig. 3c, TicToc shows different performances from Fig. 8 in the original paper.
The performance of TicToc improves as the number of threads increases, but when the number of threads exceeds a specific number, the performance starts
to deteriorate due to an increase in read/write contention.
Therefore, in the original paper, we considered the possibility of a sort of optimization on TicToc and tried to introduce Cicada backoff optimization.
This is shown as TicToc + BO in Fig. 3c.
In our environment, TicToc + BO showed a similar performance curve of TicToc to that of Fig. 9 in the original paper.
The third reproduction is Cicada [16].
The workload was set almost the same as the original paper.
The details of the workload also are described in the graph caption.
The differences from the original paper and here are as follows: 
(1) Redesign and reimplementation of all protocols by authors.
(2) The backoff optimization that Cicada has is installed in all protocols because this optimization technique can be implemented without using Cicada, and we found it is effective for improving performance.

Figures 4a, 4c, 4b, and 4d illustrate the experimental results.
All the results showed the same tendency as the original paper (Figs 6 and 7).
As a result of applying the backoff optimization techniques fairly to all protocols, MOCC or TicToc won over almost all the given parameters,
which is inconsistent with the original paper.
Evaluation on the original paper compared different systems.
Therefore, it is considered that different designs and implementations between the systems affected the performance in the evaluation of the original paper.


==> vldb_format/src/repro.tex <==
\section{Reproduction of Prior Work}
\label{sec:Reproduction of Prior Work}
\input{src/repro_figure}

% CCBench measurement
Before presenting our analysis, we need to validate the correctness of CCBench implementation.
We demonstrate that CCBench successfully reproduces the experimental result in some of the prior work.
% DBx1000 measurement
We also evaluated DBx1000~\cite{dbx1000} that is one of standard analysis platforms as used by third person~\cite{10.1145/3399666.3399910} to validate the behavior of CCBench.
% 
In all graphs about DBx1000, we set {\tt MAX\_TXN\_PER\_PART} to 3000000 so that each plot point shows an average of 20 times of runs and the duration of each run is 4.5 to 10 seconds.
For access method, we used hash index for DBx1000 and Masstree for CCBench.
For memory allocator, we used jemalloc for DBx1000 and {\sf assertive version reuse} for CCBench.

\subsection{MOCC}
The first reproduction is about MOCC~\cite{wang2016mostly}.
Our MOCC implemention has two differences from original one (temperature and MQL), as described in Section~\ref{sec:Implementing Optimization Techniques}.
To confirm the graph shown in the original paper can be reproduced by our implementation,
% hoshino
we experimented with the settings shown in Figs. 6 and 7 in \cite{wang2016mostly}.
The detail of the workload are described in the graph caption.

The experimental results in Fig. \ref{fig:ycsbC_tuple50_tps} appropriately reproduce Fig. 6 in the original paper. The performance scales with the number of threads in the read-only workloads.
%
%The reason is that there is no interaction between threads.
%The reason why the performance improvement rate deteriorates after 112 threads is that there are only 112 physical cores,
We guess the reason why MOCC underperforms Silo after 168 threads is due to the overhead of MOCC.
% hoshino
When MOCC reads a record, it accesses the corresponding temperature information and checks whether the temperature is high or not.
% DBx1000
The results of DBx1000 is also illustrated and their behaviors are similar to ours.

% hoshino
The results in \ref{fig:silo-mocc_tuple50_rratio10-100_tps} and \ref{fig:silo-mocc_tuple50_rratio10-100_ar} appropriately reproduce Fig.7 in the original paper. When the write rate increases from 0\% to 10\%, the abort rate rapidly increases, and the performance deteriorates.
%
The reason is that write operation produces a large amount of the read validation failures.
In Fig.~\ref{fig:silo-mocc_tuple50_rratio10-100_tps}, the performance of Silo deteriorates at a write rate of 0-40\%,
but the performance improves at a write rate of 40-60\%.
This is a trade-off between reduced read/write conflicts due to reduced write operations and frequent read validation failures due to increased read operations.
Compared to that, MOCC shows stable performance, which is considered to progress steadily by temperature control.
% DBx1000
The results of DBx1000 is also illustrated and their behaviors are similar to ours.

% Summary
{\rm MOCC} and {\rm Silo} exhibit scalability in Fig. \ref{fig:ycsbC_tuple50_tps} above, while {\rm MOCC} and {\rm FOEDUS} in Fig. 6 of \cite{wang2016mostly} shows almost the same result.
Fig. \ref{fig:silo-mocc_tuple50_rratio10-100_tps} show the throughput of MOCC and Silo when varying write ratio. This result is almost the same to Fig. 7 in \cite{wang2016mostly}.
Fig. \ref{fig:silo-mocc_tuple50_rratio10-100_ar} abort ratio of {\rm Silo} and {\rm MOCC}, and this is consistent with Fig. 7 in \cite{wang2016mostly}.
%
In summary, CCBench appopriately reproduces the results of MOCC in tendency, and the results of CCBench are consistent with that of DBx1000.
%

\subsection{TicToc}
The second reproduction is about {\rm TicToc}~\cite{yu2016tictoc}.
To confirm our implementation can reproduce the graph shown in \cite{yu2016tictoc},
we experimented with the settings shown in Figs. 6, 7, and 8 in \cite{yu2016tictoc}.
The detail of the workload are described in the graph caption.
We set epoch interval longer than 40 ms so that cache-line conflicts for global epoch rarely occur in {\rm Silo}.
\input{src/tictoc_repro.tex}

We found a noteworthy phenomenon.
In Fig.~\ref{fig:tuple10m_val1k_ycsb_high_tps}, the behaviors of {\rm Silo} and {\rm TicToc'} are different from those of Fig. 8 in \cite{yu2016tictoc}.
The performance of {\rm TicToc'} improves as the number of threads increases,
but when the number exceeds a certain value,
the performance starts to deteriorate due to an increase in the read/write conflicts.
Therefore, we consider a sort of backoff is applied to {\rm TicToc} in \cite{yu2016tictoc}, and attach {\sf adaptive backoff} to {\rm TicToc}.
This is shown as {\rm T'+BO} in Fig.~\ref{fig:tuple10m_val1k_ycsb_high_tps}.
{\rm T'+BO} shows a similar performance curve of that of Fig. 9 in \cite{yu2016tictoc}.
We consider that the original TicToc protocol shown as {\rm T+ONW} demonstrate lower performance due to excessive delay and read validation failures.
{\sf TicToc-NoWait} releases all locks at detecting a write lock conflict in validation phase, inserts fixed delays, and retries validation phase.
The amout of this delays is not controllable and it extends read phase, which tends to fail read validation.
Therefore, {\rm T+ONW} show low performance in this graph and {\rm TicToc'} is better due to short read phase.
Hereafter, we denote {\rm TicToc} that adopts the {\sf NoWait} instead of {\sf TicToc-NoWait} in the rest of this paper.
% DBx1000
The results of DBx1000 is also illustrated in the Figures, and their behaviors are similar to ours.

% Summary
Fig. \ref{fig:tuple10m_val1k_ycsbC_tps} above shows Silo and TicToc' exhibit linear scalability in read-only workload, and Fig. 6 in \cite{yu2016tictoc} shows almost the same result.
Fig. \ref{fig:tuple10m_val1k_ycsb_medium_tps} above and Fig. 7(a) in \cite{yu2016tictoc} show almost the same result.
%
In summary, CCBench appopriately reproduces the result of {\rm TicToc} in tendency, and the results of CCBench are consistent with that of DBx1000.

\subsection{Cicada}
\label{sec:Cicada}
The third reproduction is about Cicada~\cite{lim2017cicada}.
The workload parameters were set almost the same as those in \cite{lim2017cicada}.
The details of the workload are described in the graph caption.
The differences of this paper from the original paper are as follows:
(1) redesign and reimplementation of all protocols by authors.
(2) {\sf adaptive backoff} are installed in all protocols.
because it is easily attachable and effective for performance improvement.

Figures
\ref{fig:ycsbA_tuple10m_ope16_rmw_skew099_tps},
\ref{fig:ycsbA_tuple10m_ope16_rmw_skew0-099_th28_tps}, 
\ref{fig:ycsbB_tuple10m_ope16_rmw_skew0-099_th28_tps},
and
\ref{fig:ycsbB_tuple10m_ope1_rmw_skew099_tps}
%
illustrate the experimental results that reproduce Fig. 6a, 6b, 6c, and 7 in the original paper respectively.
%
\input{src/cicada_repro_comment.tex}




==> vldb_format/src/repro_figure.tex <==
 \begin{figure*}[tb]
 \begin{tabular}{ccc}
  \begin{minipage}{0.3\hsize}
   \subcaptionbox{Read Only Workload.\label{fig:ycsbC_tuple50_tps}}
   {\includegraphics[scale=1.1]{fig/reproduction/comp_ycsbC_tuple50_tps.pdf}}
  \end{minipage}
  &
  \begin{minipage}{0.3\hsize}
   \subcaptionbox{Read-Write YCSB. 224 threads.\label{fig:silo-mocc_tuple50_rratio10-100_tps}}
   {\includegraphics[scale=1.1]{fig/reproduction/comp-silo-mocc_tuple50_rratio10-100_tps.pdf}}
  \end{minipage}
  &
  \begin{minipage}{0.3\hsize}
   \subcaptionbox{Read-Write YCSB. 224 threads.\label{fig:silo-mocc_tuple50_rratio10-100_ar}}
   {\includegraphics[scale=1.1]{fig/reproduction/comp-silo-mocc_tuple50_rratio10-100_ar.pdf}}
  \end{minipage}
 \end{tabular}
 \caption{Reproduction of MOCC. YCSB, 50 records, 10 ops/trans, Skew 0, Payload 4 bytes, reads are pure read, writes are read modify write.}
\end{figure*}

\begin{figure*}[tb]
  \begin{tabular}{ccc}
    \begin{minipage}{0.33\hsize}
      \subcaptionbox{YCSB (Read-Only). 2 queries per transaction, skew 0.\label{fig:tuple10m_val1k_ycsbC_tps}}
      {\includegraphics[scale=1.02]{fig/reproduction/comp_tuple10m_val1k_ycsbC_tps.pdf}}
    \end{minipage}
    &
    \begin{minipage}{0.33\hsize}
      \subcaptionbox{YCSB (Medium Contention). 16 queries per transaction, 90\% reads-10\% writes, skew 0.8.\label{fig:tuple10m_val1k_ycsb_medium_tps}}
      {\includegraphics[scale=1.02]{fig/reproduction/comp_tuple10m_val1k_ycsb_medium_tps.pdf}}
    \end{minipage}
    &
    \begin{minipage}{0.33\hsize}
      \subcaptionbox{YCSB (High Contention). 16 queries per transaction, 50\% reads-50\% writes, skew 0.9\label{fig:tuple10m_val1k_ycsb_high_tps}}
      {\includegraphics[scale=1.02]{fig/reproduction/comp_tuple10m_val1k_ycsb_high_tps.pdf}}
    \end{minipage}
  \end{tabular}
  \caption{Reproduction of TicToc. 10M records, payload 1K bytes.}
\end{figure*}

\begin{figure*}[tb]
  \begin{tabular}{cccc}
    \begin{minipage}{0.23\hsize}
     \subcaptionbox{Write-Intensive. 16 requests/trans, skew 0.99, 50\% RMW - 50\% pure reads\label{fig:ycsbA_tuple10m_ope16_rmw_skew099_tps}}
      {\includegraphics[scale=0.8]{fig/reproduction/comp_ycsbA_tuple10m_ope16_rmw_skew099_tps.pdf}}
    \end{minipage}
    &
    \begin{minipage}{0.23\hsize}
      \subcaptionbox{Write-Intensive. 28 threads. 16 requests/trans, 50\% RMW - 50\% pure reads\label{fig:ycsbA_tuple10m_ope16_rmw_skew0-099_th28_tps}}
      {\includegraphics[scale=0.8]{fig/reproduction/comp_ycsbA_tuple10m_ope16_rmw_skew0-099_th28_tps.pdf}}
    \end{minipage}
    &
    \begin{minipage}{0.23\hsize}
      \subcaptionbox{Read-Intensive. 28 threads. 16 requests/trans, 5\% RMW - 95\% pure reads\label{fig:ycsbB_tuple10m_ope16_rmw_skew0-099_th28_tps}}
      {\includegraphics[scale=0.8]{fig/reproduction/comp_ycsbB_tuple10m_ope16_rmw_skew0-099_th28_tps.pdf}}
    \end{minipage}
   &
    \begin{minipage}{0.23\hsize}
      \subcaptionbox{Read-Intensive. 1 requests/trans, skew 0.99, 5\% RMW - 95\% pure reads\label{fig:ycsbB_tuple10m_ope1_rmw_skew099_tps}}
      {\includegraphics[scale=0.8]{fig/reproduction/comp_ycsbB_tuple10m_ope1_rmw_skew099_tps.pdf}}
    \end{minipage}
  \end{tabular}
  \caption{Reproduction of Cicada. 10M records, payload 100 bytes}
\end{figure*}


==> vldb_format/src/tictoc_repro.tex <==
The experimental results are shown in Figs. \ref{fig:tuple10m_val1k_ycsbC_tps}, \ref{fig:tuple10m_val1k_ycsb_medium_tps}, and \ref{fig:tuple10m_val1k_ycsb_high_tps}.
{\sf TicToc'} uses NoWait optimization intead of {\sf TicToc-NoWait}.
When a write lock collision is detected, the transaction aborts and retries.
{\sf T + ONW} uses all TicToc original optimizations including {\sf TicToc-NoWait}.
{\sf T'+ BO} is TicToc' with Cicada adaptive backoff.

Fig.~\ref{fig:tuple10m_val1k_ycsbC_tps} shows that Silo and TicToc' show comparable performance
in read-only workloads exceeding 20 M tps, which is consistent with Fig. 6 in the original paper.
In Fig.~\ref{fig:tuple10m_val1k_ycsb_medium_tps}, Silo, and TicToc' both scale in performance.
This is also consistent with Fig. 7 in the original paper.
Silo shows a performance of about 4M tps, and the performance of TicToc' was slightly lower than that.
% DBx1000
The results of DBx1000 is also illustrated in the Figures, and their behaviors are similar to ours.

==> vldb_format/src/tmp/related_core.tex <==
{\sf

Yu et al.~\cite{yu2014staring} evaluated concurrency control protocols with one thousand cores.
The protocols are three 2PLs and four T/Os.
As for the benchmarks, YCSB and TPC-C are used.
Throughputs and the breakdown of execution time are shown.
Five recent protocols evaluated in this paper~\cite{tu2013speedy}~\cite{kim2016ermia}~\cite{wang2016mostly}~\cite{yu2016tictoc}~\cite{lim2017cicada} were not included.
Wu et al.~\cite{wu2017empirical} empirically evaluated MVCC protocols.
They discussed the theory and techniques superior in some workload situations.
They focused on MVCC and did not evaluate SVCC protocols proposed recently~\cite{wang2016mostly}~\cite{tu2013speedy}~\cite{yu2016tictoc}~\cite{lim2017cicada}
Harding et al.~\cite{10.14778/3055540.3055548} evaluated distributed concurrency control protocols.
No distributed protocols are evaluated in this paper.

Platforms to evaluate transaction processing are important and have been studied.
It includes Trireme~\cite{trireme}, Shore-MT~\cite{10.1145/1516360.1516365}, DBx1000~\cite{dbx1000} and Peloton~\cite{peloton}.
The evaluations of these studies provide users mainly a way to investigate the scalability of protocols, which is significant today for increasing CPU cores.
On the other hand, none of them does not care varying workload parameters at a highly parallel environment.
This paper fixes the number of worker thread to 224, and provides analysis with varying other parameters: skew, payload size, transaction size, and cardinality.
%
Besides, this paper enables to apply optimization techniques to all the protocols even though it has not been applied in the original paper.
%
}


==> vldb_format/src/tmp/repro-proofread.tex <==
\subsection{Reproduction of Prior Work}
	
When evaluating concurrency control protocols, the performance of protocols should be compared under fair conditions. The meaning of fairness may vary depending on contexts, and we think the following two conditions should be satisfied for a fair comparison.

Fairness Condition 1. Basic modules should be shared: The base modules of an evaluation platform should be shared. Access methods (e.g., Masstree) and local datasets (read and write sets) need to be shared among protocols. The effects of memory allocator should be
eliminated as much as possible. The workload should be generated in the same way. This is important because the performance of a protocol depends on not only the design principle but also engineering details. The performance of modern protocols is deeply related to the exploitation of underlying hardware, and thus they are sensitive to engineering details.

This above fairness condition may not clearly be satisfied in some cases. In some papers, we see comparison protocols are not implemented by the authors. Section 4.2 in Cicada paper [16] states, ”Cicada and existing schemes in DBx1000 share the benchmark code, but have separate data
storage and transaction processing engines.”. In MOCC paper [27], pure OCC, MOCC, PCC (2PL variants) implementation uses FOEDUS, Dreadlock / WaitDie / BlindDie (2PL variants) uses Orthrus and ERMIA implementation uses ERMIA system. Three benchmark systems are mixed, In ERMIA paper [14], Silo implementation uses the Silo system while the SI / SSI use the ERMIA system, and the two benchmark systems are mixed. In these cases, a huge amount of effort by experts is required to avoid unfair comparison. Such activity is hard for non-experts. Then, we say our fairness condition 1 is not satisfied with their cases.

Wu et al. [29] use the same platform for comparing multiple multi-version protocols, which satisfies the fairness condition 1. Design philosophy on the platform of CCBench is similar to them. Their work focuses on evaluating multi-version protocols, and some modern protocols (Cicada, ERMIA, Silo, TicToc, MOCC) are out of scope there. Yu et al. [30] developed an evaluation platform DBx1000 using a CPU simulator to clarify the scalability impediments of the protocols. DBx1000 can simulate environments with up to 1024 cores. Of the seven protocols they targeted, our targets share 2PL, Silo, and TicToc. On the viewpoint of fairness condition 1, our philosophy is relevant to that of them.

Fairness Condition 2. Applicable optimization techniques should be applied: A protocol consists of a basic method and optimization technique(s). Sometimes, an optimization technique can be integrated into other basic methods even if a protocol P does not include the optimization technique O at the time of proposal, O can be applied P. For
example, RapidGC is proposed by Cicada [16], and it can be applied to both SI and ERMIA. NoWait in the validation phase of OCC is proposed by TicToc [31], and it can be applied to Silo.

We think each protocol should be compared with others in the best condition from the viewpoint of fair evaluation. As described above, the performance of a protocol highly depends on engineering details, and thus applying optimization techniques can improve performance. One may think such additional optimizations are only laborious and rarely improve
performance. One may have an objection. By applying an optimization technique to non-original basic methods, the protocol is different from the original one. However, the application of optimization techniques often improves performance, and we think each protocol should take its best
form in this paper.

Our fairness condition 2 is not satisfied sometimes. TicToc [31] does not apply NoWait to Silo. Cicada [16] does not apply RapidGC to ERMIA(SI + SSN) and Hekaton. Cicada also does not apply adaptive backoff to all protocols used by evaluations in the original paper.

3.2
A Platform for Fair Comparison

We developed CCBench, an evaluation platform for in-memory concurrency control protocols that satisfies the above fairness conditions. CCBench is publicly available on GitHub [1]. The architecture of CCBench is illustrated in Fig. 1. To satisfy fairness condition 1, all worker threads in CCBench run in a single node, and it shares the same address space.
Clients and a server run in the same process. CCBench standardizes the workload generation method. Client operations (read/write) are generated online. The generation task is combined with worker threads. For each transaction execution, workload generation based on the workload setting given before the experiment is performed. The generated workload information is stored in the STL container, and
its memory space reused throughout the experiment. Allocated memories for a local data structure (read/write set) will be reused for the next transaction, so this improves performance by avoiding memory manager overhead. We placed record data and concurrency control metadata on the same cache
line.

To fairly provide access methods for protocols in CCBench, all protocols use Masstree [17]. We implemented wrappers for the original implementation [3]. CCBench uses mimalloc [4] for a memory allocator. We conducted memory allocation evenly in all sockets by using the Linux numactl command for stable results in experiments. CCBench supports the Yahoo! Cloud Serving Benchmark (YCSB) [9] with flexible configurations on six parameters shown in Table 1. CCBench currently focuses on read and write operations only, and insert and delete operations are out of scope, which is left as future work. To determine the skew, CCBench uses a fast
approximation method [10].

To satisfy fairness condition 2, CCBench provides seven optimization techniques, as shown in Table 2. (1) Distributed counter: mitigating simultaneous accesses to a shared single counter. (2) Invisible read: a read operation that does not pollute the cache memory. (3) Version inlining: allocating space to keep versions in the record header. (4)
NoWait: immediate abort when detecting a conflict. (5) Extra Read: retry of the read operation in optimistic protocols. (6) Adaptive backoff: artificial delay before restarting an aborted transaction. (7) RapidGC: frequently updating timestamp watermark for garbage collection in multi-version protocols. CCBench enables additional optimization techniques to 2PL, Silo, TicToc, SI, ERMIA, and Cicada.

It should be noted that CCBench does not support read-only optimization techniques introduced in Silo, FOEDUS, MOCC, and ERMIA. This is because this optimization improves performance in a specific case (i.e., 99\% read-only transactions, 1\% write transactions, skew at 0.99), and such
a workload does not appear in this paper

3.3 Implementing Optimization Techniques
2PL: For efficiency, we implemented the reader/writer lock system used in the protocol from scratch.
Silo: We padded the global epoch (64 bits) into the cache line size (64 bytes) to reduce cache pollution that can be caused by the global epoch state change. The calculation of commit tid is computationally expensive since it requires loops for both the read set and the write set.
We reduced these two loops by calculation at write lock acquisition and read verification, which leads efficiency.

ERMIA: We adopted the latch-free SSN to avoid expensive SSN serial validation. This implementation avoided the validation from being a critical section. We implemented the leveraging existing infrastructure that integrates pstamp and sstamp to reduce memory usage. We optimized the transaction mapping table. In a straightforward way, the mapping table is designed as a two-dimensional global array with a thread number, TID, cstamp, and last cstamp, which requires a lock manager for updates and read
over the rows. This clearly causes performance degradation due to serialization and cache pollution. Therefore, we design a data structure that expresses the rows in a one-dimensional array so that it can be latched with a single atomic compare-and-swap (CAS) operation, and performance was improved by avoiding serialization and cache
pollution for row element access. In our ERMIA implementation, we adopted rapid garbage collection (RapidGC) in Cicada. CASed transaction mapping table objects and version objects are garbage collected based on calculating a threshold that is not accessed by other workers. The transaction mapping table object exploits our aggressive version reuse
described later in this section, and the load on the memory manager is almost eliminated.

TicToc: We implemented all the three optimization methods (no-wait locking in the validation phase, preemptive aborts, timestamp history). We also improved the algorithm 5 in the original paper by removing redundant read timestamp updates. It should be noted that if the recorded read timestamp and updating value is the same, there is no need to
perform it.

MOCC: In the original paper, MOCC periodically resets temperature information. This approach changes many cache lines to the invalid state simultaneously, and performance deteriorates. We instead perform temperature management only for the record that caused read validation failure. When resetting the temperature, the epoch at that time is added
to the temperature information. At the time of temperature control, the epoch at that time is compared with the epoch attached to the temperature information. If the epoch is different, we reset the temperature information. Therefore, the performance was improved by reducing the cache pollution cost and the resetting cost while finely controlling the temperature. We did not implement MQL lock since our
environment has only 4 NUMA nodes, and its novel effect would be limited. We instead used the reader/writer lock that is also used by 2PL implementation.

Cicada: We implemented all the six optimization techniques (sort write set by contention, pre-check version consistency, adaptive backoff, early aborts, rapid garbage collection, and best-effort inlining). In addition, we fixed a logical bug, which is the incomplete version consistency check in the validation phase. The original paper only confirms that the read version is still the visible version. However, it needs to check if it is the latest visible version too. If a newer version exists in the observation range, it means that it should have been read and the transaction view will be broken.

As for the one-sided synchronization, we turned off it to provide higher efficiency. Aggressive Version Reuse for MVCC: In multi-version protocols (SI, ERMIA, and Cicada), some operations such as creating new versions and deleting old versions provide a load on the memory manager, which also true for memory managers with thread-local memory pools.
So, we worked on a new optimization method, aggressive version reuse that avoids overloading the memory manager in multi-version protocols. By using the aggressive version reuse, each worker thread maintains a container for future version reuse. When garbage collection occurs, collected versions are stored in this container. When a new version is requested, it is taken from this container if this container is not empty. Otherwise, it requests a memory space to the memory manager as usual. As an optimization in our experiment, our system expects the necessary memory space for the first garbage collection in advance, and it allocates
them in advance. By this optimization, our multi-version protocols put almost no burden on the memory manager.

3.4 Reproduction of Prior Work
Before introducing the result of the evaluation, we need to validate the correctness of CCBench implementation. We demonstrate that CCBench successfully reproduces the experimental result in some of the prior work.

3.4.1 MOCC
The first reproduction is MOCC [27]. The MOCC we implemented has two differences, as described in Section 3.3.
In order to confirm the graph shown in the original paper can be reproduced by our implementation, we conduct an experiment with the settings shown in Figs 6 and 7 of the original paper. The settings are also described in the graph caption.
The experimental results are shown in Fig. 2a that the performance scales with the number of threads in the read-only workload. It reproduces the result of Fig. 6 in the original paper. The reason is that there is no interaction between threads. The reason why the performance improvement rate deteriorates after 112 threads is that there
are only 112 physical cores, and the reason that the MOCC performance is slightly lower than Silo is that there is a new calculation process. On reading, MOCC calculates the temperature information address. Also, it performs a process for determining whether the temperature is high, which requires memory access. This process that not
exist in Silo, and it may differentiate their results. The results shown in Figs. 2b and 2c show that when the write rate increases from 0\% to 10\%, the abort rate rapidly increases, and the performance deteriorates. This experiment is the reproduction of Fig. 7 in the original paper. The reason is that write operation produces a large amount of the read validation failures. In Figure 2b, the performance of Silo deteriorates at a write rate of 0-40\%, but the performance improves at a write rate of 40-60\%. This is a trade-off between reduced read/write contentions due to reduced write operations and frequent read validation failures due to increased read operations. Compared to that, MOCC shows stable performance, which is considered to progress steadily by temperature control.

3.4.2 TicToc
The second reproduction is TicToc [31]. To confirm our implementation can reproduce the graph shown in the original paper, we experiment with the settings shown in Figs 6, 7, and 8 of the original paper. The details of the workload are also described in the graph caption. We set epoch interval long so that it does not to occur cache line contentions in Silo.

Figure 3a shows that Silo and TicToc show comparable performance in read-only workloads, exceeding 20 M tps, which is consistent with Fig. 6 in the original paper. In Figure 3b, Silo and TicToc both scale in performance. This is also consistent with Fig. 7 in the original paper.
On the other hand, we found an impressive result. In Fig. 3c, TicToc shows different performances from Fig. 8 in the original paper. The performance of TicToc improves as the number of threads increases, but when the number of threads exceeds a specific number, the performance starts
to deteriorate due to an increase in read/write contention.
Therefore, in the original paper, we considered the possibility of a sort of optimization on TicToc and tried to introduce Cicada backoff optimization. This is shown as TicToc + BO in Fig. 3c. In our environment, TicToc + BO showed a similar performance curve of TicToc to that of Fig. 9 in the
original paper. The third reproduction is Cicada [16]. The workload was set
almost the same as the original paper. The details of the workload also are described in the graph caption. The differences from the original paper and here are as follows: (1) Redesign and reimplementation of all protocols by authors. (2) The backoff optimization that Cicada has is installed in all protocols because this optimization technique can be implemented without using Cicada, and we found it is effective for improving performance.

Figures 4a, 4c, 4b, and 4d illustrate the experimental results. All the results showed the same tendency as the original paper (Figs 6 and 7). As a result of applying the backoff optimization techniques fairly to all protocols, MOCC or TicToc won over almost all the given parameters,
which is inconsistent with the original paper. Evaluation on the original paper compared different systems. Therefore, it is considered that different designs and implementations between the systems affected the performance in the evaluation of the original paper.

==> vldb_format/src/tpcc.tex <==
To evaluate protocols at a highly parallel environment, TPC-C benchmark is not suitable.
%
It is because the purpose of this paper is to find out factors that deeply affect performance at a highly parallel environment (i.e. 224 threads) that is highly contended or highly conflicted.
%
First, the workload of TPC-C is low-contention and low-conflict~\cite{wang2016mostly} and thus the workload is not less related to our purpose although this kind of analysis has been conducted in conventional studies~\cite{trireme,wu2017empirical,dbx1000}.
%
Second, the configurable parameters in TPC-C are only the warehouse and the number of threads, and these parameters are not enough for our us who explore performance factors in a variety of situations and we need a set of parameters that can generate such situations.
%
Without using TPC-C, we succeeded to clarify the relationship between three major performance factors and many optimization methods, and to suggest new two optimization methods (read phase extension in Section \ref{sec:Effect of Extra Read and Read Phase Extension Method} and aggressive GC in Section \ref{sec:discussion-towards-version-lifetime-control}).
%


==> vldb_format/src/unknown.tex <==
\section{New Performance Factor}
\input{src/delay}
\input{src/version-lifetime-control}


==> vldb_format/src/version-lifetime-control.tex <==
\section{Control of Version Lifetime}
\label{sec:version-lifetime-control}
\input{src/version-lifetime-control_figure}
%This section describes that MVCC protocols suffer from many versions,
%the state-of-the-art protocols have not overcome the problem yet, and
%more aggressive control of version lifetime is
%necessary for MVCC protocols to achieve high performance under various kinds of workloads.

The life of a version begins when it is created by a corresponding write operation of a transaction.
The version state is called visible during the period when other transactions can read it.
Otherwise, the version state is called non-visible.
Recent CC protocols typically make the version visible at the pre-commit phase of the transaction (e.g. early lock release~\cite{aether}).
After a while, the life of the version ends and it is made non-visible.
SVCC protocols typically make a version by overwriting its previous version,
where the former becomes visible and the later becomes non-visible at the same time.
MVCC protocols typically make a version on a different memory fragment from other visible versions
of the same record, so the life of them do not end
unless the explicit operations such as garbage collection (GC) work.

\subsection{Confirming Overhead of Versions}
\label{sec:problem-many-visible-versions}
% Is this claim correct?
It is claimed that the performance of MVCC should suffer from the existence of many visible versions~\cite{10.14778/2095686.2095689,10.1145/2723372.2749436}.
%The number of visible versions grows rapidly because the protocols demonstrate high throughput with much frequent execution of write operations.
Creating many visible versions leads to a significant burden due to memory exhaustion or increase of cache misses for traversal or installation.
MVCC protocols can provide higher performance than that of SVCC protocols for their larger scheduling spaces.
However, architectural issues sometimes negate the benefits as mentioned in Section \ref{sec:changing_database_size}.
% 
We analyze this knowledge in depth. Proposals of MVCC protocols often demonstrate its novel performance compared to SVCC protocols under high contention workloads.
% using only the throughput.
%The throughput provides knowledge under a macro view, and any knowledge under a micro view is provided.
%We first confirm the claim using the throughput, and then conduct a micro analysis.
%
To begin with, we measured the throughput varying the skew from 0 to 0.99.% for the macro analysis.
The results are shown in Fig.~\ref{fig:comp_tuple100m_skew0-099}.
Here we focus on the difference between Cicada (MVCC) and Silo (SVCC).
In Fig.~\ref{fig:comp_ycsbA_tuple100m_skew0-099_tps} and \ref{fig:comp_ycsbA_tuple100m_skew0-099_ar} of YCSB-A,
Cicada outperforms Silo when skew is higher than 0.8.
% add by kawashima->rev by hoshino
It should be noted that we observed more superiority of Cicada with larger payload size.
%
%In Fig.~\ref{fig:comp_ycsbA_tuple100m_skew0-099_ar}, the abort ratio of Cicada is lower than that of Silo in the same skew range.
%{\bf In Fig.~\ref{fig:comp_ycsbB_tuple100m_skew0-099_tps} and \ref{fig:comp_ycsbB_tuple100m_skew0-099_ar} of YCSB-B, we observe similar behavior with skew 0.95 and 0.99.}\footnote{\bf graph changed. how should we do?}
%It is considered that the skew range of YCSB-B is smaller than that of YCSB-A
%because a larger read ratio leads to smaller contentions even with the same skew.
This behavior can be explained that Cicada has larger scheduling spaces than that of Silo, however, we confirm the claim that the performance of MVCC suffer from many versions~\cite{10.14778/2095686.2095689,10.1145/2723372.2749436}.

% Micro analysis
The large scheduling space is supported by many versions, and it can be an overhead. This overhead has not been clearly analyzed yet on modern protocols. 
%The management of  multiple-version management is not negligible~\cite{weikum2001transactional}.
We show the latency breakdown with skew 0 where MVCC is disadvantageous in Fig.~\ref{fig:latency_breakdown_tuple100m_skew0}.
In Fig.~\ref{fig:comp_cicada-silo_ycsbA_tuple100m_gci10us_224th_main-latency},
and Fig.~\ref{fig:comp_cicada-silo_ycsbB_tuple100m_gci10us_224th_main-latency},
we find the major overhead of Cicada exists in read and write operations rather than validation or GC. 
%
To clarity the reasons of the overhead, we designed a SVCC version of Cicada, Cicada-SV that overwrites the inline versions of Cicada. This behavior does not need to allocate new areas and therefore it performs like a SVCC protocol.
%
We prepared a workload where transactions are completely partitioned to avoid contentions because the Cicada-SV does not cope with the contentions.
The result is illustrated in Fig.~\ref{fig:latency_breakdown_tuple100m_skew0_cicada-sv}.
The latency of Cicada-SV and Silo is almost the same there.
We consider that the overhead of Cicada in Fig.~\ref{fig:comp_cicada-silo_ycsbA_tuple100m_gci10us_224th_main-latency} and \ref{fig:comp_cicada-silo_ycsbB_tuple100m_gci10us_224th_main-latency} is caused by the cost of version chain traversal, and the increase in cache misses.

Since many visible versions incurs performance degradation, its reduction should improve performance. {\sf RapidGC} is an effective optimization method to solve this problem.
To analyze the behavior of {\sf RapidGC}, we varied the {\sf RapidGC} interval setting and measured the throughput of Cicada as illustrated in Fig.~\ref{fig:comp_cicada-ninline_ycsbA_tuple1m_gci1us-1s_tps}.
We observe high throughput when GC interval is less than 100us as claimed in literature~\cite{wu2017empirical,lim2017cicada}.
%
%The remaining plots will be explained in Section~\ref{sec:limitation-of-current-approaches}.
This is because the number of visible versions is small, and most of them are kept in the cache.
Then, can {\sf RapidGC} with short interval perform efficiently for any workloads? The answer is no. We explain details in Section \ref{sec:limitation-of-current-approaches}.

{\bf Insight 5.~}
Silo and TicToc can outperform Cicada even under a low contention situation (skew 0.99, YCSB-B)
though both of them exhibit the same performance at the similar low contention situation as shown in Fig. 7 of \cite{lim2017cicada}.
%Parameter sets besides skew (e.g. write ratio, cardinality, et al) that forms a contention situation should be considered in evaluation.
%
Latency breakdown of Cicada-SV is almost the same as that of Silo, which means version management cost of Cicada is not negligible even under a low contention workload.
Therefore, we claim Fig. in \cite{lim2017cicada} is misleading.
We consider the reasons for this inconsistent result is caused by the use of multiple different reference implementations as mentioned in Section \ref{sec:Cicada}, and we claim the evaluation of CC protocol should be done at a single platform.
%

\subsection{Limit of Current Approach}
\label{sec:limitation-of-current-approaches}
We claim that even state-of-the-art GC does not reduce visible versions enough if there is a long transaction.
This is because modern protocols assume that transaction execution is one-shot, and the size of a transaction is relatively small (e.g. 16 for YCSB).
Long transactions except read-only ones are conventionally unthinkable in modern OLTP studies.
We investigated the behavior of the {\sf RapidGC} using workloads of third experiment shown in Section~\ref{sec:problem-many-visible-versions} with a long transaction.
%
To generate a long transaction, we add an artificial delay at the end of the read phase of them.
Both the long and the short transactions use the same number of operations with the same read-write ratio.
Only one worker thread executes a long transaction,
and the remaining worker threads execute short transactions.
The skew is set to 0 so that conflicts of record accesses rarely occur and do not affect performance, 
even if there exists such a long transaction.

We measured the performance of Cicada under the workload described above, varying {\sf RapidGC} interval settings and the delay of a long transaction.
Fig.~\ref{fig:comp_cicada-ninline_ycsbA_tuple1m_gci1us-1s_tps} illustrates the result.
We could not obtain the result with 1 sec delay because such a case requires huge amount of memory and thus the process was killed by the Linux OOM (out-of-memory) killer.
%
All the results in the Figure with delays saturate their performances. The saturation points are exactly when the GC intervals are the same as the delays of the long transactions.
%
For example, the green line includes long transaction with $10^2$ us delay, and its performance saturates when GC interval is $10^2$ us.
%
It is because current any GCs do not collect visible versions that the active long transaction may be read by active long transactions. Until the transaction finishes, a GC cannot collect versions under the current GC schemes.


%This result can be explained as the actual GC interval becomes around 100 ms.
%Actually, GC interval setting means the calculation interval of the timestamp watermark
%that indicates the visible versions below the timestamp can be collected.
%
%Even if the machine is equipped with 1.5 TB of DRAM, a fatal shortage of memory occurs unless it executes GC at intervals of less than 1 second.
%Even the novel RapidGC does not cope with a simple workload with long transactions.

\if 0
Second, we evaluated the timestamp history optimization of TicToc.
TicToc is classified in SVCC because it maintains one version for one record.
However, we can classify TicToc in MVCC
because it has the timestamp history optimization,
which preserves metadata of the recent versions to have more chances to verify.
It does not have visible contents of multiple versions but does visible metadata of them.
TicToc paper~\cite{yu2016tictoc} reported they could not find
workloads that the optimization takes effect.
Then we also could not find such workloads.
Theoretically, we expect that such optimizations
take effect with more visible versions, but not so many.
\fi

\subsection{Aggressive Garbage Collection}
\label{sec:discussion-towards-version-lifetime-control}

From the limitation of current GC scheme described in Section \ref{sec:limitation-of-current-approaches}, 
we suggest a GC, {\sf Aggressive Garbage Collection} that aggressively collects versions beyond the current ones is necessary to deal the workloads with long transactions. 
%though the page model for MVCC protocols~\cite{weikum2001transactional} assumes that the version lifetime is forever.
%In other words, MVCC protocols must work under the constraint that the number of existing visible versions in the main memory is limited.
%
An example of such a protocol is to integrate MVTO protocol with a GC method that aggressively collects visible versions. Using the protocol, some versions are made non-visible even though active or future transactions need to read them.
Such a protocol may incur read operation failures unlike conventional MVTO, and needs to handle such a case by aborting the transaction and retrying it with a new timestamp.
%
Restricting the amount of versions has been discussed in kVSR~\cite{10.5555/645478.654954} or 2V2PL~\cite{10.1145/320141.320146,10.1145/582318.582330}.
They keep only the latest contiguous versions and less flexible than our suggestion.
We suggest the visible versions do not need to be contiguous, and the number of versions can be flexible on contexts.
%
An interesting topic in this scheme is the risk of starvation. One way for the mitigation can be the management of priorities among transactions such as wait-die~\cite{10.1145/320251.320260}, and this topic has not yet been discussed in modern MVCC studies.

We suggest two optimizations for write operations on the viewpoint of the aggressive protocols.
%
The first optimization is version overwriting that creates a new version by overwriting the memory segment of an old version, which becomes non-visible at the same time, like SVCC protocols.
Version overwriting is efficient because two operations are combined into one operation.
The second optimization is non-visible writes that make versions non-visible from the beginning of their life.
The idea of non-visible writes is originally proposed as Thomas write rule~\cite{10.1145/320071.320076}
%that works as follows: if two ordered write operations for the same record arrived in the opposite order of time, the former operation that arrived later could become non-visible, not making it visible at all. Non-visible writes do not seem to be used by
and recently generalized as Non-visible write rule (NWR)~\cite{nakazono2019invisiblewriterule} to deal with blind writes.
We have a chance to develop novel protocols and optimization techniques on version lifetime control to improve MVCC protocols.

{\bf Insight 6. }
Even state of the art garbage collection can not improve performance of MVCC if a single long transaction is mixed into the workload. An aggressive approach can solve this problem by aggressively change version state to non-visible for both read and write, even though it is still visible.


==> vldb_format/src/version-lifetime-control_figure.tex <==
\begin{figure*}[tb]
\begin{tabular}{cccc}
\begin{minipage}{0.23\hsize}
\subcaptionbox{YCSB-A Throughput \label{fig:comp_ycsbA_tuple100m_skew0-099_tps}}
{\includegraphics[scale=0.9]{fig/version-lifetime-control/comp_ycsbA_tuple100m_skew06-099_tps.pdf}}
\end{minipage}
&
\begin{minipage}{0.23\hsize}
\subcaptionbox{YCSB-A Closing up High Skew \label{fig:comp_ycsbA_tuple100m_skew0-099_ar}}
{\includegraphics[scale=0.9]{fig/version-lifetime-control/comp_ycsbA_tuple100m_skew09-099_tps.pdf}}
\end{minipage}
&
\begin{minipage}{0.23\hsize}
\subcaptionbox{YCSB-B Throughput \label{fig:comp_ycsbB_tuple100m_skew0-099_tps}}
{\includegraphics[scale=0.9]{fig/version-lifetime-control/comp_ycsbB_tuple100m_skew06-099_tps.pdf}}
\end{minipage}
&
\begin{minipage}{0.23\hsize}
\subcaptionbox{YCSB-B Closing up High Skew \label{fig:comp_ycsbB_tuple100m_skew0-099_ar}}
{\includegraphics[scale=0.9]{fig/version-lifetime-control/comp_ycsbB_tuple100m_skew09-099_tps.pdf}}
\end{minipage}
\end{tabular}
\caption{Impact of workload skew: 100M records, 224 threads, payload 4 bytes, 10 ops/trans.}
\label{fig:comp_tuple100m_skew0-099}
\end{figure*}

\begin{figure}[tb]
\begin{tabular}{cc}
\begin{minipage}{0.45\hsize}
\subcaptionbox{YCSB-A \label{fig:comp_cicada-silo_ycsbA_tuple100m_gci10us_224th_main-latency}}
{\includegraphics[scale=0.9]{fig/version-lifetime-control/comp_cicada-silo_ycsbA_tuple100m_gci10us_224th_main-latency.pdf}}
\end{minipage}
&
\begin{minipage}{0.45\hsize}
\subcaptionbox{YCSB-B \label{fig:comp_cicada-silo_ycsbB_tuple100m_gci10us_224th_main-latency}}
{\includegraphics[scale=0.9]{fig/version-lifetime-control/comp_cicada-silo_ycsbB_tuple100m_gci10us_224th_main-latency.pdf}}
\end{minipage}
\end{tabular}
\caption{Latency breakdown: skew 0, 100M records, 224 threads, payload 4 bytes, 10 ops/trans.}
\label{fig:latency_breakdown_tuple100m_skew0}
\end{figure}

\begin{figure}[tb]
\begin{tabular}{cc}
\begin{minipage}{0.45\hsize}
\subcaptionbox{YCSB-A \label{fig:comp_cicada-silo-part_ycsbA_tuple100m_gci10us_224th_main-latency}}
{\includegraphics[scale=0.9]{fig/version-lifetime-control/comp_cicada-silo-part_ycsbA_tuple100m_gci10us_224th_main-latency.pdf}}
\end{minipage}
&
\begin{minipage}{0.45\hsize}
\subcaptionbox{YCSB-B \label{fig:comp_cicada-silo-part_ycsbB_tuple100m_gci10us_224th_main-latency}}
{\includegraphics[scale=0.9]{fig/version-lifetime-control/comp_cicada-silo-part_ycsbB_tuple100m_gci10us_224th_main-latency.pdf}}
\end{minipage}
\end{tabular}
\caption{Latency breakdown of Cicada-SV and Silo under a partitioned workload.}
\label{fig:latency_breakdown_tuple100m_skew0_cicada-sv}
\end{figure}


%
% long tx
%
\begin{figure}[t]
  \centering
  \includegraphics[scale=1.0]{fig/version-lifetime-control/comp_cicada-ninline_ycsbA_tuple1m_gci1us-1s_tps.pdf}
  \caption{Analysis of RapidGC: YCSB-A, skew 0, 224 threads, 1M records, payload 4 bytes, 10 ops/trans.
Each legend indicates the inserted delay of long transactions.}
  \label{fig:comp_cicada-ninline_ycsbA_tuple1m_gci1us-1s_tps}
\end{figure}


